Ontology Interoperability: A Comprehensive Framework for Industry-Scale Applications

Different ontologies with conflicting and overlapping concepts cause havoc in the design, develop, and deploy phases of ontology-driven applications. In this work, we propose a comprehensive ontology interoperability framework for industrial-scale ontology-driven applications. The framework employs three state-of-the-art semantic techniques in different phases of the ontology engineering (OE) life cycle: ontology design patterns (ODPs) in the design phase, ontology matching and versioning (OM\&OV) in the develop phase, and ontology validation (OVA) in the deploy phase, to achieve better ontology interoperability.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> anu-thesis-abstract.tex <==
\section*{Abstract}

Different ontologies with conflicting and overlapping concepts cause havoc in the design, develop, and deploy phases of ontology-driven applications. In this work, we propose a comprehensive ontology interoperability framework for industrial-scale ontology-driven applications. The framework employs three state-of-the-art semantic techniques in different phases of the ontology engineering (OE) life cycle: ontology design patterns (ODPs) in the design phase, ontology matching and versioning (OM\&OV) in the develop phase, and ontology validation (OVA) in the deploy phase, to achieve better ontology interoperability.

We propose a set of new ODPs to capture common and well-agreed concepts and relations in the smart building domain. To do so, we first analyse four popular ontologies used in the smart building domain (Brick Schema, RealEstateCore, Project Haystack, and Google Digital Buildings) and evaluate these ontologies through axiomatic design and empirical assertion using real-world building data. While there is no one-size-fits-all ontology, we then extract the merits of each ontology to build ODPs, including building spaces, equipment and systems, points and measurements.

We develop a novel OM system using large language models (LLMs). Agent-OM uses state-of-the-art LLM agents that leverage infrastructure to deliver improved OM performance in a fully-automated and domain-independent manner. Agent-OM participates in the Ontology Alignment Evaluation Initiative (OAEI) 2025 campaign and showcases its generative capability in handling OM tasks at various levels of granularity. Agent-OV extends Agent-OM to explicitly target OV tasks, including new OM4OV task formulation and evaluation, with a cross-reference mechanism for OM4OV optimisation.

We present two new OVA approaches. We propose a crowdsourced OM validation approach to unlock the potential of using crowdsourcing techniques for OM validation. With three quality-assurance mechanisms, this approach can be integrated with existing OM systems to mitigate the bias and reduce the workload of human annotators. Secondly, we propose ontology-compliant knowledge graphs (OCKGs) to validate the ontology in KGs. We define three subtasks: ontology compliance within a KG, ontology compliance over KGs, and pattern-based compliance. We demonstrate the process of constructing OCKGs and highlight their utility in ontology validation and decision-making.

A video presentation of the thesis work is available at \url{https://figshare.com/projects/Zhangcheng_Qiang_s_PhD_Project/284749}.

==> anu-thesis-acknowledgements.tex <==
\section*{Acknowledgements}

First of all, I would like to thank my family for their support during my PhD journey. I would like to thank the academics, students, and professional staff in the Research School of Computing and the Graduate Research School at the Australian National University (ANU) for their continued support during my PhD journey.

I am very grateful to my master's supervisors, Pari Delir Haghighi, Prem Prakash Jayaraman, and Yuxin Zhang, for opening the research gate for me. It was my good fortune to have Armin Haller, Sergio José Rodríguez Méndez, and Pouya Ghiasnezhad Omran contribute as initial supervisors for my PhD. They inspired my choice of an ontology engineering topic, and without their support, I could not have been embedded in the welcoming, intellectually challenging, and rewarding research environment offered by the ANU.

I want to particularly mention my appreciation for my growth as a scholar made by my former supervisory panel chair, Qing Wang (ANU). Unfortunately, and sadly for me, she is no longer alive to witness this important event of the completion of my thesis. I will always be grateful for what she gave me as the foundation of my research career. Alex Potanin, as her successor, has done a remarkable job carrying on her legacy.

My sincere thanks go to Weiqing Wang (also known as Teresa Wang). Her feedback is always timely, instructive, and insightful, and I deeply admire her academic rigour and passion for lifelong learning. I feel privileged to have Jing Jiang (ANU) on my supervisor panel and to benefit from her efforts to connect natural language processing (NLP) to the Semantic Web Community. My supervisor from the Commonwealth Scientific and Industrial Research Organisation (CSIRO), Subbu Sethuvenkatraman, and his colleagues Stuart Hands, Daniel Hugo, and Gabe Fierro, have helped bring my work to real-world industry-scale applications.

Finally, I would like to express my deepest gratitude to my primary supervisor, Kerry (Lea) Taylor, widely known as the key contributor to Semantic Sensor Network (SSN) and Sensor, Observation, Sample, and Actuator (SOSA). Her research has inspired many subsequent research and innovations, serving as an Archimedes' lever that cracks the nuts of using ontologies for the Internet of Things (IoT). As an academic supervisor, she has supported me throughout my PhD journey and provided constructive advice on my work. As a life coach, she has shared her life experiences with me and helped me overcome many challenging obstacles. As a world-class researcher, she set a great example for all young researchers.

\newpage

\textbf{Funding Acknowledgement:} I acknowledge the funding support from the Commonwealth Scientific and Industrial Research Organisation (CSIRO).

\textbf{Declaration on Generative AI:} During the preparation of this work, the author used generative artificial intelligence (AI) tools in order to grammar and spell check, and to improve the text readability. After using the tools, the author reviewed and edited the content and takes full responsibility for the thesis content.

Generative AI is intrinsic to the research reported here and in this role it is properly identified throughout the work.

==> anu-thesis-acronyms.tex <==
\newacronym{ANU}{ANU}{Australian National University}
\newacronym{CSIRO}{CSIRO}{Commonwealth Scientific and Industrial Research Organisation (Australia's National Science Organisation)}

\newacronym{KG}{KG}{Knowledge Graph}
\newacronym{OE}{OE}{Ontology Engineering}
\newacronym{ODP}{ODP}{Ontology Design Pattern}
\newacronym{OM}{OM}{Ontology Matching}
\newacronym{OV}{OV}{Ontology Versioning}
\newacronym{OVA}{OVA}{Ontology Validation}
\newacronym{OVF}{OVF}{Ontology Verification}
\newacronym{DOVA}{DOVA}{Data-Driven Ontology Validation}
\newacronym{OCKG}{OCKG}{Ontology-Compliant Knowledge Graph}
\newacronym{SE}{SE}{Software Engineering}
\newacronym{SOSA}{SOSA}{Sensor, Observation, Sample, and Actuator Ontology}
\newacronym{SSN}{SSN}{Semantic Sensor Network Ontology}
\newacronym{SAREF}{SAREF}{Smart Applications REFerence Ontology}
\newacronym{DUL}{DUL}{DOLCE+DnS Ultralite Ontology}
\newacronym{PROV-O}{PROV-O}{Provenance Ontology}
\newacronym{ISWC}{ISWC}{International Semantic Web Conference}
\newacronym{WOP}{WOP}{Workshop on Ontology Design and Patterns}
\newacronym{OM@ISWC}{OM@ISWC}{Ontology Matching Workshop at ISWC}
\newacronym{OAEI}{OAEI}{Ontology Alignment Evaluation Initiative}
\newacronym{OWL}{OWL}{Web Ontology Language}
\newacronym{RDFS}{RDFS}{Resource Description Framework Schema}
\newacronym{SKOS}{SKOS}{Simple Knowledge Organisation System}
\newacronym{AHU}{AHU}{Air Handling Unit}
\newacronym{HVAC}{HVAC}{Heating, Ventilation, and Air Conditioning}
\newacronym{AAE}{AAE}{Actuation-Actuator-Effect}
\newacronym{SAN}{SAN}{Semantic Actuator Network Ontology}
\newacronym{EEP}{EEP}{Execution-Executor-Procedure}
\newacronym{SEAS}{SEAS}{Smart Energy Aware Systems Ontology}
\newacronym{AML}{AML}{AgreementMakerLight}
\newacronym{ML}{ML}{Machine Learning}
\newacronym{LLM}{LLM}{Large Language Model}
\newacronym{XAI}{XAI}{Explainable Artificial Intelligence}
\newacronym{RAG}{RAG}{Retrieval-Augmented Generation}
\newacronym{SHACL}{SHACL}{Shapes Constraint Language}

\newacronym{TBox}{TBox}{Terminological Box}
\newacronym{ABox}{ABox}{Assertion Box}
\newacronym{OQuaRE}{OQuaRE}{Ontology Quality Evaluation}
\newacronym{LBD}{LBD}{Linked Building Data}
\newacronym{ODPs}{ODPs}{Ontology Design Patterns}
\newacronym{CAGR}{CAGR}{Compound Annual Growth Rate}
\newacronym{5Vs}{5Vs}{Volume, Variety, Velocity, Veracity, and Value}
\newacronym{IoT}{IoT}{Internet of Things}
\newacronym{BMS}{BMS}{Building Management System}
\newacronym{ASO}{ASO}{Automated System Optimisation}
\newacronym{Brick}{Brick}{Brick Schema}
\newacronym{RECore}{RECore}{RealEstateCore Ontology}
\newacronym{Haystack}{Haystack}{Project Haystack Ontology}
\newacronym{DB}{DB}{Google’s Digital Buildings}
\newacronym{RDF}{RDF}{Resource Description Framework}
\newacronym{SQuaRE}{SQuaRE}{System product Quality Requirements and Evaluation}
\newacronym{KB}{KB}{Knowledge Base}
\newacronym{IFC}{IFC}{Industry Foundation Classes}
\newacronym{DCH}{DCH}{Data Clearing House (CSIRO Platform)}
\newacronym{HHW}{HHW}{Heating Hot Water}
\newacronym{CHW}{CHW}{Chilled Water}
\newacronym{BOT}{BOT}{Building Topology Ontology}
\newacronym{SPARQL}{SPARQL}{SPARQL Protocol and RDF Query Language}
\newacronym{GeoSPARQL}{GeoSPARQL}{Geographic SPARQL}
\newacronym{QUDT}{QUDT}{Quantities, Units, Dimensions, and Types Ontology}
\newacronym{ASHRAE}{ASHRAE}{American Society of Heating, Refrigerating and Air-Conditioning Engineers (Professional Association)}
\newacronym{NFL}{NFL}{No Free Lunch (Theorem)}
\newacronym{LBD-CG}{LBD-CG}{LBD Community Group}

\newacronym{QA}{QA}{Question Answering}
\newacronym{AI}{AI}{Artificial Intelligence}
\newacronym{CoT}{CoT}{Chain of Thought}
\newacronym{ICL}{ICL}{In-Context Learning}
\newacronym{NLP}{NLP}{Natural Language Processing}
\newacronym{CRUD}{CRUD}{Create, Read, Update, and Delete}
\newacronym{RRF}{RRF}{Reciprocal Rank Fusion}
\newacronym{API}{API}{Application Programming Interface}
\newacronym{DL}{DL}{Deep Learning}
\newacronym{BFO}{BFO}{Basic Formal Ontology}
\newacronym{CoT-SC}{CoT-SC}{CoT with Self-Consistency}
\newacronym{CI}{CI}{Confidence Interval}
\newacronym{ToT}{ToT}{Tree of Thoughts}
\newacronym{GoT}{GoT}{Graph of Thoughts}
\newacronym{SLM}{SLM}{Small Language Model}

\newacronym{RPM}{RPM}{Requests Per Minute}
\newacronym{TPM}{TPM}{Tokens Per Minute}
\newacronym{GPU}{GPU}{Graphics Processing Unit}
\newacronym{CPU}{CPU}{Central Processing Unit}
\newacronym{MELT}{MELT}{Matching EvaLuation Toolkit}
\newacronym{RR}{RR}{Reciprocal Rank}
\newacronym{MRR}{MRR}{Mean Reciprocal Rank}

\newacronym{NLG}{NLG}{Natural Language Generation}
\newacronym{EDOAL}{EDOAL}{Expressive \& Declarative Ontology Alignment Language}
\newacronym{SSSOM}{SSSOM}{Simple Standard for Sharing Ontological Mappings}

\newacronym{CR}{CR}{Cross Reference}
\newacronym{HTML}{HTML}{Hypertext Markup Language}
\newacronym{URI}{URI}{Uniform Resource Identifier}

\newacronym{RLHF}{RLHF}{Reinforcement Learning from Human Feedback}
\newacronym{DPO}{DPO}{Direct Preference Optimization}
\newacronym{TP}{TP}{True Positive}
\newacronym{FP}{FP}{False Positive}

\newacronym{FAIR}{FAIR}{Findable, Accessible, Interoperable, and Reusable}
\newacronym{OWA}{OWA}{Open World Assumption}

==> anu-thesis-dedication.tex <==
\begin{figure}
\centering
{\large\usefont{OT1}{qzc}{m}{n}\selectfont 
To family, friends, and the wonderful universe we are intimately connected with
\\[4cm]\phantom{1}}
\end{figure}

==> anu-thesis-disclaimer.tex <==
\section*{Disclaimer}

This thesis is my original work. Exceptions are properly referenced. Information derived from published and unpublished work has been referenced and cited in the body of the text and listed in the bibliography.

Author's publications arising from the research for this thesis by chapters.

\setcounter{table}{-1}
\begin{table}[!h]
\scriptsize
\centering
\captionsetup{list=no}
\label{tab: publications}
\begin{tabular}{m{2cm}m{12cm}}

\toprule
\textbf{Chapter} & \textbf{Publications} \\
\midrule

\multirow{1}{*}{Chapter~\ref{chap: introduction}} &
\bibentry{qiang2025ecosystem} \\
\midrule

\multirow{1}{*}{Chapter~\ref{chap: literature}} &
\bibentry{qiang2025ecosystem} \\
\midrule

\multirow{1}{*}{Chapter~\ref{chap: building-odps}} &
\bibentry{qiang2023systematic} \\
\midrule

\multirow{1}{*}{Chapter~\ref{chap: agent-om}} &
\bibentry{qiang2023agent} \\ 
\midrule

\multirow{1}{*}{Chapter~\ref{chap: om4ov}} &
\bibentry{qiang2024om4ov} \\ 
\midrule

\multirow{1}{*}{Chapter~\ref{chap: om-validation}} &
\bibentry{qiang2026unlocking} \\
\midrule

\multirow{1}{*}{Chapter~\ref{chap: ockgs}} &
\bibentry{qiang2023ontology} \\
\midrule

\multirow{1}{*}{Chapter~\ref{chap: conclusion}} &
\bibentry{qiang2025ecosystem} \\
\midrule

\multirow{1}{*}{Appendix A} &
\bibentry{qiang2023systematic} \\
\midrule

\multirow{1}{*}{Appendix B} &
\bibentry{qiang2025oaei} \\
\midrule

\multirow{1}{*}{Appendix C} &
\bibentry{qiang2024oaei} \\
\bottomrule

\end{tabular}
\end{table}

\begin{flushright}
	\includegraphics[width=0.2\textwidth]{author-signature.pdf}\\[2mm]
	\authorfullname
	
	\fullthesisdate
\end{flushright}

==> qiang-anu-thesis-appendices/agent-om-oaei-2025.tex <==
\chapter[Agent-OM Results for OAEI 2025]{Agent-OM Results for OAEI 2025}
\label{appendix: agent-om-oaei-2025}

This appendix presents the system paper submitted to the Ontology Alignment Evaluation Initiative (OAEI)~\citep{oaei} 2025 campaign as required by participation.

We present the results obtained in the OAEI 2025 campaign using our Agent-OM system. This is our first participation in the OAEI campaign, featuring two variants with different large language models (LLMs): The \emph{production} version uses commercial LLMs for optimal performance, while the \emph{lite} version uses open-source LLMs for cost-effectiveness. Experimental results in eight OAEI tracks demonstrate the generative power of Agent-OM in handling OM tasks from diverse domains, languages, and vocabularies. We also outline future directions to improve our system.

\section{Presentation of the System}

Agent-OM is one of the leading systems for ontology matching (OM). Leveraging the power of LLMs and the advantages of LLM agents, the system achieves performance comparable to state-of-the-art systems in simple OM tasks and surpasses them in complex and few-shot OM tasks.

\subsection{New features of Agent-OM 2025 edition}

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]

\item Agent-OM has been extended for better functionality and usability.
{\renewcommand{\labelitemi}{-}
\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item We develop Agent-OM-Lite, a free and lite version for cost-effectiveness in large-scale OM.
\item We extend Agent-OM for ontology versioning~\citep{qiang2024om4ov} and LLM hallucination evaluation~\citep{qiang2024oaei}.
\item We extend Agent-OM to support the latest DeepSeek models~\citep{guo2025deepseek} and OpenAI open-source models~\citep{gpt-oss}.
\item We extend the precision-recall-F1 chart used in Agent-OM to an interactive user tool~\citep{p-r-f1-vis}.
\end{itemize}
}

\item Agent-OM has been re-engineered to support OM tasks lacking a reference alignment. We now allow users to upload only the source and target ontologies. If the system detects that no reference alignment exists, it will create a dummy one to enable the pipeline. The alignment generated by Agent-OM itself will subsequently replace the dummy reference file.

\item Agent-OM has been upgraded to interpret OWL restrictions. The key challenge is that these restrictions contain nested logical expressions with blank nodes. The new function is attached to the semantic retriever and now the retriever can capture both hierarchical and logical relationships. Packaged in an LLM-based tool, it can be connected for complex tasks and unplugged for tasks where it is not required.

\item Agent-OM has been optimised for reproducibility. We employ several new hyperparameters to instruct LLMs to return stable output over multiple runs. We use $top\_k = 1$ and $top\_p = 1.0$ to ensure that LLMs always choose the top-one token and do not filter the output. Note that these parameters may not be modifiable in commercial LLMs. For example, the $top\_k$ value is currently not available in OpenAI models. We use $repeat\_penalty = 1.0$ (or similar parameters, $presence\_penalty = 0.0$ and $frequency\_penalty = 0.0$) to assign no penalty for repeated output from LLMs; in other words, to encourage LLMs to produce repetitive and stable outputs.

\end{itemize}

\subsection{Agent-OM in the OAEI 2025 campaign}

There are two Agent-OM variants that participate in the OAEI 2025 campaign.

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item \textbf{Agent-OM} is the production version of Agent-OM. The backend uses commercial LLMs and the corresponding embedding models. The production version achieves optimal performance, but requires extensive access to commercial APIs. The results show slight differences across different runs due to limited support for reproducibly fixing the model's hyperparameters.
\item \textbf{Agent-OM-Lite} is the lite version of Agent-OM. The backend uses open-source LLMs for both language processing and text embedding. Although the performance of the lightweight version is usually poorer than that of the production version, it offers an alternative solution for cost-constrained or security-constrained scenarios. The result is more stable across different runs.
\end{itemize}

\subsubsection{System settings}

Figure~\ref{fig: llm-variations} provides the LLM variations available for OAEI 2025. For commercial API-accessed LLMs used in Agent-OM, gpt-4o~\citep{gpt-4o} with the timestamp tag 2024-05-13 has the optimal performance and stability. However, its API cost can be expensive for large-scale OM tasks. Alternatives include the late-breaking version without the timestamp tag and the mini version gpt-4o-mini~\citep{gpt-4o-mini}. Note that the late-breaking version may produce less stable results, while the mini version can lower the matching performance. For open-source llama-3~\citep{llama-3} models used in Agent-OM-Lite, the large-size model llama-3-70b can perform better than the small-size model llama-3-8b, but the execution time may be longer.

\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{qiang-om-2025-figures/LLM-Variations.png}
\caption{LLM variations available for OAEI 2025.}
\label{fig: llm-variations}
\end{figure}

Table~\ref{tab: hyperparameter-setting} shows the hyperparameter settings for OAEI 2025. We use gpt-4o(-mini) with the text embedding model ada-002~\citep{ada-002} for the production version Agent-OM and llama-3 for Agent-OM-Lite. The global settings of similarity\_threshold = 0.90 and top@k = 3 may not be optimal for each track. We recommend trying different settings to find a customised setting for each task. The new LLM hyperparameters may cause additional execution time for LLMs. If the task does not have a reproducibility requirement, we suggest setting the temperature to 0.0 and ignoring other hyperparameters. There is only a slight difference between multiple runs with this setting. The system hyperparameter $top@k$ is used to restrict the top $k$ matching candidates chosen by Agent-OM and its lite version, while the LLM hyperparameter $top\_k$ is used to restrict the top $k$ tokens selected by the LLM used in Agent-OM and its lite version. The $top\_p$ value is not functional when $top\_k=1$. 

\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.2}
\tabcolsep=0.15cm
\caption{Hyperparameter settings for OAEI 2025.}
\label{tab: hyperparameter-setting}
\begin{adjustbox}{width=1\columnwidth,center}
\begin{tabular}{|c|l|l|}
\hline
\multicolumn{3}{|l|}{\textbf{System Hyperparameters}}                                                                                       \\ \hline
\multicolumn{3}{|l|}{$similarity\_threshold=0.90, top@k=3, seed=42$}                                                                        \\ \hline
\multirow{1}{*}{\textbf{System Variant}} & \multirow{1}{*}{\textbf{LLM}} & \multirow{1}{*}{\textbf{LLM Hyperparameters}}                  \\ \hline
\multirow{2}{*}{\textbf{Agent-OM}}  & gpt-4o(-mini)     & $temperature=0.0, top\_p=1.0, presence\_penalty=0.0, frequency\_penalty=0.0$      \\ \cline{2-3}
                                    & ada-002           & $embedding\_vector\_length=1536$                                                  \\ \hline
\multicolumn{1}{|c|}{\textbf{Agent-OM-Lite}} & llama-3  & $temperature=0.0, top\_k=1, repeat\_penalty=1.0,embedding\_vector\_length=4096$   \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

Table~\ref{tab: vocabulary-setting} shows the ontology structural terms interpreted for OAEI 2025. We observe that OAEI tracks mainly use OWL (\url{http://www.w3.org/2002/07/owl#})/RDFS (\url{http://www.w3.org/2000/01/rdf-schema#}) and SKOS (\url{http://www.w3.org/2004/02/skos/core#}) for their vocabularies. The syntactic retriever processes class and property names, while the lexical retriever processes descriptive terms, and the semantic retriever processes hierarchical and logical terms.

\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.2}
\tabcolsep=0.15cm
\caption{Ontology structural terms interpreted for OAEI 2025.}
\label{tab: vocabulary-setting}
\begin{adjustbox}{width=1\columnwidth,center}
\begin{tabular}{|c|l|l|}
\hline
\multirow{1}{*}{\textbf{Retriever}}& \multirow{1}{*}{\textbf{OWL/RDFS}}                     & \multirow{1}{*}{\textbf{SKOS}}                \\ \hline
\multirow{2}{*}{\textbf{Syntactic}} & owl:Class, owl:ObjectProperty, owl:DatatypeProperty   & skos:Concept                                  \\
                                    & rdfs:label,...                                        & skos:prefLabel, skos:altLabel,...             \\ \hline
\multirow{1}{*}{\textbf{Lexical}}   & rdfs:comment,...                                      & skos:definition, skos:note,...                \\ \hline
\multirow{4}{*}{\textbf{Semantic}}  & rdfs:subClassOf, rdfs:subPropertyOf,...               & skos:broader, skos:narrower, skos:related,... \\
                                    & owl:equivalentClass, owl:equivalentProperty,...       & skos:exactMatch, skos:closeMatch,...          \\ 
                                    & rdfs:domain, rdfs:range,...                           & skos:hasTopConcept, skos:topConceptOf,...     \\
                                    & owl:Restriction, owl:onClass, owl:onProperty,...      &                                               \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

\subsubsection{Performance reporting}

For the confidence of each mapping, Agent-OM provides an approximate range (e.g. $confidence\geq0.90$), but not the exact value (e.g. $confidence=0.97$). This is because Agent-OM applies reciprocal rank fusion (RRF)~\citep{cormack2009reciprocal} on top of the matching results, and the ranking results do not have a statistical link to confidence. We use RRF to overcome two limitations of the traditional approach by computing a mean of syntactic, lexical, and semantic matching results (as illustrated in Figure~\ref{fig: rrf-approach}):

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\arabic*)]
\item The traditional approach cannot determine the best match between very similar entities. For example, entities may have the same mean value despite having different results in syntactic, lexical, and semantic matching (coloured blue in the figure). By computing and accumulating their rankings, the RRF approach is able to distinguish the best match from other close matches.
\item The traditional approach is very sensitive to insufficient input data causing semantic matching to fail. For example, an entity with missing results in semantic matching will obtain a very low mean value (coloured red in the figure). In such cases, the RRF approach is able to minimise the impact of missing values so that the entity with missing values becomes comparable with other entities.
\end{enumerate}

\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{qiang-om-2025-figures/RRF-Approach.png}
\caption{Traditional Approach vs Reciprocal Rank Fusion (RRF) Approach.}
\label{fig: rrf-approach}
\end{figure}

\newpage

Agent-OM is expected to have a longer execution time than traditional OM systems. Agent-OM is built on LLM agents, which are inherently characterised by latency behaviours. Its powerful capability in reasoning is achieved by accumulating historical context and enabling a comprehensive tool-augmented extension. This results in a lengthy context fed into LLMs, as well as increased resource usage in tool calling and memory access~\citep{kim2025cost}. Additionally, for accessing commercial API-accessed models (e.g. gpt-4o and gpt-4o-mini), the execution time is under the control of the API provider and not of the matcher. Guardrails are typically applied to restrict the number of requests per minute (RPM) and tokens per minute (TPM). For example, the OpenAI rate limits given in~\citep{openai-rate-limits}. For accessing open-source models (e.g. llama-3), the execution time depends on the settings of the local machine. On machines equipped with graphics processing units (GPUs), the processing is significantly faster than on machines with only central processing units (CPUs). Agent-OM has multiple create, read, update, and delete functions (CRUD) on its database. The time used in querying and searching is driven by the choice of database implementation.

\subsection{Link to the system alignments}

The system alignments are stored in the folder named OAEI\_2025 at \url{https://github.com/qzc438/ontology-llm/tree/master/campaign/}. For large datasets, the complete results are stored in the folder named OAEI\_2025 at \url{https://github.com/qzc438/ontology-llm-large-datasets/tree/master/campaign/}.

Under each track folder, predict.csv/predict.xml corresponds to our system alignment, whereas true.csv corresponds to the reference alignment. The confidence for each mapping in predict.csv/predict.xml is greater than or equal to 0.90, produced by the setting of $similarity\_threshold=0.90$. Note that we do not include the element <measure> in our alignment file, while the evaluation conducted in the Matching EvaLuation Toolkit (MELT)~\citep{hertling2019melt} will add \verb|<|measure rdf:datatype=``xsd:float''\verb|>|1.0\verb|<|/measure\verb|>| in this case. The result.csv file reports the measures of precision, recall, and F1 score. Some rows present intermediate partial results, but rows ending with ``llm\_with\_agent'' in the ``Alignment''column present the final matching results. The execution time is not reported due to variations in the API provider (for commercial API-accessed LLMs) and computational power (for open-source LLMs). It follows a linear growth with the number of entities if no additional optimisations are applied, such as those in section~\ref{sub-sec: improvement}. The cost.csv file reports the API charge for API-accessed LLMs. Open-source LLMs are used free-of-charge.

\section{Results}

Table~\ref{tab: agent-om-participation} shows Agent-OM participation in the OAEI 2025 TBox/schema matching tracks. Agent-OM focuses on one-to-one equivalence mapping in the TBox/schema matching tasks. The current system has limited support for instance matching and link discovery. We do not participate in the TBox/schema matching tracks that contain interactive matching and complex matching types or relations.

\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.2}
\tabcolsep=0.15cm
\caption{Agent-OM in the OAEI 2025 TBox/schema matching tracks.}
\label{tab: agent-om-participation}
\begin{adjustbox}{width=1\columnwidth,center}
\begin{tabular}{|c|l|l|l|c|}
\hline
\multirow{1}{*}{\textbf{Track Name}} & \multirow{1}{*}{\textbf{Track Domain}}
& \multirow{1}{*}{\textbf{System Variant}} & \multirow{1}{*}{\textbf{Chosen LLM}} & \multirow{1}{*}{\textbf{Evaluation}}    \\ \hline
anatomy         & Human and Mouse Anatomy                   & Agent-OM      & gpt-4o-2024-05-13        & complete           \\ \hline
conference      & Research Conference                       & Agent-OM      & gpt-4o-2024-05-13        & complete           \\ \hline
multifarm       & Conference Extension on Multilingualism   & Agent-OM      & gpt-4o-mini-2024-07-18   & -                  \\ \hline
bio-ml          & Biomedical                                & Agent-OM-Lite & llama-3-8b               & partial            \\ \hline
biodiv          & Biodiversity and Ecology                  & Agent-OM-Lite & llama-3-8b               & -                  \\ \hline
dh              & Digital Humanities                        & Agent-OM      & gpt-4o-2024-05-13        & complete           \\ \hline
arch-multiling  & Archaeology Multiling                     & Agent-OM      & gpt-4o-2024-05-13        & complete           \\ \hline
ce              & Circular Economy                          & Agent-OM      & gpt-4o-2024-05-13        & complete           \\ \hline
\multicolumn{5}{c}{Tracks labelled ``-'' were unable to publish Agent-OM results due to platform issues or communication failures.} \\
\end{tabular}
\end{adjustbox}
\end{table}

We refer readers to the official website for the results of Agent-OM in the OAEI 2025 campaign: \url{https://oaei.ontologymatching.org/2025/results/}. Note that the results are produced from a single trial by the authors, and slight differences may occur across multiple runs due to the non-determinism of LLMs. The system variant and chosen LLM are determined by balancing performance and cost efficiency. For small tasks, we use our premium Agent-OM working with the premium gpt-4o-2024-05-13 model, which gives our best results at a high cost. For medium-sized tasks, we use Agent-OM with the inexpensive gpt-4o-mini-2024-07-18 model. For large-scale tasks, we use Agent-OM-Lite with the free-of-charge open-source llama-3-8b model running entirely on our local machine.

Given the rank of some matcher $rank_i$ on track $i$, and the number of participants on that track, our goal is to normalise all reciprocal ranks to a scale of [0, 1], with 1 corresponding to the highest rank and 0 to the lowest. Therefore, the normalised reciprocal rank ($RR^*$) and the overall mean reciprocal rank ($MRR^*$) are defined as:

\begin{equation}
RR^*_i=1-\dfrac{(\text{rank}_i-1)}{(\text{number of participants}_i-1)} \qquad MRR^*=\frac{1}{N} \sum_{i=1}^{N} RR^*_i
\end{equation}

Figure~\ref{fig: rank} shows Agent-OM's normalised $RR^*$ per track and overall $MRR^*$ on the tracks shown as ``complete'' in Table~\ref{tab: agent-om-participation}. We can see no pattern in Agent-OM's precision vs recall performance ranking running across the tracks, although this may reflect track-wise precision-recall variability in other matchers. The conference and dh tracks have a notable gap between rankings in precision and recall, suggesting room for improvement. Regarding $MRR^*$, we observe that Agent-OM's precision and F1 score are very similar, suggesting that Agent-OM could be more competitive by prioritising improvements of recall over precision.

\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{qiang-om-2025-figures/campaign-rank-2025.png}
\caption{Agent-OM's normalised reciprocal rank ($RR^*$) per track and overall mean reciprocal rank ($MRR^*$).}
\label{fig: rank}
\end{figure}

\section{General Comments and Conclusions}

\subsection{Comments on the results}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\arabic*)]

\item We apply Agent-OM to three previously evaluated tracks (anatomy, conference, and mse) in~\citep{qiang2023agent} and two new tracks (dh and ce). While the mse track is not participating in the 2025 campaign, we provide our results for this track on GitHub for reference. The results indicate that Agent-OM is resilient in performing tasks from diverse domains with varying levels of complexity and ontology structural terms used. Although performance by traditional systems on simple tasks remains comparable, we believe that Agent-OM is paving the way for shifting to general-purpose domain-independent OM systems.

\item We apply Agent-OM to two multilingual tracks (multifarm and arch-multiling). We find that matching ontologies expressed in the same language is more successful than matching different languages, although having English as one of the pair of different languages is clearly advantageous. Further, matches between ontologies using languages from the same language family (e.g. English matched with European languages) are better than those between different language families. In some cases, these patterns do not apply to the Chinese language. This may be fundamentally due to the high-tech dominance of the English language, so LLMs are commonly trained in English. English has incorporated many aspects of European languages (Germanic, French, and Latin) as well as vocabulary from other global languages. Chinese uses a different tokenisation to English, but most LLMs are able to deal with Chinese, perhaps due to plentiful Chinese training data.

\item We apply Agent-OM-Lite to two biomedical tracks (bio-ml and biodiv). We find that the computation time for these two tracks is significantly longer than for other tracks. This is because the ontologies used in these tracks are large ontologies and Agent-OM always captures syntactic, lexical, and semantic information for each ontology entity. In general, it is a useful practice because it addresses two common matching scenarios: the same concept with different names and different concepts with the same name. However, in some tasks in the biomedical domain, it is rare for different concepts to have the same name, for example, ncit-doid in bio-ml and fish-zooplankton in biodiv. Therefore, it could be worthwhile to initially match only by syntactic matching and to assess intermediate results. For those tasks where performance is excellent, matching could stop there. For those tasks with poor performance, proceeding to the much more computationally-demanding LLM-based lexical and semantic steps could be justified. 

\end{enumerate}

\subsection{Discussion on ways to improve the proposed system}
\label{sub-sec: improvement}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\arabic*)]

\item Agent-OM can be used for both subsumption matching and one-to-many/many-to-many matching. However, such matches are susceptible to the similarity threshold chosen. When similarity is very high, we could declare three matches (i.e. equivalence, subsumption, and inverse subsumption), but we cannot determine which to use. Although one entity can have multiple closely-matched candidates, it is hard to determine the best similarity threshold as a cut-off point. In some cases, one could look for a ``gap'' in the similarity scores to define the cut-off point, obtaining a different cut-off for each mapping.

\item Agent-OM is currently using bidirectional validation to reduce LLM hallucinations, but it is not efficient when the input data to the OM system is unbalanced. One of the ontologies may be much larger than another. In such settings, the system should select the smaller ontology as the starting point so that validation can be applied to fewer matching candidates.

\item After LLM validation, an extra step of human validation could be useful for precise mappings. Although LLMs can serve as oracles acting as domain experts~\citep{lushnei2025large}, several limitations should be taken into account. For example, the llama-3-8b model may treat ``A is the subclass of B'' and ``B is the subclass of A'' as contradictions, even though these two statements indicate the equivalence of A and B.

\end{enumerate}

In the era of LLMs, we believe that there are two pathways to develop modern LLM-based OM systems. One is to explore the new LLM infrastructure, and the other is the LLM fine-tuning. The former often injects external knowledge from retrieval-augmented generation (RAG)~\citep{lewis2021retrievalaugmented} into the LLMs, while the latter uses training data to update the internal knowledge of the LLMs. A communication module (e.g. LLM agent) is the critical component of the LLM infrastructure, while high-quality data is the key to finding the ``Aha! moment'' for LLM fine-tuning. Recent research focusing on LLM infrastructure includes~\citep{qiang2023agent,hertling2023olala,giglou2024llms4om,zhang2024large,taboada2025ontology,nguyen2025kroma}, while LLM fine-tuning is addressed in~\citep{qiang2024oaei,he2024language,sousa2025complex,yang2025language}.

\subsection{Comments on the OAEI test cases}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\arabic*)]
\item The namespaces in reference.xml are mixed with ``\url{http://knowledgeweb.semanticweb.org/heterogeneity/alignment\#}'' (with \#) and ``\url{http://knowledgeweb.semanticweb.org/heterogeneity/alignment}'' (without \#). A script has been provided to normalise the inconsistent use of namespaces according to the Alignment API format~\citep{edoal2011}.
\item The ontologies used in the OAEI campaign require a cleaning procedure. Some information irrelevant to the OM task needs to be removed, for example, the metadata of the entity (creator and date/time), which is not relevant to the entity's meaning. Including this metadata can confuse the similarity assessment.
\item A complete reference is the key to ensuring a fair comparison. We identify two primary reasons for the low performance in certain tracks. a) Some reference alignments have missing mappings. We suggest using LLMs as a tool to validate existing correspondences or to discover missing mappings~\citep{qiang2024does}. b) Some ontologies have some entities with properties (e.g. skos:related) that refer to external resources with naming conventions using codes. In this case, the name carries no natural language meaning and may be confusing to LLMs. We suggest removing these references to external ontologies. Alternatively, we could extend Agent-OM to retrieve external ontologies and use them in our matching process.
\item For machine learning and LLM fine-tuning for OM, data sampling for the training set needs to be diverse with respect to concepts so that LLMs can learn the domain knowledge. For example, if the alignment includes food nutrition, then the training data is expected to include food nutrition concepts. Several examples of data sampling for OM can be found in~\citep{hertling2024oaei}.
\end{enumerate}

\subsection{Comments on the OAEI measures}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\arabic*)]
\item The output formats for OM systems vary. OAEI only accepts the Alignment API format. There is a need to develop a unified pipeline to convert different formats to the Alignment API format.
\item LLMs are non-deterministic by nature. An update to the current platform may be required to ensure that LLMs are employed in a uniform setting. We suggest introducing a stream ``LLM Arena for OM'', in which all systems are expected to use the same LLM and hyperparameter settings for the campaign.
\end{enumerate}

\paragraph*{Publication Statement}

Most of the work presented in this chapter has been published as~\bibentry{qiang2025oaei}.

==> qiang-anu-thesis-appendices/oaei-llm.tex <==
\chapter[OAEI-LLM: A Benchmark Dataset for Ontology Matching]{OAEI-LLM: A Benchmark Dataset for Understanding Large Language Model Hallucinations in Ontology Matching}
\label{appendix: oaei-llm}

This appendix demonstrates how Agent-OM can be used to develop a benchmark dataset to evaluate the hallucinations of large language models (LLMs) in ontology matching (OM) tasks.

LLM hallucinations commonly occur in domain-specific downstream tasks, with no exception in OM. The prevalence of using LLMs for OM raises the need for benchmarks to better understand LLM hallucinations. The OAEI-LLM dataset is an extended version of the Ontology Alignment Evaluation Initiative (OAEI)~\citep{oaei} datasets that evaluate LLM-specific hallucinations in OM tasks. We outline the methodology used in dataset construction and schema extension, and provide examples of potential use cases.

LLMs have shown incredible capabilities in natural language generation (NLG) and question answering (QA). In the Semantic Web community, LLMs have recently been used in OM. Although LLMs offer a strong background knowledge base for OM, they may miss some true mappings and generate a number of false mappings. This phenomenon has been observed in several recent papers in~\citep{he2023exploring,norouzi2023conversational,hertling2023olala,qiang2023agent,giglou2024llms4om,amini2024towards}. It is mainly caused by LLM hallucinations, where LLMs tend to generate unreliable answers when they do not have sufficient background knowledge or have biased domain knowledge~\citep{zhang2023siren}.

\newpage

The conference track is one of the OAEI campaigns that evaluates OM tasks in conference organisation. It includes several reference alignments between different ontologies related to research conference management~\citep{cheatham2014conference,solimando2014detecting,solimando2017minimizing,zamazal2017ten}. For example, ``\texttt{http://cmt\#Chairman}'' and ``\texttt{http://conference\#Chair}'' form a pair of valid match in the CMT-Conference alignment. LLMs can experience hallucinations when they mistakenly categorise a pair of matched entities to be unmatched entities. This often happens because it is very difficult for LLMs to understand polysemous words, such as where the word ``chair'' refers to the person who chairs the conference, and not to the furniture used at the conference. LLM hallucinations can also occur when one of the matched entities is mismatched with other entities. For example, LLMs may consider ``chair'' in the context of a research conference to have a similar meaning to ``conference chair''. Therefore, ``\texttt{http://conference\#Chair}'' can be mismatched to ``\texttt{http://cmt\#ConferenceChair}''. Both the former case of missing true mappings and the latter case of generating false mappings will have a negative impact on the matching performance. It seems feasible to mitigate LLM hallucinations using fine-tuning, but there are few datasets that can be used to provide baseline references.

Established in 2004, OAEI has become the largest community of specified ontology matching challenges. Over the years, OAEI has developed several multi-ontology tracks across a wide range of topic domains. We observe that no tracks have covered the topic of LLM hallucinations in OM tasks. For this reason, we propose to extend the current OAEI datasets to construct a new dataset called OAEI-LLM, which serves to measure the degree of hallucination by LLMs in OM tasks. The new dataset compares the original human-labelled results with LLM-generated results, classifies different types of hallucinations made by different LLMs, and records the information with a new schema extension. We believe this dataset would benefit research in understanding LLM hallucinations in matching tasks and thereby research in improving LLM-driven OM.

\section{Methodology}

\subsection{Dataset Construction}

\autoref{fig: methodology-oaei} illustrates the procedure for constructing the dataset. The original OAEI datasets provide three files: the source ontology ($O_s$), the target ontology ($O_t$), and their OAEI Reference ($R_{oaei}$). We implement an LLM-based OM system to generate the alignment file LLM Alignment ($A_{llm}$). The system takes $O_s$ and $O_t$ as inputs and generates a set of predicted mappings. We constrain our mappings to the case of only one-to-one mappings, that is, every entity in the source ontology is mapped to at most one entity in the target, and each entity in the target ontology occurs in at most one mapping. The matching assessment procedure detailed below will compare $R_{oaei}$ with $A_{llm}$ and find their differences.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.6\linewidth]{qiang-iswc-2024-figures/Methodology.png}
\caption{Procedure for constructing the dataset.}
\caption*{An LLM Alignment of the source and target ontologies is compared with the OAEI Reference and recorded in the OAEI-LLM Benchmark.}
\label{fig: methodology-oaei}
\end{figure}

For each mapping $(e1,e2)\in R_{oaei}$, we consider that it is not an LLM hallucination if there exists $(e1', e2') \in A_{llm}$ such that $e1 = e1'$ and $e2 = e2'$. We categorise LLM mapping errors in three ways, as shown in Table~\ref{tab: types}.

\begin{table}[htbp]
\caption{Different types of LLM mapping errors.}
\label{tab: types}
\begin{tabularx}{\textwidth}{lX}
\toprule
Type & Definition\\
\midrule
\textbf{Missing from LLM} & For a specific pair $(e1,e2) \in R_{oaei}$, there is no pair $(e1',e2') \in A_{llm}$ that satisfies $(e1 = e1')$ exclusive-or $(e2 = e2')$. \\
\textbf{Missing from OAEI} & For a specific pair $(e1',e2') \in A_{llm}$,  there is no pair $(e1,e2) \in R_{oaei}$ that satisfies $(e1 = e1')$ exclusive-or $(e2 = e2')$.\\
\textbf{Incorrect} & For a specific pair $(e1,e2) \in R_{oaei}$, there exists a pair $(e1',e2') \in  A_{llm}$ that either satisfies $e1 = e1'$ and $e2 \neq e2'$ or satisfies $e1 \neq e1'$ and $e2 = e2'$.\\
\bottomrule
\end{tabularx}
\end{table}

\newpage

The matching assessment process identifies the alignment from which a missing mapping is missing. It also determines a categorisation of incorrect mappings as follows:

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item False-mapping: LLMs map the entity to an irrelevant entity.
\item Disputed-mapping: LLMs map the entity to a relevant entity, but it does not align with the OAEI Reference. We call this mapping type ``disputed'' because we cannot guarantee the OAEI Reference is always correct. LLMs may discover a more precise matching entity.
\item Align-up: LLMs map the entity to its intended superclass.
\item Align-down: LLMs map the entity into its intended subclass.
\end{itemize}

In practice, the notions of \emph{relevant} and \emph{intended} are implemented by the chosen matching assessment process. We use an LLM-based evaluator for matching assessment, and directly query the LLM for relevance and superclass and subclass relationships. At this time we cannot recommend a particular LLM to be used.

\subsection{Schema Extension}

The OAEI tracks use a general alignment format derived from the Expressive and Declarative Ontology Alignment Language (EDOAL)~\citep{edoal2011}. An example to represent a valid match of ``\texttt{http://cmt\#Chairman}'' and ``\texttt{http://conference\#Chair}'' is illustrated as follows: Each mapping is recorded in a tag \textit{<Cell>}. The schema uses the tags \textit{<entity1>} and \textit{<entity2>} to record the pair of entities, the tag \textit{<measure>} to present their similarity, and the tag \textit{<relation>} to indicate their relations.

We extend the current EDOAL mapping schema to record the new information related to LLM hallucinations. The Simple Standard for Sharing Ontological Mappings (SSSOM)~\citep{matentzoglu2022simple} could be an alternative base to extend for our purpose. Code Snippet~\ref{lst: example} illustrates an example of an OAEI-LLM reference alignment using our proposed extended EDOAL mapping schema. For each mapping, different types of hallucinations can occur in different LLMs. Each of them is recorded in the tag \textit{<hallucination>}. In the extended version of the example (shown in blue, green, and purple), the first segment depicts the LLM hallucinations that occurred in claude-3-sonnet~\citep{llm-claude-3-sonnet}, which is a case of a mapping missing from the LLM. The second segment illustrates the LLM hallucinations that occurred in llama-3-8b~\citep{llm-llama-3-8b}, indicating an incorrect mapping to the entity ``\texttt{http://cmt\#ConferenceChair}''. The matching assessment classifies this mapping as a ``disputed mapping''.

\begin{lstlisting}[label=lst: example, basicstyle=\ttfamily\small, language=XML, caption={An example of an OAEI-LLM reference alignment using our proposed extended EDOAL mapping schema. Text generated by Agent-OM is shown in green. Text generated by LLM-based evaluator is shown in purple.}]
<map>
    <Cell>
        <entity1 rdf:resource="http://cmt#Chairman"/>
        <entity2 rdf:resource="http://conference#Chair"/>
        <measure rdf:datatype="xsd:float">1.0</measure>
        <relation>=</relation>
        (*@\textcolor{blue}{<hallucination>}@*)
            (*@\textcolor{blue}{<llm>claude-3-sonnet</llm>}@*)
            (*@\textcolor{blue}{<category>}\textcolor{teal}{missing}\textcolor{blue}{</category>}@*)
            (*@\textcolor{blue}{<source>}\textcolor{teal}{llm}\textcolor{blue}{</source>}@*)
        (*@\textcolor{blue}{</hallucination>}@*)
        (*@\textcolor{blue}{<hallucination>}@*)
            (*@\textcolor{blue}{<llm>llama-3-8b</llm>}@*)
            (*@\textcolor{blue}{<category>\textcolor{teal}{incorrect}</category>}@*)
            (*@\textcolor{blue}{<entity1 rdf:resource=\textcolor{teal}{"http://cmt\#ConferenceChair"}/>}@*)
            (*@\textcolor{blue}{<type>\textcolor{violet}{disputed mapping}</type>}@*)
        (*@\textcolor{blue}{</hallucination>}@*)
    </Cell>
</map>
\end{lstlisting}

\section{Potential Use Cases}

\subsection{Benchmarking LLMs for OM Tasks}

Different LLMs can perform differently on the same OM task. However, running an LLM-based matcher on a traditional OAEI dataset can only observe the differences in precision, recall, and F1 score. Using the extended version of OAEI-LLM, we can additionally quantify the LLM errors made by counting each of the different types of errors we have identified. Therefore, it becomes possible to understand the tendency of LLMs to generate incorrect answers or to provide relevant but not precise answers. This could also be a valuable supplement to enhance an LLM leaderboard for OM tasks. Indeed, this same additional information on matching failures could also be helpful if adopted more widely by non-LLM ontology matchers.

\subsection{A Dataset for Fine-tuning LLMs Used in OM Tasks}

Fine-tuning is a common approach used in LLMs to inject domain knowledge, but a significant amount of data typically needs to be provided. Unlike the traditional OAEI datasets, which only provide information on matched entities, OAEI-LLM provides extensive information identifying when and how LLM hallucinations occur, and even the mismatched entities caused by LLM hallucinations. This could be used to generate high-quality training data to fine-tune LLMs.

\section{Limitations}

In this study, we only demonstrate the simplest one-to-one equivalent mappings. More generally, the reference alignment can be incomplete or contain one-to-many mappings, while the matching type can also go beyond equivalence to include subsumption matching and complex matching. Such sophisticated cases may cause additional types of LLM hallucinations. Some LLM hallucinations could be mitigated by providing more ontology structure as context to the LLM, for example, by employing the locality principle of traditional matchers~\citep{jimenez2011logic}. Nevertheless, the proposed benchmark dataset will be useful until LLM-based matchers achieve perfection.

In our work to date we use a moderately simple LLM-based evaluator to perform the matching assessment. The assessment may vary depending on the LLM used. A more sophisticated matching assessment could use a voting process by multiple LLMs or human expert judgement to generate a more reliable OAEI-LLM benchmark dataset.

\section{Further Work}

The OAEI tracks can be divided into three categories: schema matching (i.e. TBox matching), instance matching (i.e. ABox matching), and interactive matching (i.e. matching that involves user interaction). Correspondingly, OAEI-LLM will also have three variants.

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item OAEI-LLM-T will focus on comprehending LLM hallucinations in the TBox, with a specific interest in the formal use of terminologies in ontology design and implementation.
\item OAEI-LLM-A will focus on addressing LLM hallucinations in the ABox, in which an ontology contains a schema together with many instance entities (similar to ontology-based knowledge graphs).
\item OAEI-LLM-I will focus on understanding how user interaction could be used to mitigate LLM hallucinations and estimating the level of user interaction required for LLM-based OM tasks.
\end{itemize}

\paragraph*{Publication Statement}

Most of the work presented in this chapter has been published as~\bibentry{qiang2024oaei}.

==> qiang-anu-thesis-content/agent-om.tex <==
\chapter{Agent-OM: Leveraging LLM Agents for Ontology Matching}
\label{chap: agent-om}

Ontology matching (OM) enables semantic interoperability between different ontologies and resolves their conceptual heterogeneity by aligning related entities. OM systems currently have two prevailing design paradigms: conventional knowledge-based expert systems and newer machine learning-based predictive systems. While large language models (LLMs) and LLM agents have revolutionised data engineering and have been applied creatively in many domains, their potential for OM remains underexplored. This study introduces a novel agent-powered LLM-based design paradigm for OM systems. With consideration of several specific challenges in leveraging LLM agents for OM, we propose a generic framework, namely Agent-OM (Agent for Ontology Matching), consisting of two agents for retrieval and matching, with a set of OM tools. Our framework is implemented in a proof-of-concept system. Evaluations of three Ontology Alignment Evaluation Initiative (OAEI)~\citep{oaei} tracks over state-of-the-art OM systems show that our system can achieve results very close to the long-standing best performance on simple OM tasks and can significantly improve the performance on complex and few-shot OM tasks.

LLMs are pre-trained with an enormous corpus of common knowledge and therefore have powerful generative capabilities. Despite the success of using LLMs in a wide range of applications, leveraging LLMs for downstream tasks still has several challenges. (1) LLMs are pre-trained models that do not capture late-breaking information. (2) LLM hallucinations are often observed in domain-specific tasks and hamper their reliability. LLMs often generate unsound responses that are syntactically sound but factually incorrect~\citep{ji2023survey}. (3) LLMs are good models of linguistic competence, but have shown limited capabilities in non-linguistic tasks, such as planning and routing. LLMs were originally designed for sequential question answering (QA), but most real-world tasks are designed with complex logic and do not follow a straightforward single path~\citep{valmeekam2023large}.

To overcome the limitations of LLM customisation for downstream tasks, LLM-based autonomous agents have become a prominent research area. In the field of artificial intelligence (AI), the notion of agents was first introduced in the famous Turing Test~\citep{turing1950}, referring to intelligent computational entities that can display human-like behaviours. Such AI agents have fallen short of human-level capabilities, as they can only act on simple and heuristic policy functions learnt from constrained environments and they lack efficient central control to simulate the human learning process~\citep{wang2023survey}. LLMs, with remarkable success in demonstrating autonomy, reactivity, pro-activeness, and social ability, have attracted growing research efforts aiming to construct AI agents, so-called LLM agents~\citep{xi2023rise}.

The core concept of LLM agents is to employ the LLM as a controller rather than as a predictive model only (a.k.a. Model as a Service). LLM agents extend LLM capabilities with advanced planning, memory, and pluggable tools, and allow LLMs to communicate with open-world knowledge~\citep{llm-agent}. (1) Planning breaks down a complex task into simpler and more manageable subtasks. LLMs can also receive feedback on plans and perform reflection and refinement. The most practical technique used for LLM planning is chain-of-thought (CoT)~\citep{wei2023chainofthought}. (2) Tools allow LLMs to call external resources for additional information. They are often invoked by LLM agent actions. (3) Memory provides context to inherently stateless LLMs, including short-term memory and long-term memory. Short-term memory can be considered as context information obtained from planning and tools via in-context learning (ICL)~\citep{brown2020language}. Long-term memory often uses database storage with retrieval-augmented generation (RAG)~\citep{lewis2021retrievalaugmented} to retain information. Unlike fine-tuning, where models need to be retrained to learn new context data, ICL/RAG instead augments the LLM prompts with new information. ICL/RAG is more scalable for working with dynamic information. Almost 90\% of use cases can be achieved by ICL/RAG-based search and retrieval~\citep{gptrag}. A recent paper~\citep{ovadia2023finetuning} demonstrates that RAG surpasses fine-tuning across a diversity of knowledge-intensive tasks.

There are two dominant design paradigms for OM systems: traditional knowledge-based OM systems that implement pre-defined logic and expert knowledge; and more recent learning-based OM systems that transform the matching task into machine-enhanced learning and prediction. The former expert systems require extensive expert knowledge, while the latter predictive systems need extensive high-quality data to train the model. The prevalence of LLMs and LLM agents has driven many successful domain-specific applications. However, in the context of OM, using LLMs and LLM agents is currently under-explored. Leveraging LLMs and LLM agents for OM tasks is not an intuitive task; the challenges will be presented in the Related Work section.

This study introduces a novel agent-powered LLM-based design paradigm for OM systems. We propose a generic framework and implement it with a proof-of-concept system. The system extends LLM capabilities beyond general QA, offering a powerful problem solver for OM tasks. The system includes tools that facilitate information retrieval, entity matching, and memory storage. The system is compared to state-of-the-art OM systems, achieving considerable matching performance improvements across three OAEI tracks. Specifically, this study makes the following contributions:

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]

\item We introduce a new agent-powered LLM-based design paradigm for OM systems and propose a novel Agent-OM framework. It consists of the following key components:
\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item A LLM acts as a central ``controller'' to link different modules and instruct their functions via prompt engineering;
\item A pair of planning modules use CoT for OM decomposition;
\item A set of OM tools use ICL/RAG to mitigate LLM hallucinations;
\item A shared memory module uses dialogue and hybrid data storage to support the search and retrieval of entity mappings.
\end{itemize}

\item We implement our proposed Agent-OM framework in a proof-of-concept system. The system deals with several critical downstream challenges in leveraging LLM agents for OM, such as cost-effective entity information retrieval, matching candidate selection, and search-based matching functions.

\item The experimental results of the system show that Agent-OM achieves results very close to the best long-standing performance on simple OM tasks and significantly improves matching performance on complex and few-shot OM tasks.

\end{itemize}

An ontology contains classes, properties, and individuals. In this study, we consider only classes and properties, and individuals are excluded. Possible logical relations between classes (respectively properties) can be equivalence ($\equiv$) and subsumption (either $\subseteq or \supseteq$). In this study, we only consider the logical relation of equivalence ($\equiv$) between classes and properties.

\section{Related Work}

OM is typically a non-trivial but essential alignment task for data integration, information sharing, and knowledge discovery~\citep{shvaiko2011ontology}. While matching is a prerequisite for interoperating applications with heterogeneous ontologies, OM systems are designed to automate the matching process. The conventional approach using knowledge-based OM systems, such as LogMap~\citep{jimenez2011logmap1,jimenez2011logmap2}, AgreementMakerLight (AML)~\citep{faria2013agreementmakerlight,faria2014agreementmakerlight}, and FCA-Map~\citep{zhao2018matching,li2021combining} has been shown to be precise and effective. However, it is resource-hungry and labour-intensive. It is often difficult to find domain experts to evaluate the matches, and any group of experts may not be able to cover all domain concepts that an expert system requires. A new approach uses machine learning (ML), implemented in systems such as BERTMap~\citep{he2022bertmap} and LogMap extension LogMap-ML~\citep{chen2021augmenting}. ML-based OM systems employ the concept of training and testing in ML, using ontology entities as features for model training or fine-tuning and then using the model to predict additional correspondences. Specifically, the leading system BERTMap uses a common language model originating from natural language processing (NLP) (i.e. BERT~\citep{devlin2019bert}).

Although ML-based approaches have shown a significant improvement in matching performance, their training-testing paradigm is not feasible for LLMs. The number of parameters used in LLMs is much larger than those of common language models. This means retraining the entire LLM is usually infeasible, and fine-tuning such a large model requires a number of samples that may be infeasibly large for OM. A survey in~\citep{zong2022survey} implies that 1000 is a reasonable number of training samples to fine-tune GPT-3~\citep{brown2020language}, but generally speaking, a domain ontology has only around 100-200 entities. Furthermore, currently some LLMs are only accessible through a web service. This means that training or fine-tuning LLMs risks leaking sensitive information, while synthetic data, on the other hand, makes it difficult to ensure training quality.

Early studies using LLMs for OM can be found in~\citep {he2023exploring} and~\citep{norouzi2023conversational}. Both works use a purely prompt-based approach. The prompts are structured as a binary question: given an entity from the source ontology and an entity from the target ontology, the LLMs perform a classification task to determine whether these two entities are identical or not. A similar approach is also used in OLaLa~\citep{hertling2023olala} and LLMs4OM~\citep{giglou2024llms4om}, but their candidate generation is integrated with the embedding extractor models.~\cite{amini2024towards} explore the potential of using LLMs for complex ontology OM challenges.

LLM agents were introduced in AutoGPT~\citep{autogpt} and BabyAGI~\citep{babyagi}. The recent release of OpenAI GPTs~\citep{gpts}, Microsoft Copilot~\citep{copilot}, and Copilot Studio~\citep{copilotstudio} has sparked interest in LLM agents. Building applications with LLM agents allows users to build their own custom GPTs to support custom business scenarios. In ontology-related tasks, LLM-driven agents have shown impressive performance in automating manual activities in the broader task of ontology engineering. These works pay attention to the use of conversational dialogue to enhance the agent's capabilities with human feedback. While this is suitable for tasks that require humans to be in the loop, such as collecting competency questions in ontology engineering~\citep{zhang2024ontochat} or validating extended terms in ontology learning~\citep{giglou2023llms4ol}, modern OM seeks to automate a complex task with minimal human intervention. Contrasting with these works, our aim is to design a new infrastructure that is able to instruct LLM agents to use planning to decompose a complex task into steps and to use tools to facilitate automated matching (a.k.a. function calling), instead of purely using agent-based conversational dialogue, even when specialised as ontology-oriented dialogue like~\citep{payne2014negotiating,zhang2024large}.

We introduce our novel agent-powered LLM-based design paradigm for OM systems. We have two generic agents; each one is self-contained and designed to instruct LLMs to use extensive planning, memory, and tools, thus unlocking their generative capabilities to handle various types of OM tasks in different contexts. Meanwhile, as a key enabler for precise decision-making, we also limit the current LLM's flaws in hallucination, context understanding, and non-linguistic reasoning. Several OM-related tools have been created for this purpose. These tools enable LLM agents to simulate a traditional OM system, automating the entire matching process without human intervention. The overall infrastructure offers high scalability and allows extensive customisation. To the best of our knowledge, this study is the first to introduce an LLM-agent-based framework for OM tasks.

\section{Methodology}
\label{sec: approach}

Given a source ontology ($O_s$) and a target ontology ($O_t$), OM aims to find an alignment (A) that contains a set of pair-matched entities $\{(e_i, e_j) \mid e_i \in O_s, e_j \in O_t\}$. A classical matching process has two main steps: retrieval and matching. The retrieval step involves retrieving internal information from the ontology itself ($R_{int}$) and external information from a domain-specific thesaurus ($R_{ext}$). The matching step involves selecting the matching candidates ($M_{sel}$), running the matching algorithms ($M_{alg}$), and refining the matching results ($M_{ref}$). A classical OM can be formulated as:

\begin{equation}
R_{int} \Rightarrow R_{ext} \Rightarrow M_{sel} \Rightarrow M_{alg} \Rightarrow M_{ref}
\end{equation}

Figure~\ref{fig: architecture} shows the architecture of \emph{Agent-OM}, our agent-powered LLM-based OM framework. It retains the original input and output of the classical OM but modularises the two main steps with autonomous LLM agents, namely Retrieval Agent ($Agent\_{R}$) and Matching Agent ($Agent\_{M}$). These two LLM agents have their own planning modules and related tools but share memory. The memory is responsible for storing the information retrieved from the Retrieval Agent ($R_{sto}$) and facilitating the search of the stored information by the Matching Agent ($M_{sea}$). Therefore, an agent-based OM is formulated as:

\begin{equation}
Agent\_R_{(R_{int} \Rightarrow R_{ext} \Rightarrow R_{sto})} \Rightarrow Agent\_M_{(M_{sea} \Rightarrow M_{sel} \Rightarrow M_{alg} \Rightarrow M_{ref})}
\end{equation}

\begin{figure}[!t]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2025-figures/Methodology.png}
\caption{Architecture of Agent-OM. All components are executed twice, once for each of the source and target ontologies, apart from the matching merger tool that combines the results from each pass.}
\label{fig: architecture}
\end{figure}

For each autonomous agent, the workflow is described as follows. The planning module decomposes a complex task into several subtasks and defines the order of subtasks and tools to be invoked. The plan is stored in the dialogue and passed to the LLMs. LLMs then invoke the tools to perform the subtasks. The tools may communicate with each other, with intermediate results stored in the dialogue. The tools can also access the database via the create, read, update, and delete functions (CRUD) provided. The entire workflow is driven by LLM prompts. We use solid lines to show the actual workflow controlled by the LLMs, and dotted lines to show the implicit link between a subtask and its corresponding tool activated by the LLMs.

\subsection{Retrieval Agent}

The Retrieval Agent is responsible for extracting entities from the ontologies, eliciting their metadata and ontology context information, and storing them in the hybrid database. For each entity extracted from the source and target ontologies, the planning module generates the instruction for retrieving the relevant information and feeding it into the LLMs to invoke the corresponding retrieval tools. The tools used in the Retrieval Agent include Metadata Retriever, Syntactic \& Lexical \& Semantic Retriever, and Hybrid Database Store with Content Embedder, described as follows.

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]

\item Metadata Retriever ($R_{int}$): The metadata retriever collects the metadata of the input entity from the ontology, including its \emph{category} (i.e. either from the \emph{source} ontology or from the \emph{target} ontology) and \emph{type} (i.e. \emph{class} or \emph{property}).

\item Syntactic Retriever ($R_{int}$): The syntactic retriever is responsible for providing a unified text preprocessing result. A common text preprocessing pipeline consists of tokenisation, normalisation, stop words removal, and stemming/lemmatisation~\citep{manning2008introduction}. According to our previous study~\citep{qiang2024does}, only tokenisation and normalisation help both matching completeness and correctness. The other two pipeline methods, stop words removal and stemming/lemmatisation, could cause unwanted false mappings. For this reason, our syntactic retriever considers only tokenisation and normalisation. We select white spaces to separate the words so that the outputs are short sentences that are easier for LLMs to interpret.

\item Lexical Retriever ($R_{int}$ \& $R_{ext}$): We consider three key aspects of the entity's lexical information: the general meaning ($R_{ext}$), the context meaning ($R_{ext}$), and the content meaning ($R_{int}$). In OM tasks, the general meaning is traditionally generated from Wikidata~\citep{vrandevcic2014wikidata} or similar corpus-based knowledge bases (KBs). As LLMs are trained from these KBs, we use the prompt \textit{``What is the meaning of \{entity\_name\}?''} for the same function. However, using only the general meaning is not sufficient. Using the context constraint \textit{``Context: \{context\}''} is effective in domain-specific tasks. Popular GPT-based domain applications, such as LawGPT~\citep{zhou2024lawgpt} and MedicalGPT~\citep{wang2023huatuo}, use similar approaches. Additionally, we also retrieve content information from \texttt{rdfs:label}, \texttt{rdfs:comment}, and other annotation properties, where the ontology creators may add comments or explanations. These are also useful for retrieving the meaning of the entity.

\item Semantic Retriever ($R_{int}$): The entity's semantic information includes its basic triple-based relations and more complex logic-based axioms. In this study, we only consider triple-based relations that can be verbalised into a more natural language-like presentation via a prompt-based verbalisation tool. Such verbalisation tools are not capable of handling complex logic-based axioms. These functions can only be achieved with external packages, such as OWL Verbaliser~\citep{owlverbaliser}, Sydney OWL Syntax~\citep{cregan2007sydney}, and the DeepOnto~\citep{he2023deeponto} verbalisation module~\citep{he2023language}.

\item Hybrid Database Store with Content Embedder ($R_{sto}$): We use a hybrid database system consisting of a traditional relational database and an advanced vector database. Entity metadata, such as the entity's category and type, are stored in the traditional relational database. In contrast, natural language-based content information, such as the entity's syntactic, lexical, and semantic information, is vectorised via a text embedding model and then stored in the vector database to enable similarity search based on relative distance in the vector space. A unique key links these two databases.

\end{itemize}

\subsection{Matching Agent}

The Matching Agent is responsible for finding possible correspondences, ranking and refining the results according to different criteria, and selecting the best matching candidate. For each entity extracted from the ontologies, the planning module generates the instruction for the matching types to be considered and feeds it into the LLMs to invoke the corresponding matching tools. The planning module first selects the source ontology as a starting point, extracting the entities from the ontology. Then, different matchers perform syntactic, lexical, or semantic matching functions to find the best match for the input entity, using a hybrid database search across the relational and vector databases. A predicted mapping is based on a summarised profile measure of syntactic matching, lexical matching, and semantic matching, with matching validation. The same procedure applies to the target ontology as a starting point, and the results of the common matching candidates are combined. The tools used in the Matching Agent include Hybrid Database Search, Metadata Matcher, Syntactic \& Lexical \& Semantic Matcher, Matching Summariser, Matching Validator, and Matching Merger, described as follows.

\begin{itemize}[wide, labelindent=0pt]

\item Hybrid Database Search ($M_{sea}$): The hybrid database search serves as an interface for the database accessible by the Metadata Matcher and Syntactic \& Lexical \& Semantic Matcher.

\item Metadata Matcher ($M_{sel}$): Given an input entity, the metadata matcher collects the category and type of the input entity from the relational database.

\item Syntactic \& Lexical \& Semantic Matcher ($M_{sel}$): Given an input entity, the syntactic \& lexical \& semantic matchers search for similar syntactic/lexical/semantic information respectively in the vector database using cosine similarity, defined for entities $\mathbf{A}$  and $\mathbf{B}$ as:

\begin{equation}
S_C(\mathbf{A}, \mathbf{B})
= \frac{\mathbf{A} \cdot \mathbf{B}}{\|\mathbf{A}\| \|\mathbf{B}\|}
= \frac{\sum_{i=1}^{n} \mathbf{A}_i \mathbf{B}_i}{\sqrt{\sum_{i=1}^{n} \mathbf{A}_i^2} \cdot \sqrt{\sum_{i=1}^{n} \mathbf{B}_i^2}}
\end{equation}

An extended search in the relational database is then used to filter the results based on the entity's metadata.

\item Matching Summariser ($M_{alg}$): We use reciprocal rank fusion (RRF)~\citep{cormack2009reciprocal} to summarise the matching results. Viewing each of the syntactic, lexical, and semantic descriptions as a document, the purpose of reciprocal rank is to accumulate the inverse of the ranks $r$ of documents $d$ over three ranking results from syntactic, lexical, and semantic matching, defined as:

\begin{equation}
\label{eq: rrf}
RRF(d \in D) = \sum_{r\in R} \frac{1}{k + r(d)}
\end{equation}

$k$ is a constant parameter that is conventionally set to 0 as we do here. This ensures that the formula most highly rewards the most highly-ranked entities. In our case, we are evaluating each entity that occurs in the top@k of each of the three rankings (i.e. syntactic matching, lexical matching, and semantic matching), and combining their results as an overall matching summary. Note that the ``k'' in top@k has no relation to the ``k'' in Definition~\ref{eq: rrf} above.

\item Matching Validator ($M_{ref}$): Validation is a critical step in minimising LLM hallucinations, as illustrated in SelfCheckGPT~\citep{manakul2023selfcheckgpt}. We also apply this method to the summarised results. We ask the LLM a binary question \textit{``Question: Is \{entity\_name\} equivalent to \{matching\_entity\_name\}? Context: \{context\} Answer the question within the context. Answer yes or no. Give a short explanation.''} to check whether the predicted entity is equivalent to the input entity in the provided context. For computational efficiency, we iterate the comparison over all the top@k candidates in order of rank and select the highest-ranked match with a "yes" answer for the matching merger.

\item Matching Merger ($M_{ref}$): The matching merger is responsible for combining the results. The first pass focuses on the source ontology to find matches in the target ontology. The second pass focuses on the target ontology to find matches in the source ontology. We select only the correspondences that occur identically on both passes. As an agent-based system, this could be extended to use multi-agent negotiation via the correspondence inclusion dialogue~\citep{payne2014negotiating}.

\end{itemize}

\section{Implementation}
\label{sec: implementation}

We implement our design of the framework in a proof-of-concept system. The components and their implementation are as follows:

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]

\item LLMs: Our system supports a wide range of LLMs, including OpenAI GPT~\citep{llm-gpt}, Anthropic Claude~\citep{llm-claude}, Meta Llama~\citep{llm-llama}, Alibaba Qwen~\citep{llm-qwen}, Google Gemma~\citep{llm-gemma}, and ChatGLM~\citep{glm2024chatglm}. We select 10 models for this study. 4 models are API-accessed commercial LLMs, while the other 6 are open-source LLMs. Table~\ref{tab: llm-version} gives the details. For API-accessed LLMs, we include two models of different sizes for each family of models. For open-source LLMs, we select models with similar sizes (7-9 billion parameters) from different families. They are accessed via the Ollama library~\citep{ollama}.

\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.2}
\tabcolsep=0.15cm
\caption{Details of LLMs used in the study.}
\label{tab: llm-version}
\begin{tabular}{|c|l|c|l|} 
\hline
\multicolumn{1}{|c|}{\textbf{Family}} & \multicolumn{1}{|l|}{\textbf{Model}}& \multicolumn{1}{|c|}{\textbf{Size}}   & \multicolumn{1}{|l|}{\textbf{Version}}    \\ \hline 
\multirow{2}{*}{GPT}                  & gpt-4o                              & N/A       & gpt-4o-2024-05-13                 \\ \cline{2-4}
                                      & gpt-4o-mini                         & N/A       & gpt-4o-mini-2024-07-18            \\ \cline{1-4}
\multirow{2}{*}{Claude}               & claude-3-sonnet                     & N/A       & claude-3-sonnet-20240229          \\ \cline{2-4}
                                      & claude-3-haiku                      & N/A       & claude-3-haiku-20240307           \\ \cline{1-4}
\multirow{2}{*}{Llama}                & llama-3-8b*                         & 4.7 GB    & Ollama Model ID: 365c0bd3c000     \\ \cline{2-4}
                                      & llama-3.1-8b*                       & 4.9 GB    & Ollama Model ID: 46e0c10c039e     \\ \cline{1-4}
\multirow{2}{*}{Qwen}                 & qwen-2-7b*                          & 4.4 GB    & Ollama Model ID: dd314f039b9d     \\ \cline{2-4}
                                      & qwen-2.5-7b*                        & 4.7 GB    & Ollama Model ID: 845dbda0ea48     \\ \cline{1-4}       
\multirow{1}{*}{Gemma}                & gemma-2-9b*                         & 5.4 GB    & Ollama Model ID: ff02c3702f32     \\ \cline{1-4}
\multirow{1}{*}{GLM}                  & glm-4-9b*                           & 5.5 GB    & Ollama Model ID: 5b699761eca5     \\ \hline
\multicolumn{4}{c}{* Open-source LLM (retrieved December 1, 2024).} \\
\end{tabular}
\end{table}

\item Planning: We select the LangChain library~\citep{langchain}. The library provides a wide range of agents. We select the tool calling agent (a.k.a. function calling agent). At the time of writing, the LangChain library only supports this type of agent used with commercial API-accessed LLMs. To extend our framework to open-source LLMs, we employ the similar concept of ``chain'' to simulate the tool calling agent for open-source LLMs.

\item Memory: (1) Short-term memory: We use a conversational dialogue to store the original intermediate output of each operating process, with no map-reduce applied. (2) Long-term memory: We select a hybrid database consisting of a traditional relational database and an advanced vector database. PostgreSQL~\citep{postgresql} supports a standalone integration of the traditional relational database and the extended vector database using pgvector~\citep{pgvector}. We select OpenAI embedding models~\citep{openaiembeddingmodels} for the content embedding in the vector database. Alternatives are Google Vertex AI Embeddings~\citep{vertexaiembeddings} or Sentence-BERT~\citep{reimers2019sentencebert}, but the dimension of the embedding changes between different embedding models.

\item Tools: To demonstrate the flexibility of our framework, we present the usage of prompt-based tools and programming-based tools, as well as the tools that combine a mixture of prompt-based and programming-based tools.

\end{itemize}

\subsection{Ontology Naming Conventions}

Naming conventions for entities fall into two types: the name has a natural language meaning, or the name is a code. In the following, we call them respectively text-type and code-type. We observe that LLMs can perform well with meaningful entity names (e.g. ProgramCommitteeChair and Chair\_PC). Often in larger biomedical ontologies, entities are codes (e.g. MA\_0000270 or NCI\_C33736) and their meaningful descriptions are recorded in their labels or comments. For this type of naming convention, current LLMs tend to generate the wrong synthesised label or comment corresponding to the code. For example, LLMs can mistakenly interpret the codes ``MA\_0000270'' and ``NCI\_C33736'' both to be ``liver'', while the intended meanings of these two codes are ``eyelid tarsus'' and ``Tarsal\_Plate'' respectively.

To handle the variety of ontology naming conventions and to standardise their usage in LLM-based OM, we use a unified naming convention in this study. If the entity is named by a code (i.e. code-type), we use its label or comment instead. For example, we use ``eyelid tarsus'' and ``Tarsal\_Plate'' instead of ``MA\_0000270'' and ``NCI\_C33736'' respectively. In case the two ontologies reuse the same entity name, we assign a prefix to each entity name with its serial number, category, and type. For example, if it were the case that ``ProgramCommitteeChair'' appears in both source and target ontologies, the unique identifier for each entity would be ``023-Source-Class-ProgramCommitteeChair'' and ``042-Target-Class-ProgramCommitteeChair''.

\subsection{Running Example}
\label{sub-sec: running example}

To demonstrate the functioning of our framework, we choose the CMT-ConfOf alignment as a sample alignment. The CMT Ontology is the source ontology and the ConfOf Ontology is the target ontology. Both ontologies contain similar concepts related to conference organisation. The running example aims to find the best matching entity in the target ontology corresponding to the entity ``\texttt{http://cmt\#ProgramCommitteeChair}'' in the source ontology.

\subsubsection{Retrieval Agent}

Table~\ref{tab: retriever} illustrates the tool calling in the Retrieval Agent. For the entity ``\texttt{http://cmt\#ProgramCommitteeChair}'', the agent first calls the Metadata Retriever to find its category and type. Then the Syntactic Retriever is invoked, giving the output \textit{``program committee chair''}. The agent next invokes the Lexical Retriever to generate a detailed description: \textit{``In the context of a conference, `ProgramCommitteeChair' refers to...''.} The Semantic Retriever generates related triple relations, such as \texttt{(ProgramCommitteeChair, rdfs:subClassOf, ProgramCommitteeMember)}. These triples are verbalised using natural language: \textit{``The class `ProgramCommitteeChair' is a subclass of `ProgramCommitteeMember'.''}

\begin{table*}[htbp]
\centering
\footnotesize
\renewcommand\arraystretch{1.2}
\tabcolsep=0.15cm
\caption{Tool calling in the Retrieval Agent.}
\label{tab: retriever}
\begin{adjustbox}{height=0.9\height,center}
\begin{tabular}{p{1.12\linewidth}}
\hline
\textbf{Tool: Metadata Retriever}    \\ \hline
\textbf{Input:} entity\_uri = ``\texttt{http://cmt\#ProgramCommitteeChair}'' \\
\textbf{Extract:}  source\_or\_target = ``Source'', entity\_type = ``Class'' \\ \hline
\hline
\textbf{Tool: Syntactic Retriever}    \\ \hline
\textbf{Input:} entity\_uri = ``\texttt{http://cmt\#ProgramCommitteeChair}''  \\
\textbf{Extract:} entity\_name = ``ProgramCommitteeChair'' from entity\_uri.  \\
\textbf{Method:} tokenise\_and\_normalise(entity\_name)  \\
\textbf{Output:} entity\_syntactic = \textit{``program committee chair''} \\ \hline
\hline
\textbf{Tool: Lexical Retriever}    \\ \hline
\textbf{Input:} entity\_uri = ``\texttt{http://cmt\#ProgramCommitteeChair}'', context = ``conference''  \\
\textbf{Extract:} entity\_name = ``ProgramCommitteeChair'' from entity\_uri.  \\
extra\_information from annotation properties related to entity\_uri. \\
\textbf{Prompt:} \textit{Question: What is the meaning of \{entity\_name\}? Context: \{context\} Extra Information: \{extra\_information\} Answer the question within the context and using the extra information.}  \\
\textbf{Output:} entity\_lexical = \textit{``In the context of a conference, `ProgramCommitteeChair' refers to...''} (AI-generated content)  \\ \hline
\hline
\textbf{Tool: Semantic Retriever}    \\ \hline
\textbf{Input:} entity\_uri = ``\texttt{http://cmt\#ProgramCommitteeChair}'' \\
\textbf{Method:} generate\_subgraph(entity\_uri) \\
\textbf{Output:} entity\_subgraph consists of triples related to entity\_uri. \\
\textbf{Prompt:} Verbalise triples into phrases: \{entity\_subgraph\} \\
\textbf{Output:} entity\_semantic = \textit{``The class `ProgramCommitteeChair' is a subclass of `ProgramCommitteeMember'...''} (AI-generated content)  \\ \hline
\hline
\textbf{Tool: Hybrid Database Store with Content Embedder}    \\ \hline
\textbf{Input:} entity\_uri = ``\texttt{http://cmt\#ProgramCommitteeChair}'', \\
source\_or\_target = ``Source'', entity\_type = ``Class'' \\
\textbf{Extract:} entity\_id = ``023-Source-Class-ProgramCommitteeChair''  \\
\textbf{Query: Create a relational database and store entity's metadata} 
\begin{lstlisting}[language=SQL]
DROP TABLE IF EXISTS ontology_matching CASCADE;
CREATE TABLE ontology_matching (entity_id VARCHAR(1024) PRIMARY KEY, 
entity_uri TEXT, source_or_target TEXT, entity_type TEXT);
INSERT INTO ontology_matching (entity_id, entity_uri, source_or_target, entity_type)
VALUES ({entity_id}, {entity_uri}, {source_or_target}, {entity_type});
\end{lstlisting}
\textbf{Input}: entity\_syntactic = \textit{``program committee chair''}, \\
entity\_lexical = \textit{``In the context of a conference, `ProgramCommitteeChair' refers to...''},    \\
entity\_semantic = \textit{``The class `ProgramCommitteeChair' is a subclass of `ProgramCommitteeMember'...''},  \\
matching\_table = "syntactic\_matching/lexical\_matching/semantic\_matching"   \\
\textbf{Extract}: content\_embedding based on entity\_syntactic/entity\_lexical/entity\_semantic.  \\
\textbf{Query: Create a vector database and store entity's syntactic, lexical, and semantic information}
\begin{lstlisting}[language=SQL]
CREATE EXTENSION IF NOT EXISTS vector;
DROP TABLE IF EXISTS {matching_table};
CREATE TABLE {matching_table} 
(entity_id VARCHAR(1024) NOT NULL REFERENCES ontology_matching(entity_id), 
content TEXT, embedding vector(1536));
INSERT INTO {matching_table} (entity_id, content, embedding)
VALUES ({entity_id}, 
{entity_syntactic}/{entity_lexical}/{entity_semantic}, {content_embedding});
\end{lstlisting}
\textbf{Output:} One relational database table (ontology\_matching) and three vector database tables (syntactic\_matching, lexical\_matching, and semantic\_matching). \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}

While each entity has its own syntactic, lexical, and semantic information, a naive approach to deciding if two entities are the same is to generate a binary question for every pair of entities as a prompt to the LLM: \textit{``Is Entity1 equivalent to Entity2? Consider the following: The syntactic information of Entity1 is... The lexical information of Entity1 is... The semantic information of Entity1 is... The syntactic information of Entity2 is... The lexical information of Entity2 is... The semantic information of Entity2 is... ''} This approach has two limitations.  (1) The binary comparison is costly because the complexity of the comparison is the product of the number of entities in the source ontology and the target ontology. (2) LLMs have token limits that restrict the number of tokens processed for each interaction. Combining all the retrieved information may exceed token limits.

We bypass these limitations by (1) using an open question instead and (2) storing useful information in a searchable database. Figure~\ref{fig: database} shows the entity metadata and content information stored in the relational database and the vector database, respectively. On one hand, the entity's metadata is needed to find an exact match. For example, ``\texttt{http://cmt\#ProgramCommitteeChair}'' is a class in the source ontology, so the matched entity would ideally be a class in the target ontology. On the other hand, content information including an entity's syntactic, lexical, and semantic information is obtained from a similarity-based match because they are usually retrieved as natural language, which can be more ambiguous than metadata. Similarity between natural language terms is commonly based on embedding vectors,  for which the vector database enables fast similarity searches.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.65\linewidth]{qiang-vldb-2025-figures/Database.png}
\caption{Storing ``\texttt{http://cmt\#ProgramCommitteeChair}'' in the database.}
\label{fig: database}
\end{figure}

\subsubsection{Matching Agent}

Table~\ref{tab: matcher} demonstrates the tool calling in the Matching Agent. Given ``\texttt{http://cmt\#ProgramCommitteeChair}'' from the source ontology, the matching entities found by each matcher are stored in the LLM dialogue and combined using the RRF function. The result of the Matching Summariser is a list of predicted mappings. The next step is to refine the predicted mappings. The Matching Validator asks a binary question to compare whether the given entity is the same or different to the predicted matching entity in RRF-descending order. Because the validator receives a ``yes" answer for the first iteration of the entity ``\texttt{http://confOf\#Chair\_PC}'', the Matching Agent outputs ``\texttt{http://confOf\#Chair\_PC}'' as the best matching entity found in the target ontology. The Matching Merger combines the results from the same procedure applied in the search from ``\texttt{http://confOf\#Chair\_PC}'' in the target ontology. These two terms are considered as matched entities only if the mapping can be found bidirectionally (i.e. ``\texttt{http://cmt\#ProgramCommitteeChair}'' is also found to be the best matching entity in the source ontology for the search from ``\texttt{http://confOf\#Chair\_PC}'' in the target ontology).

\begin{table*}[htbp]
\centering
\footnotesize
\renewcommand\arraystretch{1.2}
\tabcolsep=0.15cm
\caption{Tool calling in the Matching Agent.}
\label{tab: matcher}
\begin{adjustbox}{height=0.9\height,center}
\begin{tabular}{p{1.12\linewidth}}
\hline
\textbf{Tool: Hybrid Database Search with Metadata Matcher}    \\ \hline
\textbf{Input:} entity\_uri = ``\texttt{http://cmt\#ProgramCommitteeChair}'', source\_or\_target = ``Source''\\
matching\_table = ``syntactic\_matching/lexical\_matching/semantic\_matching'' \\
\textbf{Query: Find entity id} 
\begin{lstlisting}[language=SQL]
SELECT o.entity_id FROM ontology_matching o
WHERE o.entity_uri = {entity_uri} and o.source_or_target = {source_or_target};
\end{lstlisting}
\textbf{Output:} entity\_id = ``023-Source-Class-ProgramCommitteeChair''\\
\textbf{Query: Find entity metadata} 
\begin{lstlisting}[language=SQL]
SELECT o.entity_type, m.embedding 
From ontology_matching o, {matching_table} m
WHERE o.entity_id = m.entity_id AND o.entity_id = {entity_id};
\end{lstlisting}
\textbf{Output:} entity\_type = ``Class'', content\_embedding = [...]  \\ \hline
\hline
\textbf{Tool: Hybrid Database Search with Syntactic \& Lexical \& Semantic Matcher}    \\ \hline
\textbf{Input:} content\_embedding = [...], \\
matching\_table = ``syntactic\_matching/lexical\_matching/semantic\_matching'', \\
similarity\_threshold = 0.90, top\_k = 3, source\_or\_target = ``Source'', entity\_type = ``Class'' \\
\textbf{Query: Find matching candidates} 
\begin{lstlisting}[language=SQL]
WITH vector_matches AS (
SELECT entity_id, 1 - (embedding <=> '{content_embedding}') AS similarity
FROM {matching_table}
WHERE 1 - (embedding <=> '{content_embedding}') >= {similarity_threshold})
SELECT o.entity_id, v.similarity as similarity 
FROM ontology_matching o, vector_matches v
WHERE o.entity_id IN (SELECT entity_id FROM vector_matches) 
AND o.entity_id =  v.entity_id 
AND o.source_or_target != {source_or_target} 
AND o.entity_type = {entity_type}
ORDER BY v.similarity DESC
LIMIT {top_k};
\end{lstlisting}
\textbf{Output:} matching\_results = [(``syntactic\_matching'', []), (``lexical\_matching'', [``095-Target-Class-Chair\_PC'']), 
(``semantic\_matching'', [``103-Target-Class-Member\_PC'', ``114-Target-Class-Scholar'', ``092-Target-Class-Author''])]\\ \hline
\hline
\textbf{Tool: Matching Summariser}    \\ \hline
\textbf{Input:} matching\_results = [...] \\
\textbf{Method:} reciprocal\_rank\_fusion(matching\_results)\\
\textbf{Output:} matching\_summary = [(1.0, [``095-Target-Class-Chair\_PC'', ``103-Target-Class-Member\_PC'']), (0.5, [``114-Target-Class-Scholar'']), (0.33, [``092-Target-Class-Author''])] \\ \hline
\textbf{Tool: Matching Validator}    \\ \hline
\textbf{Input:} entity\_uri = ``\texttt{http://cmt\#ProgramCommitteeChair}'', \\
matching\_summary = [...], context = ``conference'' \\
\textbf{Extract:} entity\_name from entity\_uri, each matching\_entity\_name from matching\_summary.\\
\textbf{Prompt:} \textit{Question: Is \{entity\_name\} equivalent to \{matching\_entity\_name\}? Context: \{context\} Answer the question within the context. Answer yes or no. Give a short explanation.} \\
\textbf{Output:} best\_matching\_entity\_id = ``095-Target-Class-Chair\_PC''\\
``095-Target-Class-Chair\_PC'': \textit{``Yes. In the context of a conference, the term `program committee chair' is equivalent to `chair PC.' Both refer to the individual responsible for overseeing the program committee, which is tasked with organizing the conference's academic or technical program, including the review and selection of submitted papers.''} (AI-generated content) \\
``103-Target-Class-Member\_PC'': \textit{``No. The program committee chair is not equivalent to a member of the program committee (PC). The program committee chair is responsible for overseeing the entire review process, coordinating the activities of the PC members, and making final decisions on the acceptance of submissions. In contrast, a member of the PC is primarily responsible for reviewing and evaluating submitted papers.''} (AI-generated content) \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}

\addtocounter{table}{-1}

\begin{table*}[htbp]
\centering
\footnotesize
\renewcommand\arraystretch{1.2}
\tabcolsep=0.15cm
\caption[]{Tool calling in the Matching Agent - Continued.}
\begin{adjustbox}{height=0.9\height,center}
\begin{tabular}{p{1.12\linewidth}}
\hline
\textbf{Query: Find best matching entity} 
\begin{lstlisting}[language=SQL]
SELECT o.entity_uri FROM ontology_matching o
WHERE o.entity_id = {best_matching_entity_id};
\end{lstlisting}
\textbf{Output:} best\_matching\_entity\_uri = ``\texttt{http://confOf\#Chair\_PC}''\\ \hline
\hline
\textbf{Tool: Matching Merger}    \\ \hline
\textbf{Output:} Merge the best matching entity in the source ontology for the search from ``\texttt{http://confOf\#Chair\_PC}'' in the target ontology. \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}

\section{Evaluation}

\subsection{Evaluation Criteria}

In information retrieval, a common assessment of matching tasks is based on comparing predicted results with the expected output. Precision and recall are used to measure the correctness and completeness of the matching, respectively. When adapting these measures to OM, the predicted results generated by the system are denoted Alignment (A), and the expected results provided by the domain experts are denoted Reference (R)~\citep{do2003comparison}. Therefore, precision and recall for OM tasks are defined as:

\begin{equation}
Precision = \frac{|A \cap R|}{|A|} \qquad Recall = \frac{|A \cap R|}{|R|}
\end{equation}

Precision and recall are commonly combined into a single measure F1 score, defined as:

\begin{equation}
F_1 \ Score= \frac{2}{Precision^{-1} + Recall^{-1}}
\end{equation}

\subsection{Evaluation of Three OAEI Tracks}

We test our proof-of-concept system with three OAEI tracks containing different types of OM tasks. These include few-shot tasks with a small proportion of trivial correspondences (\ref{evaluation: conference-track} Test Case), simple tasks with a large proportion of trivial correspondences (\ref{evaluation: anatomy-track} Test Case 1 and~\ref{evaluation: mse-track} Test Case 3), complex tasks with a large proportion of non-trivial correspondences (\ref{evaluation: anatomy-track} Test Case 2), with complex references (\ref{evaluation: mse-track} Test Case 1), or requiring domain-specific knowledge (\ref{evaluation: mse-track} Test Case 2). We report the evaluation metrics for the best-performing singular model gpt-4o and its hyperparameter settings over a single run. We ran multiple trials and found slight differences in the results due to the non-determinism of LLMs, but these differences are not significant with respect to the precision of the results we report. For all test cases in the three OAEI tracks, we select the hyperparameter settings of similarity\_threshold = 0.90 and top@k = 3. See section~\ref{ablation: hyperparameter} for a discussion on the hyperparameter settings of Agent-OM.

\subsubsection{OAEI Conference Track}
\label{evaluation: conference-track}

The OAEI Conference Track contains pairwise alignments for 7 small and medium-sized conference-related ontologies with a total of 21 matching tasks~\citep{cheatham2014conference,solimando2014detecting,solimando2017minimizing,zamazal2017ten}. In each alignment, the trial correspondences that can be used to train the models are very limited (commonly less than 10). All conference ontologies in this track use the text-type naming convention, where the names of classes and properties have natural language meanings. We use the publicly available reference ra1-M3 as the reference (R), including class and property mappings.

Figure~\ref{fig: conference-domain} compares Agent-OM with the 15 OM systems in OAEI 2022 and OAEI 2023. Agent-OM achieves above-average performance. Its overall F1 score ranks 3/13 in 2022 and 5/12 in 2023. We note that ra1-M3 is known to be missing valid equivalence mappings~\citep{conference2023}. We believe that Agent-OM could achieve better performance over a complete reference such as ra2-M3 or rar2-M3. These are not publicly available at the time of writing.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2025-figures/conference.png}
\caption{OAEI Conference Track Test Case.}
\label{fig: conference-domain}
\end{figure}

\subsubsection{OAEI Anatomy Track}
\label{evaluation: anatomy-track}

The OAEI Anatomy Track contains a reference alignment for the mouse anatomy and the human anatomy, created and evolved from~\citep{bodenreider2005mice,beisswanger2012towards,euzenat2011ontology,dragisic2017experiences}. Both ontologies use the code-type naming convention, where the names of classes and properties are biomedical codes. The track originally contains a large proportion of trivial correspondences that have the same standardised labels (e.g. ``femoral artery'' and ``Femoral\_Artery''). We report the results of our evaluation in two parts: alignment with trivial correspondences and alignment with non-trivial correspondences.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\arabic*)]

\item Test Case 1: Figure~\ref{fig: anatomy-easy} compares Agent-OM with the results of the 12 OM systems in OAEI 2022 and OAEI 2023 for alignment with trivial correspondences. Almost all OM systems achieve relatively high precision and recall when matching with trivial correspondences. For Agent-OM, its overall F1 score ranks the second highest in 2022 and 2023.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2025-figures/anatomy.png}
\caption{OAEI Anatomy Track Test Case 1.}
\label{fig: anatomy-easy}
\end{figure}

\item Test Case 2: We remove these trivial correspondences from both the reference (R) and alignment (A) to focus the matching performance comparison on non-trivial correspondences. Figure~\ref{fig: anatomy-hard} compares Agent-OM with the results of the 12 OM systems in OAEI 2022 and OAEI 2023 for alignment with non-trivial correspondences. We observe better performance by Agent-OM. The overall F1 score of Agent-OM is superior to the 11 OM systems including an LLM-based OM system OLaLa, and only behind one deep learning (DL)-based OM system Matcha~\citep{cotovio2024matcha}, which could have benefited from an unusually large training set available for this case.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2025-figures/anatomy-filter.png}
\caption{OAEI Anatomy Track Test Case 2.}
\label{fig: anatomy-hard}
\end{figure}

\end{enumerate}

\subsubsection{OAEI MSE Track}
\label{evaluation: mse-track}

The OAEI MSE Track provides reference alignments for ontologies in materials science and engineering~\citep{engy2020}. The track contains three test cases aligning MaterialInformation~\citep{ashino2010materials}, MatOnto~\citep{matonto}, and EMMO~\citep{emmo}. The MaterialInformation and MatOnto use the text-type naming convention, while the EMMO uses the code-type naming convention.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\arabic*)]

\item Test Case 1: This test case provides a reference alignment for a fragment of MaterialInformation and the medium-sized MatOnto. The challenge of this task arises due to the reference intentionally including several subsumption correspondences, when OM systems may mistakenly map subsumptions into equivalence relations. Figure~\ref{fig: mse-1} compares Agent-OM with the results of the 4 OM systems in OAEI 2022 and OAEI 2023. Agent-OM achieves the best performance, with the highest F1 score.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2025-figures/mse-1.png}
\caption{OAEI MSE Track Test Case 1.}
\label{fig: mse-1}
\end{figure}

\item Test Case 2: This test case provides a reference alignment for the complete MaterialInformation and the medium-sized MatOnto. The challenge of this task is to align many examples of specific terminology, abbreviations, and acronyms used in materials science. For example, ``Au'' stands for ``Gold'', ``Ag'' stands for ``Silver'', and ``Cu'' stands for ``Copper''. Figure~\ref{fig: mse-2} compares Agent-OM with the results of the 4 OM systems in OAEI 2022 and OAEI 2023. Agent-OM achieves the best performance in precision, recall, and overall F1 score across the results of OAEI 2022 and OAEI 2023. We should expect an LLM-based matcher to have high recall on this test case due to its access to extensive training literature.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2025-figures/mse-2.png}
\caption{OAEI MSE Track Test Case 2.}
\label{fig: mse-2}
\end{figure}

\item Test Case 3: This test case provides a reference alignment for the complete MaterialInformation and the medium-sized EMMO. The EMMO extends the upper ontology called Basic Formal Ontology (BFO). This means that the classes in the EMMO are somewhat standardised according to the BFO classes. Figure~\ref{fig: mse-3} compares Agent-OM with the results of the 4 OM systems in OAEI 2022 and OAEI 2023. The performance of Agent-OM is competitive with the best of the OAEI 2022 results and in OAEI 2023 is bettered by the DL-based OM system Matcha.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2025-figures/mse-3.png}
\caption{OAEI MSE Track Test Case 3.}
\label{fig: mse-3}
\end{figure}

\end{enumerate}

\section{Ablation Study}

In this section, we first look into the system components, including the overall architecture, LLMs, text embedding models, hybrid database, matching validator, and matching merger. Then, we move on to the hyperparameter settings for similarity threshold and top@k.

\subsection{System Components}

\subsubsection{Architectures}

We compare Agent-OM with two simpler architectures where the OM is much more reliant on straightforward LLM use. (1) \textit{LLM-Only}: Given $O_s$ and $O_t$, this approach extracts each $e1 \in O_s$ and $e2 \in O_t$. The matching decision is purely based on LLMs without any additional information. (2) \textit{LLM-with-Context}: Given $O_s$ and $O_t$, this approach extracts each $e1 \in O_s, e2 \in O_t$ and their syntactic, lexical, and semantic information. The matching decision uses LLMs to determine whether two concepts are identical or not based on the information provided.

The experiment is run on the CMT-ConfOf alignment demonstrated in section~\ref{sub-sec: running example}. We use the GPT model gpt-4o. For Agent-OM, we choose the hyperparameter settings of similarity\_threshold = 0.90 and top@k = 3. Figure~\ref{fig: different-architecture} compares Agent-OM with \textit{LLM-Only} and \textit{LLM-with-Context}. \textit{LLM-Only} shows low precision and recall. \textit{LLM-with-Context} partially overcomes this deficiency by providing additional information, but token consumption is extremely high without optimising the matching candidate selection. The performance of \textit{LLM-with-Context} is unstable over multiple runs due to the effects of stochastic LLM results. Our Agent-OM architecture handles these challenges with tool calling agents and hybrid database searches. Note that the CMT-ConfOf alignment demonstrated here is a small alignment task, while Agent-OM is expected to be relatively more effective and efficient in large-scale OM tasks.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2025-figures/different-architecture.png}
\caption{Comparison with LLM-based architectures.}
\label{fig: different-architecture}
\end{figure}

\subsubsection{LLMs}
\label{ablation: llm}

Figure~\ref{fig: different-llm} varies LLMs in Agent-OM on the OAEI Anatomy Track. In general, API-accessed models perform better than open-source models. The leading models, gpt-4o and claude-3-sonnet, are both large API-accessed models. Among open-source models, gemma-2-9b achieves the best performance, while llama-3-8b is relatively poor. Curiously, although we see improved performance with llama-3.1-8b over its previous version, qwen-2.5-7b does not show an advantage over its previous version. This may be a side effect of LLM developers optimising for tasks other than OM. We experimented with other LLMs derived from the Llama and Qwen families and generally found poor performance, possibly due to the fine-tuning for specific tasks.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2025-figures/anatomy-llm.png}
\caption{Comparison of different LLMs. API-accessed models are shown as triangles and open-source models as circles.}
\label{fig: different-llm}
\end{figure}

\subsubsection{Text Embedding Models}

We also test three different text embeddings in~\citep{openaiembeddingmodels} on the OAEI Anatomy Track. The default length of the embedding vector is 1536 for text-embedding-ada-002 and text-embedding-3-small, and 3072 for text-embedding-3-large. We do not observe a significant difference arising from varying the text embeddings from text-embedding-3-small to text-embedding-3-large. We do not see that text-embedding-3-small and text-embedding-3-large perform better than text-embedding-ada-002.

\subsubsection{Hybrid Database} 

The use of a hybrid database unlocks the potential for search-based OM. We define $N_s$ and $N_t$ as the number of entities extracted from the source ontology ($O_s$) and the target ontology ($O_t$), respectively. In naive LLM-based OM, the matching is performed using binary questions to compare each pair of entities from $O_s$ and $O_t$ based on their relevant information. The complexity of the comparison is $N_s \times N_t$ (for retrieval and matching). In search-based OM, we first retrieve entity information from $O_s$ and $O_t$ and store it in a hybrid database. Following our design and implementation in section~\ref{sec: approach} and~\ref{sec: implementation}, the complexity is $N_s+N_t$ (for retrieval) + 0 (for search) + $k(N_s+N_t)$ (for validation) + 0 (for merge). Search-based OM is cost-effective because the inequality $(k+1)(N_s+N_t)<N_s \times N_t$ always holds in common OM task settings where $N_s, N_t \gg k+1$. We also apply two tools to reduce LLM hallucinations: the matching validator and the matching merger.

\subsubsection{Matching Validator} 

We employ a matching validator by asking the LLM to self-check the candidate correspondences. It is helpful in detecting two common types of false positive mappings: (1) non-existent mappings and (2) counter-intuitive mappings. Figure~\ref{fig: validation} compares precision, recall, and F1 score with and without validation in the three OAEI tracks we analysed. The matching results with validation generally achieved an improvement in precision and F1 score, with a slight decrease in recall. This is in line with the findings in CoT with self-consistency (CoT-SC)~\citep{wang2023selfconsistency}, where the provision of a self-check can reduce LLM hallucinations. Our experiment set the hyperparameters to similarity\_threshold = 0.90 and top@k = 3, so the improvement in matching performance is not statistically significant, but the matching validator will have a great impact on performance with lower similarity thresholds and higher top@k values.

\begin{figure}[htbp]
\centering
\subfloat{\includegraphics[width=0.333\columnwidth]{qiang-vldb-2025-figures/validation-precision.png}}
\subfloat{\includegraphics[width=0.333\columnwidth]{qiang-vldb-2025-figures/validation-recall.png}}
\subfloat{\includegraphics[width=0.333\columnwidth]{qiang-vldb-2025-figures/validation-f1.png}}
\caption{Comparison of without/with matching validator.}
\label{fig: validation}
\end{figure}

\subsubsection{Matching Merger} 

We apply a merge function $O_s \Leftrightarrow O_t$ combining the results of $O_s \Rightarrow O_t$ and $O_s \Leftarrow O_t$ to improve the matching performance. Figure~\ref{fig: merge} shows the comparison of precision, recall, and F1 score in $O_s \Rightarrow O_t$, $O_s \Leftarrow O_t$, and $O_s \Leftrightarrow O_t$ in the three OAEI tracks we analysed. The merged matching results generally achieved a significant improvement in precision and F1 score, with a slight decrease in recall. The results are in line with the findings in RAG-Fusion~\citep{ragfusion}, where providing two different paths to perform the same matching task can reduce LLM hallucinations.

\begin{figure}[htbp]
\centering
\subfloat{\includegraphics[width=0.333\columnwidth]{qiang-vldb-2025-figures/merge-precision.png}}
\subfloat{\includegraphics[width=0.333\columnwidth]{qiang-vldb-2025-figures/merge-recall.png}}
\subfloat{\includegraphics[width=0.333\columnwidth]{qiang-vldb-2025-figures/merge-f1.png}}
\caption{Comparison of $\mathbf{O_s \Rightarrow O_t}$, $\mathbf{O_s \Leftarrow O_t}$, and $\mathbf{O_s \Leftrightarrow O_t}$}
\label{fig: merge}
\end{figure}

\subsection{Hyperparameter Settings}
\label{ablation: hyperparameter} 

\subsubsection{Similarity Threshold}

We test the similarity threshold $T\in[0.50,\allowbreak0.55, \allowbreak0.60,\allowbreak...,\allowbreak0.90, \allowbreak0.95, \allowbreak1.00]$ in the three OAEI tracks we analysed. The optimal similarity threshold appears to be $T\in[0.90, 0.95]$, balancing the trade-off between precision and recall, thus achieving a higher overall F1 score. If we consider the similarity threshold as the required confidence interval (CI) for candidates for equivalence matching, this setting reflects the convention of accepting a 5-10\% probability of observing values outside the estimation. The insensitivity of the results to the threshold value is more apparent in large-scale OM tasks, such as the OAEI Anatomy Track.

\subsubsection{Top@k}

We also test the top@k values $ k\in\{1, 2, 3,..., 8, 9, 10\}$ in the three OAEI tracks we analysed. We observe that $k=1$ and $k=2$ do not provide enough candidates for the LLM to select, while appropriate correspondences are rarely found where $k>5$. We recommend setting $k\in\{3, 4, 5\}$ to balance the computational complexity and precision of the results. Note that we deal with the tie-break case where multiple entities have the same RRF scores. In such cases, the total number of entities tested may be greater than $k$ because these equally-scored entities share the same ranking.

\subsubsection{How to choose Similarity Threshold and Top@k?}

Ontologies are context-dependent conceptual models that follow different conventions and restrictions to reflect different application-level requirements~\citep{ontology2021conceptual}. The hyperparameter settings can be adjusted for each specific OM task using reference mappings to achieve an optimal result. We observe that higher similarity thresholds and lower top@k values could result in high precision where most of the trivial mappings can be found, but some more obscure true mappings may be missed, lowering recall. On the other hand, lower similarity thresholds and higher top@k values could result in high recall, but the precision may be low as more false mappings are generated during the matching process. This indicates that the applied matching refinements (validator and merger) would be more powerful in settings with lower similarity thresholds and higher top@k values. We found in our extensive OAEI experiments that threshold $T\in[0.90, 0.95]$ and top@k $k\in\{3, 4, 5\}$ were optimal. In the real-world application of Agent-OM to a matching problem with no reference, we advise choosing $T$ and $k$ within these ranges.

\section{Discussion}

Google DeepMind classifies AI autonomy into 6 levels~\citep{morris2024levels}: No AI (Level 0), AI as a tool (Level 1), AI as a consultant (Level 2), AI as a collaborator (Level 3), AI as an expert (Level 4), and AI as an agent (Level 5). We believe that the potential of LLMs is not only as a tool, a consultant, a collaborator, or an expert to answer binary classification questions in OM tasks, but also as an agent to simulate human behaviour in performing OM tasks, including data preprocessing, data preparation, data analysis, and data validation. Higher autonomy reduces barriers to accessing LLMs in OM tasks.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\arabic*)]

\item LLM-agent-based OM is more efficient than LLM-based OM. LLMs are computationally expensive. While LLM-based OM using binary classification questions has repetitive LLM prompting, LLM-agent-based OM leverages the vector database to store ontology retrieval results, reducing the financial cost of token consumption.

\item LLM-agent-based OM is also more effective than LLM-based OM. LLM-based OM is commonly observed to have limitations. Due to the nature of its large knowledge base, it is possible to discover positive correspondences but also to find unavoidable false mappings or missing true mappings. LLMs are zero-shot reasoners~\citep{kojima2022large}, but they are also few-shot learners~\citep{brown2020language}. Their capacity for reasoning depends on the richness of the information provided. With the assistance of autonomous agents for extensive planning, tools, and memory, LLM-agent-based OM can unlock the potential of LLMs and therefore feature the following advantages:

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item Context Learning: LLMs have a large corpus of background knowledge. Given a context, LLMs can select relevant background knowledge and therefore perform better in lexical matching.
\item Transitive Reasoning: LLMs can reason on transitive relationships. They can also understand general and domain-specific scenarios and apply lexical validation when necessary.
\item Self Correction: LLMs have a strong capacity for self correction. Even given a wrong statement, LLMs have good judgement to automatically remove false mappings. For example, semantic matching can cause false mappings because it considers only the data structure and ignores the linguistic meaning of the entity. However, such a small piece of false information does not influence the correct truth that LLMs nevertheless learn.
\end{enumerate}

\end{enumerate} 

Despite the success of agent-powered LLMs for OM, there may be further opportunities for improvement as follows.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\arabic*)]
\item A matching process could be more complex. Although CoT may simulate how humans plan and perform tasks, it is still an incomplete model of human thought. Human reasoning employs a more complex network of thoughts, as humans tend to try different isolated paths (i.e. ToT, tree of thoughts~\citep{yao2023tree,long2023large}), explore multiple paths (i.e. GoT, graph of thoughts~\citep{besta2024graph,yao2024got}), and backtrack, split, or merge to find the optimal solution to the problem. For example, people may use discovered mappings as input to the next iteration.
\item Prompt engineering is the key to instructing efficient LLM agents. These prompts are currently hand-crafted. For prompt-based tools, different LLMs may have varying default chat templates. Finding generic prompts across all LLMs is almost impossible. However, we provide the simplest standardised version of the prompts from our experiments. The prompts used in our system currently support mainstream LLMs, such as OpenAI GPT models, Authropic Claude models, Meta Llama 3, Alibaba Qwen 2, Google Gemma 2, and ChatGLM 4. For those models not included in the list, we also provide an interface to add new LLMs to our system, but it may require minor code customisation to fit the LLMs used. We expect that our system will support more models via open-source community efforts in the future. We seek automatic prompt engineering and will consider using soft prompts in future versions.
\item LLM hallucinations can be mitigated, but cannot be eliminated. The accuracy of the RAG remains an open question. Human-in-the-loop may remain necessary~\citep{ouyang2022training}. Advanced RAG techniques, such as including the explanatory context in the RAG process~\citep{contextual-claude}, are promising directions.
\item There is a trade-off between precision and recall. Strict rules could result in high precision where most of the trivial true mappings can be found, but some obscure true mappings may be missing. On the other hand, loose rules could result in a high recall score, but the precision score may become very low as more false mappings are generated during the matching process.
\item For LLMs used for OM, we find Moravec's paradox that \textit{``the hard problems are easy and the easy problems are hard''}~\citep[p.~192]{pinker2003language}. Although Agent-OM performs well in complex and few-shot OM tasks, it is not outstanding on simple OM tasks. We will also consider integrating the LLM-based approach with traditional knowledge-based and ML-based approaches.
\end{enumerate}

\section{Limitations}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\arabic*)]
\item We evaluate only the TBox matching datasets that match classes, object properties, and datatype properties. ABox matching datasets (including individual data instances) are not considered here due to privacy concerns in our targeted building application domain. Additional data engineering (e.g. data de-identification and fuzzing) may be required to apply LLMs to ABox matching datasets to avoid personal and sensitive information exposure.
\item Due to the high cost of API calls for API-accessed commercial LLMs, experiments with the newest commercial models (e.g. OpenAI o1 and Anthropic claude-3-opus) are not included in this study. According to our findings in section~\ref{ablation: llm}, we hypothesise that these models could achieve better performance in OM tasks.
\item There may be additional resource requirements for running open-source LLMs locally. The run time for API-accessed commercial LLMs is controlled by the LLM providers.
\end{enumerate}

\section{Conclusion}

In this chapter, we introduce a new design paradigm for OM systems. Agent-OM, an agent-powered LLM-based framework, is proposed and implemented with a proof-of-concept system. We compare our system with state-of-the-art OM systems to perform different types of OM tasks. The system has shown a powerful capability to perform OM tasks at different levels of complexity, leveraging the potential of using LLM agents for OM. We also discuss our observations on the advantages and current limitations of using LLMs and LLM agents for OM tasks.

Our work focuses on large pre-trained foundation models that are impossible to retrain and hard to fine-tune. Our approach yields good results on LLMs for OM tasks without changing the LLM model itself, but by utilising CoT, ICL/RAG, and prompt engineering techniques. It is a simple, lightweight, and natural language-driven approach with high scalability. Agent-OM is all you need. While OM has been studied for two decades or more, we are now at a point where the goal of 100\% accurate, fully-automated, and domain-independent OM seems to be within reach.

Agent-OM is one of the iconic OM systems based on LLMs and LLM agents. The system was evaluated in several domains in the OAEI 2025 campaign (see Appendix~\ref{appendix: agent-om-oaei-2025}). In addition to the system itself, we propose using Agent-OM to develop a dataset to benchmark LLM hallucinations in OM tasks (see Appendix~\ref{appendix: oaei-llm}).

Ontology versioning is a specific type of OM that we discuss in the next chapter.

\paragraph*{Publication Statement}

Most of the work presented in this chapter has been published as~\bibentry{qiang2023agent}.

==> qiang-anu-thesis-content/building-odps.tex <==
\chapter{Ontology Design Patterns for Data-Driven Smart Buildings}
\label{chap: building-odps}

Ontologies play a critical role in data exchange, information integration, and knowledge sharing across diverse smart building applications. Yet, semantic differences between the prevailing building ontologies hamper their purpose of bringing data interoperability and restrict the ability to reuse building ontologies in real-world applications. In this section, we propose and adopt a framework to conduct a systematic comparison and evaluation of four popular building ontologies (Brick Schema, RealEstateCore, Project Haystack and Google's Digital Buildings). Further, we discuss ontology compatibility and investigate building ontology design patterns (ODPs) to support ontology matching, alignment, and harmonisation. These ODPs cover building spaces, equipment and systems, and points and measurements.

Smart buildings, also known as digital buildings or intelligent buildings, have received significant attention in recent years and are contributing to digital innovation in the building industry. The global smart building market is envisioned to grow at a compound annual growth rate (CAGR) of 10.9\% by 2026, with a total market value of USD 121.6 billion~\citep{smartbuildingmarket2021}. The popularity of smart buildings is due to their ability to provide effective and efficient management of building facilities and optimum usage of resources through intelligent building systems~\citep{pritoni2021metadata}.

A smart building is a complex concatenation of structures, systems, and technology. Smart building data shows typical characteristics of ``big data'' viz: high volume, variety, velocity, veracity, and value (5Vs)~\citep{bashir2017iot}. A smart building can easily collect thousands of data points per hour. These data can come from a wide range of resources, including smart equipment, building IoT platforms, building management systems (BMS), and building facility and maintenance systems~\citep{miller2017building}. Currently, there are different approaches used by service providers and vendors for managing building data. While some buildings may have customised data models to describe relevant context, functions, and interactions within buildings, oftentimes, buildings have limited information available to represent data along with the context~\citep{smartbuildingsurvey2019}. Various studies have identified the importance of a uniform data model that could exchange building data across various sensors, devices, systems, and buildings in an integrated, dynamic, and functional manner~\citep{venugopal2012semantics,fierro2022survey,lbd2023}.

Ontologies are human-readable and machine-interpretable representations that classify entities that may exist and the relationships between them, enabling richer data description, information integration, and knowledge sharing~\citep{stephan2007knowledge}. Notably, a recent review of knowledge management in the building industry~\citep{deng2022transforming} shows that ontologies have great research significance in academia and the most extensive application fields, including the deployment of data-driven digital construction~\citep{kukkonen2022ontology,zheng2021shared}, predictive analytics and diagnostics~\citep{hu2021building,wang2021ontology,ren2021aligning}, and automated system optimisation (ASO)~\citep{schneider2020design,cao2022ontology,li2022ontology}. Approximately 90\% of the building management systems developed in the past ten years are built on (or are adopting) domain ontologies~\citep{luo2021overview}. Among these building ontologies, Brick Schema~\citep{balaji2016brick} (abbr. ``Brick''), RealEstateCore~\citep{hammar2019realestatecore} (abbr. ``RECore''), Project Haystack~\citep{john2020project} (abbr. ``Haystack''), and Google's Digital Buildings~\citep{berkoben2020digital} (abbr. ``DB'') are some of the well-known ontologies that are related to operational aspects of buildings including their air conditioning and electrical systems. See Section~\ref{subsec: selected building ontologies} and~\ref{subsec: selected building concepts} for the reasons these particular building ontologies and concepts were selected for this study. While these building ontologies tend to capture similar details and contextual information in a building, they are developed and maintained by different organisations for different purposes. As a result, building ontologies may differ in the level of abstraction. The overlapping nature is often confusing for the users, and different ways of expressing entities and their relationships hamper the interoperability between these ontologies.

The existence of different ontologies to represent the same type of building systems presents many challenges for semantic model developers and users. They are often unsure of which ontology to use to create building data models. The scalability of data-driven analytics is severely hampered due to existing interoperability limitations. While each ontology has evolved to meet a specific set of needs and abstract building information at multiple levels, there is no consistent and interpretable semantics to verify their former relationships~\citep{ASHRAE223P}, nor clearly defined case boundaries for each building ontology~\citep{brickrecore2022}. Mixing ontologies, though permitted in RDF~\citep{rdf2014}, may be impractical due to differing verification rules (e.g., OWL~\citep{owl2012} vs SHACL~\citep{shacl2017}) or query options (e.g., matching types vs tags).

We conduct a systematic comparison and evaluation of four building ontologies both in the Terminological Box (TBox) and the Assertion Box (ABox). Our objective is to discover ontology compatibility and investigate ontology design patterns (ODPs) to support building ontology matching, alignment, and harmonisation. Specifically, this study makes the following contributions:

\begin{itemize}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt]
\item A Terminological Box (TBox) evaluation of four popular building ontologies using the OQuaRE Framework. Characteristics examined include Structural, Functional Adequacy, Maintainability, Transferability, Reliability, Compatibility, and Operability. An Assertion Box (ABox) evaluation of four popular building ontologies from an empirical study of modelling a medium-sized office building in Melbourne, Australia. HVAC (Heating, Ventilation, and Air Conditioning) related Building Spaces, Building Equipment and Systems, Building Points and Measurements have been considered in the study.
\item While the results implicitly indicate that there is no universal building ontology for integrating Linked Building Data (LBD), we further conduct a systematic analysis of compatibility between ontologies, and the common and conflicting design patterns in these building ontologies. We present our results of Building Ontology Design Patterns (ODPs).
\end{itemize}

\section{Related Work}

\subsection{TBox and ABox Evaluation}

Ontologists have distinguished two types of statements in ontologies for decades, commonly referred to as the Terminological Box (TBox) and the Assertion Box (Abox)~\citep{gruber1993translation}. The TBox is a set of ``schema'' axioms (classes and their definitions). For example, an elevator is defined as ``A device that provides vertical transportation between floors, levels or decks of a building, vessel or other structure''. In contrast, the ABox is a set of ``data'' axioms. They contain instance information about actual individuals and how these individuals are linked. ABox examples included statements like ``Elevator E1 is manufactured by Kone''.

A Knowledge Base (KB) is a TBox plus an ABox. The TBox evaluation could provide a superficial view of the structural design of a given ontology. In contrast, the ABox evaluation could provide application-level detailed information and explore the key concepts and relationships. Ontologists can apply different world views (i.e., TBox) to the same ground facts (i.e., ABox).

There are many ontology TBox and ABox evaluation methods available for use. There are no universal or optimal methods, and results are subject to the context of each case. One of our purposes is to introduce a generic framework for ontology comparison and selection. A comprehensive evaluation of TBox and ABox evaluation methods is out of scope here.

\subsection{Building Ontology Comparison and Evaluation}

The majority of works comparing building ontologies are conducted horizontally, i.e., comparing the same building ontologies in different applications. For example, the evaluation of Brick is based on eight canonical applications in six diverse buildings. Brick is expressive enough to capture 98\% of BMS data points on average in a wide variety of contexts~\citep{balaji2016brick}. Similarly, RECore evaluates the ontology by applying real-world applications to three real estate companies and one research project. A pilot deployment at property company Vasakronan shows RECore could cover in excess of 80,000 physical sensors and actuators and 20,000 external signals in ten buildings~\citep{hammar2019realestatecore}. There are some attempts to conduct the comparison vertically, i.e., comparing different building ontologies on the same data. For example, authors in~\citep{bhattacharya2015short} evaluate Haystack, Industry Foundation Classes (IFC)~\citep{ifc2018}, and Semantic Sensor Network (SSN)~\citep{compton2012ssn} in three testbed buildings and quantify their shortcomings in completeness, expressiveness, and flexibility. In a different study~\citep{quinn2021case}, authors apply two industry-recognised ontologies, Brick and Haystack, to a large industry dataset called KGS Clockwork. The result shows that Brick is the superior ontology to exhibit HVAC concepts for smart buildings.

The TBox evaluation, however, is not included in these works. The ABox evaluation conducted in these works is at a horizontal level, or a vertical evaluation that only includes one or two ontologies. This means it is infeasible to abstract key concepts and relationships, and investigate common and conflicting design patterns. In this study, we apply the analysis to both TBox and ABox. Also, we compare the ABox in four well-known building ontologies at a vertical level, i.e., applying one building sample data to different building ontologies.

\section{Methodology}

Figure~\ref{fig: methodology-odps} shows the methodology used in this study. We first select the building ontology corpus, and then the comparison is conducted in two phases: the TBox evaluation and the ABox evaluation. We apply four different building ontologies (i.e., TBox) to the same building sample (i.e., ABox). The TBox evaluation focuses on evaluating ontology quality (axiomatic design), while the ABox evaluation emphasises concept coverage and information retrieval in real-world use cases (assertions). We systematically compare four building ontologies with respect to ontology compatibility, and propose generic building ontology design patterns (ODPs).

\begin{figure}[!hbt]
\centering
\includegraphics[width=0.7\linewidth]{qiang-eb-2023-figures/Methodology.jpeg}
\caption{Methodology used in this study.}
\label{fig: methodology-odps}
\end{figure}

\subsection{Selected Building Ontologies}
\label{subsec: selected building ontologies}

In this study, we use Brick 1.2, RECore 3.3, Haystack 3.9.11 (referred to as Version 4 in marketing material), and DB 0.0.1. The online links of the selected building ontologies are listed in Table~\ref{tab: ontologies and namespaces}. We examined 30 building-related ontologies and chose these four ontologies. They cover the majority of the building concepts and are under continuous development. The complete list can be found in~\ref{appendix: building ontology corpus}.

\begin{table}[!hbt]
\caption{Selected building ontologies and their online links.}
\label{tab: ontologies and namespaces}
\begin{center}
\begin{tabular}{|l|l|}
\hline
Ontologies      & Online Links\\
\hline
\small Brick    & \small \url{https://brickschema.org/}\\
\small RECore   & \small \url{https://www.realestatecore.io/}\\
\small Haystack & \small \url{https://project-haystack.org/}\\
\small DB       & \small \url{https://google.github.io/digitalbuildings/}\\
\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Selected Building Concepts}
\label{subsec: selected building concepts}

The building concepts include three main parts: (1) Building Spaces, (2) Building Equipment and Systems, and (3) Building Points and Measurements. We examined the concepts defined in 30 building ontologies and building-related domain ontologies (shown in Figure~\ref{fig: building concepts}), and these three are the top-ranked concepts that most of the ontologies include and that are closely related to smart building applications.

\begin{figure}[!hbt]
\centering
\includegraphics[width=0.8\linewidth]{qiang-eb-2023-figures/Building_Concepts.jpeg}
\caption{Building concepts in 30 building and related domain ontologies.}
\label{fig: building concepts}
\end{figure}

\subsection{The TBox Evaluation: The OQuaRE Framework}

The notion of SQuaRE-based Ontology Quality Evaluation (OQuaRE) is inspired by Software product Quality Requirements and Evaluation (SQuaRE), an evaluation standard for software products~\citep{zubrow2004software}. As ontologies can be viewed as software artifacts of the application of a conceptual modelling process, authors in~\citep{duque2011oquare} refine this standard to evaluate the ontology quality based on the graph theory. 

The OQuaRE framework is a multi-layer ontology quality evaluation model that follows a bottom-up approach (shown in Figure~\ref{fig: OQuaRE}). The overall ontology quality is determined by a set of characteristics (C$_i$) and sub-characteristics (SC$_j$) with a family of metrics (M$_k$). As the value range of each metric is variant, we use a criteria evaluation (CE$_k$) to normalise a 5-scale quality score (NM$_k$). Then, these scores are categorised into different characteristics and sub-characteristics to calculate the mean value. The overall ontology quality score is the average quality score of its characteristics and sub-characteristics.

\begin{figure}[!hbt]
\centering
\includegraphics[width=1\linewidth]{qiang-eb-2023-figures/OQuaRE_Framework.jpeg}
\caption{The architecture of the OQuaRE Framework.}
\label{fig: OQuaRE}
\end{figure}

In this study, we employ the OQuaRE framework as part of our evaluation process. OQuaRE has been applied in a wide range of domains~\citep{mozzaquatro2018ontology,alghamdi2019quantitative,roldan2020ontology,munoz2021gente,cornejo2021ontoslam,mishra2022evaluating,tibaut2022framework,sanchez2023ontology} and brings significant benefits. Firstly, it tends to convert the ontology TBox evaluation into an engineering activity that follows the guidelines of an ISO standard (ISO/IEC 25000:2005). A series of calculated quantitative values can be generated during the evaluation process. Secondly, the OQuaRE framework is semi-automatic and requires few domain experts to be involved, and only to select and evolve characteristics and sub-characteristics at the early stage. Evaluations in~\citep{duque2013evaluation} claim that there is no statistical difference between the results automatically generated by the OQuaRE framework and the manual evaluations carried out by domain experts. Lastly, OQuaRE is a generic framework that can be tailored to each particular domain by giving priorities, or changing and evolving characteristics and sub-characteristics. To the best of our knowledge, this is the first attempt to use the OQuaRE framework to evaluate building ontologies. In our use case, we use the framework to develop a highly-scalable, domain-specific, semi-automatic TBox comparison and evaluation for building ontologies.

\subsection{The ABox Evaluation: An Empirical Study}

Our comparison is based on different building ontologies representing the same sample building data, retrieved from a medium-sized office building in Melbourne. The building has 3 storeys, 69 rooms, and 18 HVAC zones. The building data is collected from a variety of building points, such as sensors, setpoints, and commands from HVAC equipment and systems installed in or embedded in the building. The metadata used for modelling purposes is obtained from the Data Clearing House (DCH)~\citep{goldsworthy2022cloud}, a data platform for managing building data using semantic models of buildings. The total number of entities in the original Brick model is 1133. We map and extend this model to RECore, Haystack, and DB.

We also evolve these data points to ensure each category contains various types of instances (individuals). For the equivalent classes within one ontology (e.g. \textit{Break\_Room} and \textit{Breakroom} in Brick), we only create one individual instance. For the synonym classes across building ontologies (e.g. \textit{Floor} in Brick and \textit{Level} in RECore), we have a mapping process and create the same named individual in each ontology. Where these individuals cannot find an exact subclass, we categorise them into the closest superclass (e.g. the zone temperature sensor is mapped to \textit{sensor} in Haystack).

\paragraph{Building Spaces}

The concept of building spaces is twofold: spaces surrounding the building and spaces within the building. For spaces surrounding the building, we capture the geographical information (e.g. region, site) and outside facilities (e.g. onsite generation, storage, parking). The spaces within the building include physical spaces (e.g. floor and room) and logical spaces (e.g. HVAC zone). Note that the definition of the room is generalised and also includes common spaces (e.g. hallway, lobby, and lounge). Based on the levels of detail in nature, rooms are categorised into different superclasses and subclasses. For example, Room B.0, 1.12, and G.20 are categorised into Room (unspecified), Office (semi-specified), and Enclosed\_Office (specified) classes, respectively. A room is usually assigned to an HVAC zone. In particular, Room B.16 is a service room and does not belong to any HVAC zone.

\paragraph{Building Equipment and Systems}

The majority of building equipment consists of HVAC equipment. We consider water coil based air conditioning systems that include air side and water side equipment: air handling units (AHU), boilers, chillers, return and supply air fans, etc. The AHU is a large unit responsible for filtering, heating, and cooling the air supply. The basic components include outside and return dampers, filters, heating and cooling valves and coils, and supply fans. Exhaust fans are installed in rooms that require additional air discharge (e.g. the server room and kitchen), while fresh air fans are used for rooms that require additional air supply (e.g. the conference room and enclosed office).

Figure~\ref{fig: schematic} illustrates the schematic of HVAC systems. All the data from these systems is collected through a centralised BMS. AHU systems usually include dampers, filters, heating and cooling coils, and supply fans. The heating hot water (HHW) and chilled water (CHW) systems include boilers, chillers, pumps, heating and cooling valves and coils. Note that heating and cooling coils are the shared components across these systems.

\begin{figure}[!hbt]
\centering
\includegraphics[width=0.9\linewidth]{qiang-eb-2023-figures/Schematic.jpeg}
\caption{The schematics of HVAC systems.}
\label{fig: schematic}
\end{figure}

\paragraph{Building Points and Measurements}

We provide various building points operating for different purposes, including alarm, command, parameter, sensor, setpoint, and status. Most of the alarm points appear in the fire panel, while setpoint and status are related to the systems and sub-systems. Command, parameter, and sensor points can be seen in all kinds of building entities (e.g. building spaces, equipment, and systems). These building points measure a wide range of building information and provide useful data for BMS. The classification of building points is defined disparately in different building ontologies. Based on the functions and outputs, we map the same individuals into the corresponding classes. We also provide a variety of measurements at the building points, including temperature, humidity, pressure, etc.

\section{Results}

The results are twofold: (1) the TBox comparison and (2) the ABox comparison.

\subsection{The TBox Comparison of Building Ontologies}

\paragraph{Metrics, Characteristics and Sub-characteristics}

We follow the metrics and evaluation criteria defined in~\citep{duque2011oquare}, while Class Richness (CROnto) is removed and replaced by Relationship Richness (RROnto). CROnto is an ABox evaluation metric that calculates the mean number of instances per class, which is not within the scope of the TBox evaluation. The metrics used in the study are listed as follows, and their evaluation criteria are shown in Table~\ref{tab: evaluation criteria of metrics}. Note that the scores are scaled from 1 to 5: 1-Not Acceptable, 2-Improvement Required, 3-Minimally Acceptable, 4-Acceptable, and 5-Exceeds Requirements.

\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item M1-Lack of Cohesion in Methods (LCOMOnto): Mean length of the paths from leaf classes to Thing (owl:Thing).
\item M2-Weighted Method Count (WMCOnto): Mean number of the path (edges between classes) from leaf classes to Thing (owl:Thing).
\item M3-Depth of subsumption hierarchy (DITOnto): Length of the largest path from leaf classes to Thing (owl:Thing).
\item M4-Number of Ancestor Classes (NACOnto): Mean number of direct superclasses per leaf class.
\item M5-Number of Children (NOCOnto): Mean number of direct subclasses per leaf class.
\item M6-Coupling between Objects (CBOOnto): Number of direct superclasses of all classes divided by the number of classes not using Thing (owl:Thing) as a direct subclass.
\item M7-Response for a Class (RFCOnto): Number of properties (owl:ObjectProperty and owl:DatatypeProperty) directly accessed from the superclass divided by the number of all classes.
\item M8-Number of properties (NOMOnto): Mean number of properties (owl:ObjectProperty and owl:DatatypeProperty) divided by the number of all classes.
\item M9-Tangledness (TMOnto): Mean number of direct superclasses of the classes with multiple inheritance (i.e., have more than one subclass).
\item M10-Relationship Richness (RROnto): Number of subconcepts (rdfs:subClassOf) defined in the ontology divided by the number of relationships (rdfs:subClassOf) and properties (owl:ObjectProperty and owl:DatatypeProperty).
\item M11-Properties Richness (PROnto): Number of object and data properties defined in the ontology divided by the number of relationships (rdfs:subClassOf) and properties (owl:ObjProperty and owl:DataProperty).
\item M12-Attribute Richness (AROnto): Mean number of property restrictions (owl:Restrictions) per class.
\item M13-Annotation Richness (ANOnto): Mean number of annotations (rdfs:comment and rdfs:label) per class.
\item M14-Relationships per concept: (INROnto): Mean number of relationships (rdfs:subClassOf) per class.
\end{enumerate}

\begin{sidewaystable*}
\centering
\caption{Evaluation criteria of the metrics (retrieved from~\citep{duque2011oquare}).}
\label{tab: evaluation criteria of metrics}
\begin{tabular}{|l|lllll|}
\hline
\multirow{2}{*}{Metrics} & \multicolumn{5}{l|}{Scores} \\ \cline{2-6} 
& \multicolumn{1}{l|}{1} & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{3} & \multicolumn{1}{l|}{4} & \multicolumn{1}{l|}{5} \\ \hline
M1-Lack of Cohesion in Methods (LCOMOnto)   & \multicolumn{1}{l|}{\textgreater 8}  & \multicolumn{1}{l|}{(6-8{]}}     & \multicolumn{1}{l|}{(4,6{]}}     & \multicolumn{1}{l|}{(2, 4{]}}    & \textless{}=2     \\ \hline
M2-Weighted Method Count (WMCOnto)          & \multicolumn{1}{l|}{\textgreater 15} & \multicolumn{1}{l|}{(11,15{]}}   & \multicolumn{1}{l|}{(8,11{]}}    & \multicolumn{1}{l|}{(5, 8{]}}    & \textless{}=5     \\ \hline
M3-Depth of subsumption hierarchy (DITOnto) & \multicolumn{1}{l|}{\textgreater 8}  & \multicolumn{1}{l|}{(6-8{]}}     & \multicolumn{1}{l|}{(4,6{]}}     & \multicolumn{1}{l|}{(2, 4{]}}    & {[}1,2{]}         \\ \hline
M4-Number of Ancestor Classes (NACOnto)     & \multicolumn{1}{l|}{\textgreater 8}  & \multicolumn{1}{l|}{(6-8{]}}     & \multicolumn{1}{l|}{(4,6{]}}     & \multicolumn{1}{l|}{(2, 4{]}}    & {[}1,2{]}         \\ \hline
M5-Number of Children (NOCOnto)             & \multicolumn{1}{l|}{\textgreater 12} & \multicolumn{1}{l|}{(8-12{]}}    & \multicolumn{1}{l|}{(6,8{]}}     & \multicolumn{1}{l|}{(3,6{]}}     & {[}1,3{]}         \\ \hline
M6-Coupling between Objects (CBOOnto)       & \multicolumn{1}{l|}{\textgreater 8}  & \multicolumn{1}{l|}{(6-8{]}}     & \multicolumn{1}{l|}{(4,6{]}}     & \multicolumn{1}{l|}{(2, 4{]}}    & {[}1,2{]}         \\ \hline
M7-Response for a Class (RFCOnto)           & \multicolumn{1}{l|}{\textgreater 12} & \multicolumn{1}{l|}{(8-12{]}}    & \multicolumn{1}{l|}{(6-8{]}}     & \multicolumn{1}{l|}{(3-6{]}}     & {[}1-3{]}         \\ \hline
 M8-Number of properties (NOMOnto)          & \multicolumn{1}{l|}{\textgreater 8}  & \multicolumn{1}{l|}{(6-8{]}}     & \multicolumn{1}{l|}{(4,6{]}}     & \multicolumn{1}{l|}{(2, 4{]}}    & \textless{}=2     \\ \hline
M9-Tangledness (TMOnto)                     & \multicolumn{1}{l|}{\textgreater 8}  & \multicolumn{1}{l|}{(6-8{]}}     & \multicolumn{1}{l|}{(4,6{]}}     & \multicolumn{1}{l|}{(2, 4{]}}    & (0,2{]}           \\ \hline
M10-Relationship Richness (RROnto)          & \multicolumn{1}{l|}{{[}0,20{]}\%}    & \multicolumn{1}{l|}{(20-40{]}\%} & \multicolumn{1}{l|}{(40-60{]}\%} & \multicolumn{1}{l|}{(60-80{]}\%} & \textgreater 80\% \\ \hline
M11-Properties Richness (PROnto)            & \multicolumn{1}{l|}{{[}0,20{]}\%}    & \multicolumn{1}{l|}{(20-40{]}\%} & \multicolumn{1}{l|}{(40-60{]}\%} & \multicolumn{1}{l|}{(60-80{]}\%} & \textgreater 80\% \\ \hline
M12-Attribute Richness (AROnto)             & \multicolumn{1}{l|}{{[}0,20{]}\%}    & \multicolumn{1}{l|}{(20-40{]}\%} & \multicolumn{1}{l|}{(40-60{]}\%} & \multicolumn{1}{l|}{(60-80{]}\%} & \textgreater 80\% \\ \hline
M13-Annotation Richness (ANOnto)            & \multicolumn{1}{l|}{{[}0,20{]}\%}    & \multicolumn{1}{l|}{(20-40{]}\%} & \multicolumn{1}{l|}{(40-60{]}\%} & \multicolumn{1}{l|}{(60-80{]}\%} & \textgreater 80\% \\ \hline
M14-Relationships per class (INROnto)       & \multicolumn{1}{l|}{{[}0,20{]}\%}    & \multicolumn{1}{l|}{(20-40{]}\%} & \multicolumn{1}{l|}{(40-60{]}\%} & \multicolumn{1}{l|}{(60-80{]}\%} & \textgreater 80\% \\ \hline
\end{tabular}
\end{sidewaystable*}

We keep the 5 characteristics from the original paper~\citep{duque2011oquare}: Structural (S), Functional Adequacy (F), Maintainability (M), Reliability (R), and Operability (O). We also add 2 new characteristics, Transferability (T) and Compatibility (C), related to the model transformation and modification process. Some of the sub-characteristics under these 7 characteristics have evolved. Table~\ref{tab: associations} summarises the associations between characteristics, their sub-characteristics, and the metrics involved.

\begin{sidewaystable*}
\centering
\caption{Associations between characteristics, sub-characteristics, and metrics (evolved from~\citep{tibaut2022framework}).}
\label{tab: associations}
\begin{tabular}{|l|l|l|}
\hline
Characteristics                             & Sub-characteristics                       & Metrics Included           \\ \hline
\multirow{4}{*}{Structural (S)}             & Formal Relations Support (S-FRS)          & M10                        \\ \cline{2-3} 
                                            & Cohesion (S-C)                            & M1                         \\ \cline{2-3} 
                                            & Tangledness (S-T)                         & M9                         \\ \cline{2-3} 
                                            & Redundancy (S-R)                          & M13                        \\ \hline
\multirow{9}{*}{Functional Adequacy (F)}    & Controlled Vocabulary (F-CV)              & M13                        \\ \cline{2-3} 
                                            & Schema and Value Reconciliation (F-SVR)   & M10, M12, M13              \\ \cline{2-3} 
                                            & Consistent Search and Query (F-CSQ)       & M10, M12, M14              \\ \cline{2-3} 
                                            & Knowledge Acquisition (F-KA)              & M13, M10, M8               \\ \cline{2-3} 
                                            & Similarity (F-S)                          & M10, M12                   \\ \cline{2-3} 
                                            & Indexing and Linking (F-IL)               & M10, M12, M14              \\ \cline{2-3} 
                                            & Results Representation (F-RR)             & M12                        \\ \cline{2-3} 
                                            & Guidance and Decision Trees (F-GDT)       & M14, M12                   \\ \cline{2-3} 
                                            & Knowledge Use (F-KU)                      & M13, M12, M14, M8, M1, M4  \\ \hline
\multirow{6}{*}{Maintainability (M)}        & Modularity (M-M)                          & M2, M6                     \\ \cline{2-3} 
                                            & Reusability (M-R)                         & M2, M3, M5, M7, M8, M6     \\ \cline{2-3} 
                                            & Analysability (M-A)                       & M2, M3, M1, M7, M8, M6     \\ \cline{2-3} 
                                            & Changeability (M-C)                       & M2, M3, M1, M7, M8, M6, M5 \\ \cline{2-3} 
                                            & Modification Stability (M-MS)             & M2, M6, M1, M7, M5         \\ \cline{2-3} 
                                            & Testability (M-T)                         & M2, M3, M1, M7, M8, M6     \\ \hline
                Transferability (T)         & Adaptability (T-A)                        & M2, M3, M7, M6             \\ \hline
\multirow{2}{*}{Reliability (R)}            & Recoverability (R-R)                      & M2, M3, M8, M1             \\ \cline{2-3} 
                                            & Availability (R-A)                        & M1                         \\ \hline
                Compatibility (C)           & Replaceability (C-R)                      & M2, M3, M5, M8             \\ \hline
                Operability (O)             & Learnability (O-L)                        & M2, M1, M7, M8, M6, M5     \\ \hline
\end{tabular}
\end{sidewaystable*}

\newpage

\paragraph{Axiomatic Design Evaluation}

Figure~\ref{fig: comparison of four building ontologies} shows the results of comparing four building ontologies. The overall quality scores of the four building ontologies are all above the Minimally Acceptable level (3). Haystack (4.25) has the highest overall score, followed by Brick (3.93), RECore (3.91), and DB (3.60). The scores of the characteristics in each ontology also meet the Minimally Acceptable level (3), except for the score of Reliability (2.88) in DB. We include the detailed scores of characteristics and sub-characteristics of four building ontologies in Figure~\ref{fig: OQuaRE sub-characteristics} to explore the insights of the axiomatic design.

\begin{figure*}[!hbt]
\centering
\includegraphics[width=1\linewidth]{qiang-eb-2023-figures/Building_Ontology.png}
\caption{The TBox comparison of four building ontologies.}
\label{fig: comparison of four building ontologies}
\end{figure*}

\begin{figure*}[!hbt]
\centering
\includegraphics[width=1\linewidth]{qiang-eb-2023-figures/OQuaRE_Sub-characteristics.jpeg}
\caption{The characteristics and sub-characteristics in each building ontology.}
\label{fig: OQuaRE sub-characteristics}
\end{figure*}

\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item In Brick, 4 of 7 characteristic scores are equal to or above the Acceptable level (4). They are Structural (4.50), Maintainability (4.14), Transferability (4), and Operability (4.33). However, the characteristic scores of Functional Adequacy (3.56), Reliability (3.25), and Compatibility (3.75) are at the Minimally Acceptable level (3). The low score for Functional Adequacy is due to the sub-characteristics Similarity (F-S) and Results Representation (F-RR) mainly affected by the metric M12-Attribute Richness (AROnto), which means the attributes and axioms defined in each class are relatively insufficient. The low score for Reliability and Compatibility is mainly caused by the metric M3-Depth of subsumption hierarchy (DITOnto). Some classes defined by Brick are relatively nested.

\item In RECore, 4 of 7 characteristic scores are equal to or above the Acceptable level (4). They are Structural (4.25), Functional Adequacy (4.41), Maintainability (4.04), and Operability (4.33). However, the characteristic scores of Transferability (3.75), Reliability (3.12), and Compatibility (3.50) are at the Minimally Acceptable level (3). The low score is due to the sub-characteristics Adaptability (T-A), Recoverability (R-R), Availability (R-A), and Replaceability (C-R) mainly affected by the metrics M1-Lack of Cohesion in Methods (LCOMOnto), M2-Weighted Method Count (WMCOnto), and M3-Depth of subsumption hierarchy (DITOnto). Interestingly, the low scores for LCOMOnto and WMCOnto also indicate the average depth of classes in RECore is even deeper than Brick. However, this does not affect the characteristic of Functional Adequacy in RECore because it is neutralised by the high score of the metric M12-Attribute Richness (AROnto).

\item In Haystack, 6 of 7 characteristic scores are equal to or above the Acceptable level (4). In particular, 3 characteristic scores of Structural (4.75), Maintainability (4.48), and Operability (4.67) reach a higher score and are close to 5. This means the ontology design of Haystack is easy to maintain and operate. Similar to Brick, the low score for Functional Adequacy is affected by the metric M12-Attribute Richness (AROnto), which means the attributes and axioms defined are relatively insufficient.

\item In DB, 3 of 7 characteristic scores are equal to or above the Acceptable level (4). They are Structural (4.25), Functional Adequacy (4.04), and Operability (4). The other 3 characteristic scores of Maintainability (3.56), Transferability (3.25), and Compatibility (3.25) are at the Minimally Acceptable level (3); in particular, the score of Reliability (2.88) is below the Minimally Acceptable level (3). It is caused by the low scores of the metrics M1-Lack of Cohesion in Methods (LCOMOnto), M2-Weighted Method Count (WMCOnto), and M3-Depth of subsumption hierarchy (DITOnto). DB commonly uses the delimiter ``\_'' to separate the class name into several components in line with the original design of the BMS, but it also results in a deeper hierarchy. For example, the equipment class Multi-directional Shade (East and Southeast) (\url{http://www.google.com/DB/0.0.1/hvac#Sdc_ext_tlt_east_southeast}) has a depth of 7 (EntityType-$>$Equipment-$>$Sdc-$>$Sdc\_ext-$>$Sdc\_ext\_tlt-$>$Sdc\_ext\_tlt\_east-$>$Sdc\_ext\_tlt\_east\_southeast).

\end{enumerate}

\paragraph{Summary}

The TBox evaluation shows Haystack and Brick perform better than RECore and DB on the assessed metrics. This is because Haystack and Brick tend to be wide class hierarchies, while RECore and DB tend to be deep class hierarchies. Ontology is defined as ``a formal specification of a conceptualisation". It abstracts the concepts and their relations to merge, share, and reuse presented knowledge or deduce facts that do not exist in the knowledge base~\citep{gruninger1995methodology}. In this setting, the design of the ontology should not only aim for high coverage of the knowledge (i.e., completeness and expressiveness) but also target efficiency by minimising the classes, properties, and axioms used, and avoiding redundant definitions and an excessively deep class hierarchy, so that it can be easily used for querying and reasoning. Ideally, an ontology that scores well on TBox metrics is more compact. This is useful for applications where querying and inferencing are simple, or for IoT devices with limited data transfer capacity. We also find the following implications:

\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item Although the ontological representation of the building data helps with the Structural (S) and Operability (O), all four building ontologies observe a relatively deep and nested class hierarchy. This affects the Functional Adequacy (F) of the ontology, as well as the capabilities of Maintainability (M), Transferability (T), Reliability (R), and Compatibility (C).
\item The use of attributes and properties (usually observed in ontologies with deep class hierarchies) could help with the Functional Adequacy (F), but it also has negative impact on the Maintainability (M), Transferability (T), Reliability (R), and Compatibility (C). The complexity of the ontology class definitions makes it hard to maintain and exchange data between different building ontologies.
\item The use of subclasses and annotations (usually observed in ontologies with wide class hierarchies) could help with the Maintainability (M), Transferability (T), Reliability (R), and Compatibility (C). Such a design makes it easier to discover the nested classes, while querying and inferring the facts in the ontology may have some issues with the Functional Adequacy (F). The fact that simple ontology design decisions have mutually contradictory effects on metrics demonstrates the difficulty of balancing competing needs for creators and users of models.
\end{enumerate}

\subsection{The ABox Evaluation of Building Ontologies}

\paragraph{Concept Evaluation}

\paragraph{Building Spaces}

A building space is characterised as a contiguous part of the building with a 3D spatial extent. It can be bound physically or conceptually. An example of a building space is described as follows: \textit{``Building 003, located on the South East Precinct Site 01, is an office building with a wing Building 001. Outside the building, there is a barbeque area and surface parking. The building has three floors: Basement, Ground Floor, and First Floor. The library (Room G.13) is on the Ground Floor. It is located to the south of the restroom (Room G.14), east of the hallway (Room G.18), and opposite to the electrical room (Room G.18a). These four rooms belong to HVAC Zone G1.''} Figure~\ref{fig: building spaces} shows the model for the building spaces of our use case in each of the four ontologies.

\begin{figure*}[!hbt]
\centering
\includegraphics[width=1\linewidth]{qiang-eb-2023-figures/Building_Spaces.jpeg}
\caption{Comparison of four building ontologies representing building spaces. \href{https://ars.els-cdn.com/content/image/1-s2.0-S0378778823002840-gr7.jpg}{[Link to the full-size image]}}
\label{fig: building spaces}
\end{figure*}

\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item There are different terms referring to the building spaces in the four ontologies investigated. In Brick and RECore, building spaces are categorised into \textit{Location} and \textit{Space}, respectively. The spatial information of Haystack is classified into \textit{site} and \textit{space}. DB separates the definition of building spaces into two classes: \textit{PhysicalLocation} (physical spaces) and \textit{Zone\_hvac} (logic spaces).
\item All of the four building ontologies are able to capture the basic concepts of building spaces, such as buildings, floors, rooms, and HVAC zones. Nevertheless, they have different levels of expressiveness in representing the building-related artifacts. Brick could capture the concepts of the region, site (land) and outdoor area (outside), while the concept of the outdoor area (outside) is missing in RECore. Haystack and DB assume one building per site (although Haystack has a site class, it is defined as one building with its own unique street address). They cannot describe the spatial information related to region, site (land), and outdoor area (outside).
\item These concepts are linked by part-whole relationships. The part-whole relationship can be made and maintained once and reused plenty of times. For example, the floor is a part of the building, the room is a part of the floor, and the room is a part of the HVAC zone, etc. This idea was introduced in BOT~\citep{rasmussen2017proposing}. In Brick and RECore, the transitive property \textit{hasPart} is used. In Haystack, two inverse properties \textit{siteRef} and \textit{spaceRef} are defined. Unlike other ontologies, DB has one property \textit{hasPhysicalLocation}, and two sub-properties \textit{hasFloor} and \textit{hasRoom}. Note that no appropriate properties can be found to describe the relationship between logic zones in DB.
\item The functions of a room are expressed at different abstraction levels in the four building ontologies. Brick and RECore specify the room functions by defining new classes and subclasses for each function. In contrast, Haystack and DB only provide the general class \textit{Room}. Categories are not used in any of the ontologies.
\item All of the four building ontologies have limited expressiveness in representing the geometry of the building space (e.g. sizes, shapes, positions, angles, and dimensions) and topological connections between the building spaces (e.g. contain, adjacent, and intersect). Only RECore provides some limited functions to represent the geometry using the class \textit{geo:Geometry} and property \textit{geo:hasSerialization} from GeoSPARQL~\citep{battle2011geosparql}. It is possible to link building ontologies to BOT~\citep{rasmussen2021bot} and GeoSPARQL~\citep{battle2011geosparql}.
\end{enumerate}

\paragraph{Building Equipment and Systems}

Building equipment refers to devices that are (semi-) permanently mounted or installed in a building space, and measure, transport, or transform either materials or energy across the whole or part of the building. A system is a collection of equipment. An example of equipment and its related systems is described as follows: \textit{``AHU G1 is located in the service room (B.16) and feeds air to HVAC Zone G1. The basic components of the AHU G1 are the outside damper, return damper, filter, heating valve, cooling valve, heating coil, cooling coil, and supply fan. The AHU comprises the air system and is connected to the water system. The air system contains outside damper, return damper, filter, heating coil, cooling coil, and supply fan. In a ventilation mode, outside air and return air are passed into the ventilation air system through the outside dumper and return dumper. Then, the mixed air goes through the filter and turns into the supply air. After that, air goes through the heating coil and cooling coil (to heat or cool the air if necessary), and finally, the supply fan feeds the supply air to the HVAC Zone G1. The hot water system comprises boiler, hot water pump, heating valve, and heating coil. The supply of hot water comes from the boiler via the hot water pump. It flows through the valve and coil. The valve also modulates the flow depending on the required load (the description of the chilled water system is omitted, similar to the hot water system).''} Figure~\ref{fig: equipment and system (a)} and Figure~\ref{fig: equipment and system (b)} show the model for the building equipment and systems of our use case in each of the four ontologies.

\begin{figure*}[!hbt]
\centering
\includegraphics[width=1\linewidth]{qiang-eb-2023-figures/Equipment_and_Component.jpeg}
\caption{Comparison of four building ontologies representing building equipment and systems (a). \href{http://ars.els-cdn.com/content/image/1-s2.0-S0378778823002840-gr8.jpg}{[Link to the full-size image]}}
\label{fig: equipment and system (a)}
\end{figure*}

\begin{figure*}[!hbt]
\centering
\adjustbox{max width=\linewidth,valign=m}{\includegraphics{qiang-eb-2023-figures/System_and_Substance.jpeg}}
\vspace{-0.4cm}
\caption{Comparison of four building ontologies representing building equipment and systems (b). \href{https://ars.els-cdn.com/content/image/1-s2.0-S0378778823002840-gr9.jpg}{[Link to the full-size image]}}
\label{fig: equipment and system (b)}
\end{figure*}

\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item The classes used to describe the equipment in the four building ontologies are effectively equivalent. Some domain ontologies use the synonym \textit{Device}, but these four building ontologies all use the term \textit{Equipment}. Only Brick and RECore have the definition of the \textit{System}. Brick also defines \textit{Loop} to describe a collection of connected equipment, such as the air loop and water loop. This class is useful when it comes to primary and secondary loops in air and water systems (an example is shown in Figure~\ref{fig: system and loop}). Collection classes are not fully implemented in Haystack and DB, including systems and loops.

\begin{figure}[!hbt]
\centering
\includegraphics[width=1\linewidth]{qiang-eb-2023-figures/System_and_Loop.jpeg}
\caption{An example of system and loop in Brick.}
\label{fig: system and loop}
\end{figure}

\item Brick and Haystack do not have a classification for equipment and sub-equipment. RECore and DB use the \textit{Component} class to describe the sub-equipment, a part of the equipment. In this setting, equipment is mechanical or electrical devices that are functionally independent, while sub-equipment (i.e., component) is manufactured objects that are functionally dependent. For instance, Fan is equipment, but HVAC Fan is a component because it usually works with other building parts.

\item Equipment and system are linked by part-whole and feeds relationships. Some of the documented connection properties in DB are not fully implemented in the ontology at the time of writing. The selection of a relationship property depends on the type of connection between two objects. A logical connection uses the \textit{part-whole} relationship, while a physical connection uses the \textit{feeds} relationship. A physical connection is tangible, where one thing connects to another through piping, wiring, or other similar pathways. Physical connections are built to transmit substances. For example, the connection between the filter and the heating or cooling coil within an AHU is a physical connection. They are connected through a duct, and the air is transmitted between these two objects. The logical connection is intangible and represents an abstract concept or topology of the network. For instance, the connections between the AHU and filter, or between the AHU and heating or cooling coil, are logical connections because the filter and heating or cooling coil are parts of the AHU. Uniquely, Haystack uses reference objects to classify physical and logical connections. \textit{airRef}, \textit{hotWaterRef}, and \textit{chilledWaterRef} are physical connections, whereas \textit{equipmentRef} is used for logical connections.

\item The four building ontologies provide different levels of detail to describe feeds relationships. Rather than using plain \textit{feeds}, the predicates used in Haystack are \textit{airRef}, \textit{chilledWaterRef} and \textit{hotWaterRef}. Unlike Haystack, the property \textit{feeds} in Brick only has one sub-property \textit{feedsAir}, while RECore and DB do not have any sub-properties under \textit{feeds}.

\item It is hard for users with limited engineering knowledge to determine whether a connection is physical or logical. We found an easy way to distinguish the types of connections by using a discrete definition of equipment and component. Connections within the category (equipment and equipment, component and component) are physical (i.e., use \textit{feeds}, \textit{airRef}, \textit{hotWaterRef}, and \textit{chilledWaterRef}), while the connections across dissimilar categories (equipment and component) are logical (i.e., use \textit{hasPart} and \textit{equipmentRef}) in common.

\item All four building ontologies agree that equipment can simultaneously have two linked properties to the building space. The reason is that equipment can be located in one place but feeds into another place or HVAC zone. In our case, AHU G1 is located in the service room (B.116) but feeds the air to Zone G1, an HVAC zone on the Ground Floor.

\item The four building ontologies use different approaches to list substances. Brick and Haystack define new classes and subclasses. RECore uses enumerated individuals, while DB only provides general classes such as \textit{Air} and \textit{Water}. QUDT~\citep{hodgson2011qudt} has a finite list of qualities and could provide a way to ensure the completeness and expressiveness of the substances.

\item Regarding the properties used to link equipment and substances, the four building ontologies also provide different levels of detail. Brick and Haystack have a classification of input and output substances by using the properties \textit{hasInputSubstance} (\textit{input}) and \textit{hasOutputSubstance} (\textit{output}). RECore only has a general \textit{Substance} class. For DB, no appropriate input and output properties can be found.

\end{enumerate}

\paragraph{Building Points and Measurements}

Building points refer to sensors or actuators embedded in a building entity (i.e., a building space, equipment, or system). They can be extended to setpoints, states, commands, or parameters of an entity that produce or ingest data. Building points are the points of measurable telemetry and actuation, and measurements usually include the subject, the quantity of the subject, and the unit of measurement. An example of building points and measurements of the air temperature is described as follows: \textit{``AHU G1 feeds air to HVAC Zone G1. To have better control of the air temperature, there are four types of IoT data stored in the DCH database for review and analysis. The system enables status to track the current state of the AHU G1, i.e., whether the AHU G1 is on or off. The supply air temperature sensor is embedded in the AHU G1 and measures the supply air temperature. There are two points located in HVAC Zone G1. The zone air temperature setpoint indicates the desirable setting of the air temperature within the zone, whereas the zone air temperature sensor records the real-time temperature of the zone air.''} Figure~\ref{fig: building points and measurements} shows the model for the different building points and measurements of our use case in each of the four ontologies.

\begin{figure*}[!hbt]
\centering
\includegraphics[width=1\linewidth]{qiang-eb-2023-figures/Building_Points_and_Measurements.jpeg}
\caption{Comparison of four building ontologies representing building points and measurements. \href{https://ars.els-cdn.com/content/image/1-s2.0-S0378778823002840-gr11.jpg}{[Link to the full-size image]}}
\label{fig: building points and measurements}
\end{figure*}

\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item Among the four building ontologies, there are conflicts in the definition of building points. Brick and Haystack use the \textit{Point} class and the \textit{hasPoint} property. They define building points as measurable data points embedded in building spaces, equipment, and systems that produce and ingest data. RECore, however, uses a \textit{Capability} class and the \textit{hasCapability} property. The reason is that building points provide the capability for an entity to produce or ingest data. Depending on the functions and behaviours, building points can be specialised into different categories. DB defines building points as a field belonging to an entity.

\item There are also dissimilarities in defining the subclasses under \textit{Point} or \textit{Capability}. DB defines each point as a field, a self-descriptive object that consists of a string of subfields, for example, \textit{zone\_air\_temperature\_sensor}. Other ontologies categorise points by their functions. Haystack only has three types of building points: \textit{cmd} (command), \textit{sensor}, and \textit{sp} (setpoint). In Brick and RECore, point types also include the system state (status) and system parameters.

\item In our case, the time-series data is stored in the DCH database. Only Brick provides such a function to store the time series ID in the ontologies and allow the full dataset to be stored independently outside the ontology. This not only reduces the size of the ontology but also enables better management of the time-series data in a proper time-series database. RECore, Haystack, and DB do not have the definition of \textit{Database} and only provide one option to store time-series data directly on the knowledge graph itself.

\item A generic measurement of building points includes \textit{Building\_Point}, \textit{Observation}, \textit{Observable\_Property}, and \textit{Feature\_Of\_Interest}, as described in SSN~\citep{compton2012ssn} and SOSA~\citep{haller2019modular}. Their relationships are shown in the middle of Figure~\ref{fig: building points and measurements}. As an example, consider measuring zone air temperature. The building points are the zone temperature sensor, the observation is time-series data, the feature of interest is the zone air, and the observable property is the temperature. None of the four building ontologies could capture all the basic components of the measurement. All of them are missing or partially missing the links between \textit{Observation} and \textit{Observable\_Property} (i.e., \textit{observedProperty}), and between \textit{Feature\_Of\_Interest} and \textit{Observable\_Property} (i.e., \textit{hasProperty}). Other properties can find equivalent properties in the four building ontologies. In Brick, the property \textit{measures} is roughly equivalent to \textit{observes} and \textit{hasFeatureOfInterest}. Equivalent properties found in RECore is \textit{observes}. Besides the equivalent properties \textit{pointQuantity} and \textit{pointSubject}, Haystack also uses a property \textit{pointFunction} to specify the point functions.

\item All the equivalent classes of \textit{Observable\_Property} and \textit{Feature\_Of\_Interest} in the four building ontologies are bound to quantities and substances only. As a result, they have limitations in representing the system status (state) or setpoint. In RECore, the domain of the property \textit{observes} is the \textit{Sensor} class only. There are no appropriate properties that can be used for other types of points. In DB, this part is still under development, and related properties are missing.

\item The four building ontologies use two different approaches for the unit of measurement. Brick and RECore reuse the QUDT~\citep{hodgson2011qudt} \textit{Unit} class and its subclasses, while Haystack and DB use the enumerated individuals and list all the possible units within the ontology.

\end{enumerate}

\paragraph{Use Case Evaluation}

\paragraph{Energy Audits}

The use case evaluation is based on competency questions retrieved from application-level scenarios. We apply the four building ontologies to the use case and compare their completeness and expressiveness, i.e., how many competency questions can be answered and how well these questions are answered. Note that we set the answers for these competency questions into three categories, and ``Partially Answered'' is a medium between ``Fully Answered'' and ``Unable to Answer''. It means that only part of the information can be found, or that the answers are not explicit but implicit.

An energy audit is the assessment of total energy usage across electricity, water, and gas in a smart building and its energy-consuming systems~\citep{krarti2020energy}. The use of building ontologies enables auditors to query and retrieve the required sampling data. According to ASHRAE Standard 211~\citep{ASHRAE211}, energy audits can be performed at one of three levels: Level 1 (walk-through audit), Level 2 (detailed energy audit), and Level 3 (investment-grade audit). Each level covers the requirements of the previous level and includes additional information. We perform a Level 2 energy audit.

Table~\ref{tab: energy audits competency questions} summarises the examples of competency questions and how well each building ontology can potentially answer these questions. Details of the use case evaluation can be found in~\ref{appendix: competency questions in energy audits}. In this use case, Brick and RECore's full and partial answers add up to 18/20, followed by Haystack (16/20) and DB (2.5/20). The main limitations of the building ontologies lie in the lack of building layout presentation (i.e., geometry and floor area). This also impacts the space function breakdown related to energy use and savings. Moreover, Haystack and DB do not specify the space, equipment, and system type, which makes it hard to determine the systematic composition and restricts their use in energy audits.

\begin{sidewaystable*}
\caption{Energy Audits - The examples of competency questions answered by four building ontologies.} 
\label{tab: energy audits competency questions}
\begin{adjustbox}{width=1\linewidth,center}
\begin{tabular}{|c|l|cccc|}                            \hline
Concepts                                & Examples of Competency Questions  & B   & R   & H   & D       \\ \hline
\multirow{5}{*}{\makecell{Building Spaces}}        
                                        & \#01: What is the primary use of the building? If multiple uses, what is the fraction of floor area for each use?  
                                        & \halfcirc  & \halfcirc & \halfcirc  & \emptycirc  \\
                                        & \#02: What are the HVAC zones and their respective air-conditioned areas in the building?    
                                        & \fullcirc  & \fullcirc & \fullcirc & \halfcirc  \\
                                        & \#03: What are all the rooms and their floors in the building? 
                                        & \fullcirc  & \fullcirc & \fullcirc & \halfcirc  \\
                                        & \#04: What is the function type of each room?   
                                        & \fullcirc  & \fullcirc & \halfcirc  & \halfcirc   \\ 
                                        & \#05: What is the occupancy of each room?                             
                                        & \fullcirc & \fullcirc & \fullcirc  & \emptycirc   \\ \hline
 \multirow{6}{*}{\makecell{Building Equipment \\ \&  Systems}}  
                                        & \#06: What are the pieces of equipment and systems of equipment in the building?                                   
                                        & \fullcirc  & \fullcirc & \halfcirc  & \halfcirc   \\
                                        & \#07: What are the properties (e.g. type, physical location and functional area) of each piece of HVAC equipment?                                         
                                        & \fullcirc  & \fullcirc & \fullcirc & \halfcirc  \\
                                        & \#08: What are the components of each piece of equipment and their structural relations?   
                                        & \fullcirc  & \fullcirc & \fullcirc  & \emptycirc  \\
                                        & \#09: What is the energy use broken down by resource using the energy?               
                                        & \fullcirc  & \halfcirc & \halfcirc & \emptycirc  \\
                                        & \#10: What is the energy use broken down by end-use?
                                        & \fullcirc  & \fullcirc & \halfcirc & \emptycirc  \\
                                        & \#11: What are the energy-generating pieces of equipment in the building?                         
                                        & \halfcirc  & \fullcirc & \emptycirc & \emptycirc  \\ \hline
\multirow{5}{*}{\makecell{Building Points \\ \& Measurements}} 
                                        & \#12: What are the meters and meter types in the building?                              
                                        & \fullcirc  & \fullcirc & \fullcirc  & \emptycirc   \\
                                        & \#13: What does each meter measure (i.e., substance and quantity)?   
                                        & \halfcirc  & \halfcirc & \fullcirc  & \emptycirc  \\
                                        & \#14: What are the connections between meters and sub-meters?           
                                        & \halfcirc  & \halfcirc & \fullcirc & \emptycirc  \\ 
                                        & \#15: What are the operating parameters of each piece of equipment (e.g. setpoints and schedules)?  & \fullcirc  & \fullcirc & \fullcirc  & \emptycirc   \\
                                        & \#16: What are the time series for each meter?      
                                        & \fullcirc  & \fullcirc & \halfcirc  & \emptycirc   \\ \hline
\multicolumn{6}{c}{B - Brick, R - RECore, H - Haystack, D - DB}               \\
\multicolumn{6}{c}{\fullcirc~- Fully Answered, \halfcirc~- Partially Answered, \emptycirc~- Unable to Answer}
\end{tabular}
\end{adjustbox}
\end{sidewaystable*}

\paragraph{Summary}

The ABox evaluation shows that Brick and RECore potentially outperform Haystack and DB. From a holistic view, Brick and RECore tend to use an extensible class hierarchy to define specific types of building entities, while Haystack and DB usually only define general classes, properties, and instances. For example, the \textit{Room} class in Brick and RECore contains multiple subclasses to distinguish the room type, such as office room, conference room, and rest room. Conversely, Haystack and DB only define one general class \textit{Room}, and the room function is not detailed. This design pattern is common and can be observed in the descriptions of the building entities among all three main concepts. However, there are some exceptions. Haystack and DB also provide more detailed and specific taxonomies for classifying the sensors. In Haystack, the sensor type can be explicitly inferred by the substance (property \textit{pointSubject}) and quantity (property \textit{pointQuantity}) it measures. DB uses the delimiter ``-'' to separate the sensor’s name into several components, and these components are meaningful and may indicate its function (\textit{supply\_air\_temperature\_sensor}). We also find the following implications:

\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item On a macro level, there are well-agreed design patterns observed in building spaces, equipment, and systems. The four building ontologies use different classes and properties to describe the information related to building spaces, equipment, and systems, but their underlying definitions and axioms are similar.

\item On a micro level, conflicting design patterns appear in the four building ontologies, and they are observed in building points and measurements. The four building ontologies have different classifications of the building points, and use different definitions to illustrate the relationship between building points and building spaces, equipment, and systems (i.e., \textit{hasPoint} and \textit{hasCapability}).

\item Reusing concepts defined in existing ontologies is better for interoperability and usability than creating new ones from scratch. We recommend reusing the concepts defined in BOT~\citep{rasmussen2021bot} and GeoSPARQL~\citep{battle2011geosparql} to represent spatial information, SAREF~\citep{daniele2015created} and SAREF building extension~\citep{poveda2018extending} to represent equipment and systems, SSN~\citep{compton2012ssn} and SOSA~\citep{haller2019modular} to represent sensors and actuators, and QUDT~\citep{hodgson2011qudt} for corresponding measurements. These domain ontologies are usually more complete and expressive than the ones created locally in the building ontologies~\citep{lbd2023}.

\end{enumerate}

\section{Discussion}

There is no universal building ontology that always performs best and fits all the task requirements. In other words, the no free lunch (NFL) theorem~\citep{wolpert1997no} also applies to ontology design for smart building applications. Referring to our study, each building ontology has its pros and cons and achieves different levels of abstraction. We believe there is no context-independent reason to favour one building ontology over another. When we claim one building ontology is better than another, it is not because of its inherent features, but because of its better fitness for the task requirements. However, as a complement to NFL, comparing and evaluating building ontologies through qualitative and quantitative analysis can be a good reference for determining which building ontology to use.

In this study, we compare and evaluate four popular building ontologies with respect to both TBox and ABox components. In the TBox evaluation, we apply the OQuaRE Framework to evaluate the axiomatic design of the building ontologies. The results indicate that Haystack and Brick are better than the other two building ontologies with respect to efficiency and compactness. In the ABox evaluation, we apply four popular building ontologies to a specific building case study to conduct a fair comparison. We evaluate three main concepts: building spaces, equipment and systems, and points and measurements. For each concept, we compare and analyse the four building ontologies representing the same use case. We also use a real-world application, energy audits, to evaluate completeness and expressiveness. The results demonstrate that Brick and RECore cover more of the required domain concepts than the other two building ontologies. The conflicting results of the TBox and ABox evaluations reveal that the choice of the ontology modelling and design approach is also context-dependent. Figure~\ref{fig: modelling patterns} shows an overview of the building ontology modelling patterns.

\begin{figure}[!hbt]
\centering
\includegraphics[width=0.6\linewidth]{qiang-eb-2023-figures/Design_Pattern_Modelling.jpeg}
\caption{The overview of building ontology modelling patterns.}
\label{fig: modelling patterns}
\end{figure}

\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item Haystack and Brick are modelled as ontologies with wider class hierarchies, while RECore and DB are modelled as ontologies with deeper class hierarchies. An ontology with a wider class hierarchy usually has a relatively large number of direct subclasses with a higher Relationship Richness (RROnto). This kind of ontology usually has high concept coverage and compatibility (i.e., constructional efficiency), but keeping the consistency of axioms defined in multiple classes is problematic and affects its functional adequacy. Conversely, an ontology with a deeper class hierarchy is an ontology where classes have a relatively small number of direct subclasses, use properties and attributes more often, and have a higher Properties Richness (PROnto). An ontology with a deeper class hierarchy has low coupling and cohesion (i.e., functional efficiency), but this may affect the discoverability of the classes, and it is not easy to maintain and exchange the data with other ontologies in such an ontology design.

\item RECore and Brick are aimed towards specific detail modelling, while Haystack and DB are aimed towards generic modelling. Generic modelling with no detailed information is more flexible in composing queries and can have small effects on reducing the query execution time. Still, it encapsulates or implies the properties with idioms and usually needs to be supplemented with specific ontologies to describe more specific features where necessary. For example, generic classes can be supplemented with additional metadata on instances to embody information. On the other hand, specific modelling with detailed information aids in discoverability and ease of use for modellers. It is easier to classify an object type if there is already a suitable predefined class, though this can mean more work to maintain such a complex and specific ontology.

\item Based on the findings from our evaluation, we also abstract the key concepts and relations that are used in building ontologies. The overall picture of the ontology design patterns (ODPs) for smart building applications and how these building concepts are linked is shown in Figure~\ref{fig: design patterns}. The measurements (Status, Substance, and Unit) are placed in the centroid of the diagram, surrounded by Building Spaces, Building Equipment and Systems, and Building Points. The measurements of building equipment and systems include their status (\textit{hasStatus}), and input and output substances (\textit{hasInputSubstance} and \textit{hasOutputSubstance}). We use \textit{hasStatus}, \textit{hasQuantityKind}, and \textit{hasUnit} to describe the sensory point measurements of the building points. There are two relations between building spaces and building equipment and systems, representing the physical location (\textit{hasLocation}) and functional location (\textit{feeds}) of the equipment, respectively. Building points can be mounted on equipment and systems or directly on the building spaces using \textit{hasLocation}. They are defined as a point or function (\textit{hasPoint}/\textit{hasCapability}) provided by building entities (spaces, equipment, and systems).

\begin{figure}[!hbt]
\centering
\includegraphics[width=0.7\linewidth]{qiang-eb-2023-figures/Design_Pattern_Overview.jpeg}
\caption{The overview of building ontology design patterns.}
\label{fig: design patterns}
\end{figure}

\end{enumerate}

\section{ODPs for Data-Driven Smart Buildings}

Ontology Design Patterns (ODPs) were initially introduced in~\citep{gangemi2009ontology}, aiming to simplify ontology engineering by packaging archetypal solutions into reusable and portable building blocks. The notion of ODPs is to alter ontology engineering to be a composition task with minimal modification, i.e., assembling a collection of reusable ODP implementations and catering to specifics. In this setting, ODPs secure a level of interoperability where data can be integrated. Ontologies that follow the same ODPs have common design choices and inherent points of alignment~\citep{hitzler2016ontology}. Currently, there is a lack of criteria for how existing building ontologies can be reused and re-engineered. The conflicting design rationales, produce a heavy alignment workload to transfer data built by one building ontology to another. ODPs are neither available to the extent required nor are those that are available realised in practice within the smart building domain. Thus, along with this work, we propose building ODPs that mediate between use cases and design solutions.

\subsection{Building Spaces} 

Figure~\ref{fig: design pattern building spaces} shows the ODPs for building spaces. The concepts of building spaces include \textit{Region}, \textit{Site}, \textit{Building}, \textit{Building\_Related}, \textit{Floor}, \textit{Zone}, and \textit{Room}. They are related through part-whole relationships. In an open world assumption~\citep{drummond2006open}, it is impossible to enumerate all types of rooms. Therefore, we use a \textit{Category} class to represent the room functions instead. All these classes are categorised into the \textit{Building\_Space} class. The \textit{Building\_Space} class has two properties: \textit{hasGeometry} and \textit{hasTopologicalRelations}, representing the geometry and topological connections, respectively. The sub-properties of \textit{hasTopologicalRelations} are retrieved and evolved from BOT~\citep{rasmussen2021bot} and GeoSPARQL~\citep{battle2011geosparql}.

\begin{figure}[!hbt]
\centering
\includegraphics[width=\linewidth]{qiang-eb-2023-figures/Design_Pattern_Building_Spaces.jpeg}
\caption{ODPs for building spaces.}
\label{fig: design pattern building spaces}
\end{figure}

\subsection{Building Equipment and Systems}

Figure~\ref{fig: design pattern building equipment and systems} shows the ODPs for building equipment and systems. The concepts of building equipment and systems include \textit{Equipment}, \textit{Component}, \textit{System}, and \textit{Loop}. They are related through part-whole relationships and grouped into the \textit{Building\_Equipment\_And\_System} class. \textit{Equipment} has two properties linked to \textit{Building\_Space}, \textit{hasLocation} and \textit{feeds}. They are used to describe the physical and functional location, respectively. \textit{Equipment} and \textit{Component} have a self-contained feeds relationship, used to describe the physical connection and substance transmission between equipment and equipment, or between component and component. The property \textit{feeds} has two sub-properties: \textit{feedsAir} and \textit{feedsWater}. \textit{feedsWater} is detailed into \textit{feedsHotWater} and \textit{feedsChilledWater}. It can be extended to other substances, such as gas or other liquids. \textit{Substance} is linked to the \textit{Equipment} and \textit{Component} by using the property \textit{hasSubstance}. There are two sub-properties \textit{hasInputSubstance} and \textit{hasOutputSubstance} under \textit{hasSubstance}. We suggest the subclasses under \textit{Substance} reuse QUDT~\citep{hodgson2011qudt} and its qualities.

\begin{figure}[!hbt]
\centering
\includegraphics[width=\linewidth]{qiang-eb-2023-figures/Design_Pattern_Building_Equipment_and_Systems.jpeg}
\caption{ODPs for building equipment and systems.}
\label{fig: design pattern building equipment and systems}
\end{figure}

\subsection{Building Points and Measurements}

Figure~\ref{fig: design pattern building points and measurements} shows the ODPs for building points and measurements. Due to conflicts in defining the building points and properties used, we do not specify the type of the building points, and the properties used to describe the measurement are based on SSN~\citep{compton2012ssn} and SOSA~\citep{haller2019modular}. The property alignment of four building ontologies are listed in Table~\ref{tab: property alignment}. We suggest the subclasses under Substance reuse QUDT~\citep{hodgson2011qudt} and its units.

\begin{figure}[!hbt]
\centering
\includegraphics[width=\linewidth]{qiang-eb-2023-figures/Design_Pattern_Building_Points_and_Measurements.jpeg}
\caption{ODPs for building points and measurements.}
\label{fig: design pattern building points and measurements}
\end{figure}

\begin{table}[!hbt]
\caption{Property alignment of ODPs for building points and measurements.}
\label{tab: property alignment}
\begin{center}
\begin{adjustbox}{width=1\columnwidth,center}
\begin{tabular}{|l|l|l|l|l|}
\hline
ODPs                       & Brick                          & RECore                    & Haystack              & DB\\  \hline
\small madeObservation     & brick:timeseries               & core:generatedObservation & N/A                   & N/A\\ \hline
\small observes            & brick:measures                 & core:observes             & phIoT:pointQuantity   & N/A\\ \hline
\small hasFeatureOfInterst & brick:measures                 & core:observes             & phIoT:pointSubject    & N/A\\ \hline
\small observedProperty    & N/A                            & qudt:hasQuantityKind      & N/A                   & N/A\\ \hline
\small hasProperty         & N/A                            & N/A                       & N/A                   & N/A\\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

There is a slight difference between brick:timeseries and madeObservation/core:generatedObservation. brick:timeseries originally points to a time series reference and indicates where and how the data for this point is stored~\citep{balaji2016brick}. It can contain multiple observations for a particular period of time. However, madeObservation/core:generatedObservation only refers to one observation for a particular period of time.

\section{Conclusions}

This chapter compares and evaluates building ontologies for deploying data-driven analytics in smart buildings. The TBox and ABox characteristics of four major building ontologies are compared and evaluated. We also systematically analyse the compatibility between ontologies, and the common and conflicting ontology modelling and design patterns discovered from the study. Since the Brick, RECore, and Haystack designers now plan to align their future developments, we hope the present work will be useful to the authors of these ontologies.

While the evaluation conducted in this study is based on an office building, future work will further the comparison with respect to the capability of extension to other building types, such as commercial and residential buildings. We also plan to apply the comparison and evaluation to more building ontologies to discover solid and generic ontology modelling and design patterns, and to automate the building ontology matching, alignment, and harmonisation. The Linked Building Data Community Group (LBD-CG)~\citep{lbd2023} has similar aims.

We find that there is no ontology in our study that covers all requirements for our use case out-of-the-box. Nor can we universally declare that any ontology is ``better'' than another, even when using popular quantitative metrics. Each ontology has been designed with particular purposes in mind, and when reusing the ontologies, one designed for the purpose closest to that of the new purpose will almost certainly be the best choice~\citep{fierro2022survey}. While efforts to harmonise popular ontologies to expand their expressivity for multiple use cases will help in ontology selection, interoperability, and community knowledge sharing, we believe that a universal building ontology is unreachable. Too much complexity in an ontology can be just as damaging as too little. Even when a certain domain is considered entirely dealt with, there will remain issues with interoperability across multiple domains, for example, across buildings and smart cities. These needs for interoperability will emerge and evolve as the fabric of society evolves, and we must accept that dynamicity is here to stay. In this scenario, the ontology design and modelling patterns we have found in this work can be used as a skeleton to evolve current building ontologies and develop new building ontologies. They can also be used as a guideline to develop alignments for translation between ontologies. We propose to automate the process of pattern discovery as a key element of ontology alignment, integration, and harmonisation activities going forward. The need for these activities will endure and require ongoing research to develop sound and efficient tool support.

In the next chapter, we will focus on the first of these, ontology alignment by ontology matching.

\paragraph*{Supplementary Material Statement}

The source code, data, and/or other artifacts used in this study are available at \url{https://github.com/qzc438/Building-Ontology-Comparison-and-Evaluation} (access will be made available on request).

\paragraph*{Publication Statement}

Most of the work presented in this chapter has been published as~\bibentry{qiang2023systematic}.

==> qiang-anu-thesis-content/ockgs.tex <==
\chapter{Ontology-Compliant Knowledge Graphs}
\label{chap: ockgs}

Ontologies can act as a schema for constructing knowledge graphs (KGs), offering explainability, interoperability, and reusability. We explore \emph{ontology-compliant} KGs, aiming to build both internal and external ontology compliance. We discuss key tasks in ontology compliance and introduce our novel term-matching algorithms. We also propose a \emph{pattern-based compliance} approach and novel compliance metrics. A case study in the building sector is used to test the validity of ontology-compliant KGs. We recommend using ontology-compliant KGs to pursue automatic matching, alignment, and harmonisation of heterogeneous KGs.

An ontology is typically used as the backbone for constructing a KG, building so-called \emph{ontology-based KGs}. In this setting, the ontology and the KG are often treated as separate functional components. An ontology provides a knowledge-oriented graph schema (i.e. TBox), whereas a KG represents the corresponding data-driven instances (i.e. ABox).

With the proliferation of KGs in real-world applications, problems arise when data in the KG is generated for different user requirements. The ontology is likely to be incompatible with the data in the KG because ABox assertions may extend or be incomplete with respect to the ontology. While ABox contents can be adapted to suit a TBox, for interoperability amongst independent TBoxes, an ABox that is compatible with a number of TBoxes may be needed. Such overarching TBoxes should support conversion and exchange for cross-KG harvesting and federated searches.

Figure~\ref{fig: ontology and KG} illustrates three types of non-compliance between a KG and its ontology. (1) The ABox in the KG only refers to a few TBox terms, so its ontology has many unused classes and properties. (2) The ABox in the KG contains more information than the TBox terms, so many terms in the KG do not have corresponding named classes and properties in its ontology. (3) In a combination of (1) and (2), the ABox in the KG and the TBox in the ontology are mismatched and overlapped on both sides. Many application tasks, for example, KG embedding and ontology learning, are hampered by non-compliance between a KG and its ontology. When using KG embedding for ontology-based KGs, unused classes and properties in the ontology are noisy data. This results in inaccurate embeddings for KG terms. Ontology learning is the task of using KG to infer ontology classes and properties. KG data is diverse in nature; thus, the new ontology classes and properties learnt from a KG can differ according to KG training instances. These task-specific ontology classes and properties may violate the FAIR principles (i.e. Findable, Accessible, Interoperable, and Reusable) and can be challenging to map and integrate into the original ontology.

\begin{figure}[htbp]
\centerline{\includegraphics[width=1\linewidth]{qiang-eswc-2023-figures/Ontology-KG-Mismatching.png}}
\caption{Non-compliance between a KG and its ontology.}
\label{fig: ontology and KG}
\end{figure}

Current work mainly focuses on either schema matching (i.e. TBox-TBox compliance) or instance matching (i.e. ABox-ABox compliance). TBox-ABox compliance is underexplored. While it is questionable whether the TBox is always compliant with the ABox, ontology-based KGs assume they are compliant by nature and so exclude or ignore the three types of non-compliance. For this reason, there is rarely a compliance check in popular KG and ontology modelling libraries or editors (e.g. RDFLib~\citep{boettiger2018rdflib}, Protégé~\citep{musen2015protege}, and TopBraid Composer~\citep{topbraid2022}). Even within the Ontology Alignment Evaluation Initiative (OAEI)~\citep{oaei}, to the best of our knowledge, there are no tools available to track these mismatches and overlaps between ABox in the KG and TBox in its corresponding ontology.

\section{Related Work}

\textbf{Ontology-Based KGs} describe the traditional design for using ontologies with KGs, whereby the ontology serves as the schema for the KGs. KGs are generated using the classes and properties pre-defined in the ontology. In this setting, ontology-based KGs assume the ontology has established well-defined concepts, taxonomies, relationships, and domain axioms. Compared with ontology-less KGs, ontology-based KGs provide more formal representations for data understanding, organisation, and integration. They also enable improved logical reasoning, empowered reuse, and enhanced interoperability between different downstream applications. However, a complete ontology is almost impossible. Ontologies are built on the Open World Assumption (OWA). We cannot assume an ontology has captured all domain concepts because the absence of concepts is not interpreted as non-existence (i.e. these concepts may exist in other ontologies). A ``well-defined'' ontology also requires solid verification and validation. There is no gold standard for dealing with individual differences among opposing viewpoints.

\noindent\textbf{Ontology-Aware KGs} follow a reverse way of using ontologies with KGs. Conceptual components learnt from KGs are used to build or evolve the original ontology. The paradigm of ontology-aware KGs assumes the KG data is correct. There are two directions for constructing ontology-aware KGs. (1) Ontology reshaping is applied to data in the KG that only refers to parts of the concepts in the ontology. The goal of ontology reshaping is to create a data-oriented local schemata that preserves the domain ontology knowledge while removing unused nodes~\citep{zhou2022enhancing,zhou2022ontology}. (2) Ontology enrichment is used where data exists in the KG that is not covered by the ontology. In this case, the new concepts and relationships learnt from the KG are registered as new classes and properties in the ontology~\citep{hurlburt2021knowledge,zhao2019learning}. While ontology-aware KGs achieve partial compliance between the KG and its ontology, they still have some limitations. Concepts that have been locally reshaped and redefined are task-specific, with limited sharing and reusing capabilities. Moreover, ontology-aware KGs cannot track the poly-ontological representation of KGs as they only match one KG to one corresponding ontology.

\section{Problem Statement and Contributions}

In practice, KGs and ontologies are mostly incomplete. Neither ontology-based KGs nor ontology-aware KGs could fully handle the compliance issue between KGs and ontologies. We propose \textbf{Ontology-Compliant KGs} to fill this gap. ``Compliant'' here has two aspects: (1) The terms used in KG are in line with the definition provided by the ontology. Mismatched terms in the KG are replaced with the most relevant classes and properties defined in the original ontology. (2) The size of the ontology complies with the information coverage of the KG. There are no unused classes or properties. In this work, we also extend this definition to be ontology compliant across KGs. Joint learning, vector embedding methods, and pattern-based engineering concepts are employed to achieve the goal of both internal and external compliance between KGs and ontologies. Figure~\ref{fig: ontology-type-KGs} shows the difference between ontology-compliant KGs and the other two types of ontology-related KGs. While ontology-based and ontology-aware KGs only consider a one-way connection, in ontology-compliant KGs, the link between ontology and KG is bidirectional and can be bridged by their patterns (details are described in Section~\ref{sec: results}).

\begin{figure}[htbp]
\centerline{\includegraphics[width=1\linewidth]{qiang-eswc-2023-figures/Ontology-Type-KGs.png}}
\caption{Comparison of ontology-compliant KGs and the other two types.}
\label{fig: ontology-type-KGs}
\end{figure}

Ontology-compliant KGs have the following unique features:

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item Given an ontology and a baseline KG, ontology-compliant KGs can eliminate the unused classes and properties in the ontology and reduce misdefined terms in the KG (interpreted as Ontology Compliance \emph{within} KG).
\item Given a set of ontologies and a baseline KG, ontology-compliant KGs allow automatic transmission from one schema to another (interpreted as Ontology Compliance \emph{over} KGs).
\item Given a set of ontologies and a baseline KG, ontology-compliant KGs allow different ontology fragment representations via a pattern-based approach. These ontology fragments are provided with multiple criteria for integration, evaluation, and selection (interpreted as \emph{Pattern-based} Compliance).
\end{enumerate}

\section{Evaluation}

In the context of Industry 5.0 and the Internet of Things (IoT), digitisation and automation are becoming emerging research areas in the building sector. While a number of building and building-related ontologies have been developed, data interoperability issues have become more apparent. Different building ontologies are developed and maintained by different institutions. These ontologies are modelled at multiple levels of abstraction for various purposes, and their definitions are frequently competing and overlapping. Proposed ontology-compliant KGs would potentially help with the unified vision of building ontologies, where the data in this domain has complexity and variety in concepts and relations.

\section{Results}
\label{sec: results}

\subsection{Ontology Compliance within KG}

A KG and its ontology share all terms and topology. However, the concepts and properties defined in KG and ontology can be mismatched due to human errors, design choices, or changes in newer versions. Figure~\ref{fig: within compliance} shows different types of node matching in a snippet of an air handling unit (AHU) system represented by a KG and its ontology Brick Schema~\citep{balaji2016brick} (abbr. ``Brick''). The concepts with green colours are KG classes, while the concepts with yellow colours are ontology classes. Different matching types and their examples are shown in the table below. These also applied to the property matching between KG and its ontology.

We design Algorithm~\ref{alg: within compliance} for building ontology compliance within KG. It has two phases: (1) Entity Alignment and (2) Ontology Reconstruction. We first find non-compliant terms in the KG and replace them with the most relevant classes and properties in the original ontology, assigning a confidence score for each replacement. Then, we find all the related triples (including constraints and axioms) and restore the ontology hierarchies.

\begin{figure}[htbp]
\centerline{\includegraphics[width=1\linewidth]{qiang-eswc-2023-figures/Example-Ontology-Compliance-within-KGs.png}}
\caption{An example of ontology compliance within KG.}
\label{fig: within compliance}
\end{figure}

\begin{algorithm}[htbp]
\scriptsize

\caption{Building Ontology Compliance within KG}
\label{alg: within compliance}
\begin{multicols}{2}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE Ontology-based $KG$, Ontology $Onto$
\ENSURE  Reshaped Onto $Onto_{RE}$, Confidence $\mu$

\STATE \textbf{/* Phase 1: Entity Alignment */}\\
\STATE /* Find all terms in KG */
\STATE Concept Set $Con\_S$, Relation Set $Rel\_S$ $\leftarrow \varnothing$ 
\STATE $ Con\_S,Rel\_S \leftarrow findConceptAndRelation(KG) $

\STATE /* Find all classes and properties in Onto */
\STATE Class Set $Cls\_S$, Property Set $Pro\_S$ $\leftarrow \varnothing$
\STATE $ Cls\_S,Pro\_S \leftarrow findClassAndProperty(Onto) $

\STATE /* Divide each naming into a keyword set */
\STATE $ Con\_S,Rel\_S \leftarrow findKwd(Con\_S,Rel\_S) $
\STATE $ Cls\_S,Pro\_S \leftarrow findKwd(Cls\_S,Pro\_S) $

\STATE /* Match classes between KG and Onto */
\FOR {$ i \in Con\_S $}
\FOR {$ j \in Cls\_S $}
\IF {$ purelyMatching (i,j) \neq \varnothing $}
\STATE $ \mu_i \leftarrow 1 $
\ELSIF {$ heuristicMatching (i,j) \neq \varnothing $}
\STATE $ \mu_i \leftarrow Levenshtein Distance $
\STATE $ Con\_S \rightarrow i \land Con\_S \leftarrow j $
\ELSIF {$ semanticMatching(i,j) \neq \varnothing $}
\STATE $ \mu_i \leftarrow Similarity $
\STATE $ Con\_S \rightarrow i \land Con\_S \leftarrow j $
\ELSIF {$ topologicalMatching(i,j) \neq \varnothing $}
\STATE $ \mu_i \leftarrow Accuracy $
\STATE $ Con\_S \rightarrow i \land Con\_S \leftarrow j $
\ENDIF
\ENDFOR
\ENDFOR

\STATE /* Match properties between KG and Onto */\\
\FOR {$ k \in Rel\_S $}
\FOR {$ l \in Pro\_S $}
\STATE /* Corresponding procedure applies to Rel\_S and Pro\_S */
\ENDFOR
\ENDFOR

\STATE /* Calculate total confidence */
\STATE Total Confidence $\mu$ $\leftarrow \varnothing$ 
\STATE $ \mu \leftarrow Avarage (\mu_1, ..., \mu_i, \mu_1, ..., \mu_k)$

\STATE \textbf{/* Phase 2: Ontology Reconstruction */}\\
\STATE /* Find super-classes */
\STATE $ Onto\_{RE}$ Class Set $ RE\_Cls\_S \leftarrow \varnothing $
\STATE $ RE\_Cls\_S \leftarrow findSuperClasses(Con\_S) $

\STATE /* Find super-properties */
\STATE $ Onto\_{RE} $ Property Set $ RE\_Pro\_S \leftarrow \varnothing $
\STATE $ RE\_Pro\_S \leftarrow findSuperProperties(Rel\_S) $

\STATE /* Restore reshaped ontology */
\STATE Reshaped Ontology $ Onto_{RE} \leftarrow \varnothing $
\STATE $ Onto_{RE} \leftarrow findTriples(RE\_Cls\_S, RE\_Pro\_S) $

~\\

\RETURN $ Onto_{RE},\mu $
 
\end{algorithmic}
\end{multicols}
\end{algorithm}

The experiment uses the sample example from the Brick Schema official website (\url{https://brickschema.org/}). We synthesise a number of mismatched classes and properties with different types. The results in Table~\ref{tab: within compliance} show that reshaped ontologies can significantly reduce the original ontology size and increase the number of used and matched classes. We can also observe a trade-off between the confidence score and the level of matching applied. The confidence score slightly decreases when the level of matching increases. A potential reason is that Level 3 and Level 4 use learning-based approaches. While they are more powerful at discovering more pairs of matches, the confidence level of the matching accuracy highly depends on the models and methods used.

\begin{table}[htbp]
\renewcommand\arraystretch{1.2}
\tabcolsep=0.15cm
\caption{Evaluation of algorithm for building ontology compliance within KG.}
\label{tab: within compliance}
\begin{adjustbox}{width=1\linewidth,center}
\begin{tabular}{|r|c|c|c|}\hline
 Type of Ontology \& Matching Level     & Used Entity   & Matching Rate   & Confidence \\ \hline
Original Ontology \& Matching Lv. 1     & 0.52\%        & 46.15\%         & 100.00\%   \\
Reshaped Ontology \& Matching Lv. 1     & 30.00\%       & 46.15\%         & 100.00\%   \\
Reshaped Ontology \& Matching Lv. 2     & 38.46\%       & 76.92\%         & 97.50\%    \\
Reshaped Ontology \& Matching Lv. 3     & 42.31\%       & 84.62\%         & 88.00\%    \\
Reshaped Ontology \& Matching Lv. 4     & 46.15\%       & 92.31\%         & 78.33\%    \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

\subsection{Ontology Compliance over KGs} It is often the case that a KG may be restructured to comply with one of several different ontologies, while preserving the KG's intended information content, as illustrated in Figure~\ref{fig: over compliance}.

\begin{figure}[htbp]
\centerline{\includegraphics[width=1\linewidth]{qiang-eswc-2023-figures/Example-Ontology-Compliance-over-KGs.png}}
\caption{An example of ontology compliance over KGs.}
\label{fig: over compliance}
\end{figure}

The key task is ontology alignment and matching. Embedding-based methods are prevalent for exploring the potential matching in graphs due to their conceptual simplicity and computational operability. However, there are several challenges when applying the embedding methods to ontology alignment and matching. Firstly, not all the classes and properties from the original ontology are useful for KG instance embedding. The unused classes and properties could be noise for matching. Secondly, the respective KGs have no connection with each other. Embedding methods are based on random sampling, meaning the vector only represents the relative position of the nodes, and the vector number sets can be different. If two graphs are not tightly connected, the embedding results are most likely to be incorrect. Thirdly, the majority of the embedding methods are targeting graphs without schema. They focus more on topological matching rather than lexicographic matching. We employ our findings from ontology-compliant within KG to address the first challenge, and use their compliance as an intermediate link to connect two graphs - the second challenge, and facilitate lexicographical order - the third challenge. We design Algorithm~\ref{alg: over compliance} for building ontology compliance over KGs. It has three phases: (1) Build ontology compliance within each KG, (2) Match terms across ontologies, and (3) Match overlapping terms. Phases 1 and 2 also reuse Algorithm~\ref{alg: within compliance}.

\begin{algorithm}[htbp]
\scriptsize

\caption{Building Ontology Compliance over KGs}
\label{alg: over compliance}
\begin{multicols}{2}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE $KG_1$ and related ontology $Onto_1$, \\
$KG_2$ and related ontology $Onto_2$
\ENSURE  Matching Set $Match\_S(Onto_1,Onto_2)$,\\ Confidence Set $\mu(\mu_{within}, \mu_{over}) $

\STATE \textbf{/* Phase 1: Compliance within KG */}\\
\STATE $ Onto_{RE_1}, \mu_1 = withinComp(KG_1,Onto_1) $
\STATE $ Onto_{RE_2}, \mu_2 = withinComp(KG_2,Onto_2) $
\STATE $ \mu_{within} \leftarrow \mu_1, \mu_2 $

\STATE \textbf{/* Phase 2: Match terms across Onto */}\\
\STATE /* Create matching set */\\
\STATE Matching Set $ Match\_S(Onto_1,Onto_2) \leftarrow \varnothing $

\STATE /* Follow same procedure in Algorithm~\ref{alg: within compliance} */
\FOR {$ i \in Con\_Onto_{RE_1}, k \in Rel\_KG_1 $}
\FOR {$ j \in Con\_Onto_{RE_2}, l \in Rel\_KG_2 $}
\STATE $ Match\_S(Onto_1,Onto_2), \mu_{cmatch} \leftarrow $ Matched Con \& Rel, $ \mu_{over} \leftarrow \mu_{cmatch} $
\ENDFOR
\ENDFOR

\STATE \textbf{/* Phase 3: Match overlapping terms */}

\STATE /* Set a vector space */
\STATE Vector space $VecSpace \leftarrow \varnothing $
\STATE /* Put KGs and Onto\_{RE} */
\FOR {$ i \in KG_1, Onto_{RE_1}, KG_2, Onto_{RE_2} $}
\STATE $VecSpace \leftarrow i $
\ENDFOR

\STATE /* Put matched Onto set to build links */
\STATE $VecSpace \leftarrow Match\_S(Onto_1,Onto_2) $

\STATE /* Define embedding models */
\STATE Embedding Model $ Model \leftarrow X2Vec.train() $
\STATE /* Define vector set */
\STATE Vector Set $ Vec\_S \leftarrow Model.getEmbeddings() $

\STATE /* Add predict match for overlapping */
\STATE Predict Match $P\leftarrow \varnothing$
\FOR {Unmatched $ U \notin Match\_S(Onto_1,Onto_2) $}
\STATE $ P,\mu_{overlap} \leftarrow Vec\_S.getMostSimilar(U) $
\STATE $ Match\_S(Onto_1,Onto_2) \leftarrow (U,P) $
\STATE $ \mu_{over} \leftarrow \mu_{overlap} $
\ENDFOR

\STATE /* Summarise total confidence */
\STATE Confidence Set $\mu \leftarrow \varnothing$
\STATE $\mu \leftarrow \mu_{within}$
\STATE $\mu \leftarrow \mu_{over}$

~\\

\RETURN $ Match\_S(Onto_1,Onto_2)$, \\ 
$ \mu(\mu_{within}, \mu_{over}) $

\end{algorithmic}
\end{multicols}
\end{algorithm}

The experiment is set to predict the similarity of two overlapping properties, brick:hasPoint in Brick Schema~\citep{balaji2016brick} (abbr. ``Brick'') and core:hasCapability in RealEstateCore~\citep{hammar2019realestatecore} (abbr. ``RECore''). The ground truth is that the meanings of these two properties are very similar. Their different names are due to their different views on how building points are embedded in the building. brick:hasPoint states that the building points are the measurable data points installed in the building, whereas core:hasCapability stands for the building points are the capabilities provided by the building to produce and ingest data. We employ three different vector embedding models to evaluate the top-k searches. Exp.1 uses the traditional KG embedding without ontology compliance, and Exp.2 uses our proposed compliance algorithm. Table~\ref{tab: over compliance} shows the results of the comparison in a test run. We can see Exp.2 outperforms Exp.1 in all three sample embedding models, particularly in top-1 and top-3 searches.

\begin{table}[htbp]
\renewcommand\arraystretch{1.2}
\caption{Evaluation of algorithm for building ontology compliance over KGs.}
\label{tab: over compliance}
\begin{adjustbox}{width=1\linewidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{@k} & \multicolumn{2}{c|}{DeepWalk~\citep{perozzi2014deepwalk}} & \multicolumn{2}{c|}{Node2Vec~\citep{grover2016node2vec}} & \multicolumn{2}{c|}{Struc2Vec~\citep{ribeiro2017struc2vec}} \\ \cline{2-7} 
    & Exp.1            &Exp.2                     & Exp.1            & Exp.2                     & Exp.1            & Exp.2 \\ \hline
1   & $0.03\pm0.17\%$  & $25.86\pm4.48\%$ & $0.04\pm0.20\%$  & $15.32\pm3.70\%$ & $96.88\pm1.52\%$ & $99.98\pm0.14\%$ \\
3   & $1.36\pm1.07\%$  & $57.49\pm4.86\%$ & $13.4\pm3.35\%$  & $56.65\pm5.28\%$ & $100\pm0.00\%$   & $100\pm0.00\%$   \\
5   & $7.58\pm2.57\%$  & $75.51\pm4.17\%$ & $66.54\pm4.85\%$ & $84.86\pm3.63\%$ & $100\pm0.00\%$   & $100\pm0.00\%$   \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

\subsection{Pattern-Based Compliance}

Ontology can be decomposed into smaller ontology fragments. For example, the concepts defined in Brick Schema (abbr. ``Brick'') can be decomposed into three high-level abstraction fragments: Spaces (i.e. brick:Location), Building Equipment and Systems (i.e. brick:Equipment and brick:System), and Building Points (i.e. brick:Point). For each fragment, they can be replaced with the same concepts defined in other building ontologies, such as RealEstateCore~\citep{hammar2019realestatecore} (abbr. ``RECore'') and Project Haystack~\citep{john2020project} (abbr. ``Haystack''), or building-related domain ontologies, such as BOT~\citep{rasmussen2021bot} for spatial information, SAREF~\citep{daniele2015created} for equipment and systems, and SSN~\citep{compton2012ssn}/SOSA~\citep{haller2019modular} for building points. Figure~\ref{fig: pattern compliance} demonstrates an example of KG represented by different combinations of building and related domain ontologies. These new ontology fragments can represent the same information as the original ontology, but they can have different numbers of classes, properties, and hierarchies. If we consider ontology fragments, the problem of ontology compliance becomes more complex.

\begin{figure}[!t]
\centerline{\includegraphics[width=1\linewidth]{qiang-eswc-2023-figures/Example-Pattern-Compliance-over-KGs.png}}
\caption{An example of pattern-based compliance.}
\label{fig: pattern compliance}
\end{figure}

Figure~\ref{fig: pattern-based-architecture} shows the architecture of building pattern-based compliance. It has three main components, namely (1) Pattern Cognition, (2) Pattern Recognition, and (3) Pattern Optimisation. The basic idea is to extract the concepts, relationships, and constraints from the ontology-compliant KG. Each of them goes through a learning and matching process to find their patterns. Then, we integrate and align the same or similar patterns, and use these generic patterns to reconstruct new ontology fragments.

\begin{figure*}[!t]
\centerline{\includegraphics[width=1\linewidth]{qiang-eswc-2023-figures/Pattern-Based-Architecture.png}}
\caption{The architecture of building pattern-based compliance.}
\label{fig: pattern-based-architecture}
\end{figure*}

Ontology fragments may have different numbers of namespaces, levels of abstraction, concept coverage, depth of the class hierarchy, completeness and expressiveness, and performance metrics. Liebig's law~\citep{de1994liebig} is used for ontology fragment construction, evaluation, and selection. The multi-criteria selection depends on the minimum criteria being satisfied. We also introduce a joint-learning approach to evaluate the performance of ontology fragments. An example is shown in Figure~\ref{fig: joint approach}. Ontology Fragment 1, 2, and 3 are generated from the same KG. We fit them into the embedding model and perform the classification task according to the original KG. Based on different levels of abstraction, the classification accuracy of the KG embedding decreases at different rates. Fragment 1 and 2 have higher accuracy in Level 1 and Level 2 abstractions, but they have a significant drop in Level 3. By contrast, Fragment 3 decreases gradually at all levels of abstraction.

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.6\linewidth]{qiang-eswc-2023-figures/Accuracy-Rate.png}}
\caption{A joint approach using classification accuracy to evaluate the performance. The fluctuation of each ontology fragment varies at different levels of abstraction.}
\label{fig: joint approach}
\end{figure}

\newpage

\section{Conclusions}

In this chapter, we present a new concept of ontology-compliant KGs, showing promising results in matching and aligning ontologies within KG and over KGs. We also illustrate our design for advanced pattern-based compliance. Further work will focus on justifying the results with the capability to allow ontology compliance on large-scale KGs, and implementing pattern-based compliance in a comprehensive framework that enables automatic ontology fragment integration, evaluation, and selection for real-world application-level KGs.

\paragraph*{Supplementary Material Statement}

The code implementation is available at~\url{https://github.com/qzc438/ontology-compliant-kgs} (access will be made available on request). Results may have slight differences across different platforms and library versions.

\paragraph*{Publication Statement}

Most of the work presented in this chapter has been published as~\bibentry{qiang2023ontology}.

==> qiang-anu-thesis-content/om-validation.tex <==
\chapter{Crowd-OM: Crowdsourcing for Ontology Matching Validation}
\label{chap: om-validation}

Recent advances in large language models (LLMs) pose new challenges for ontology matching (OM). While OM systems built on LLMs have shown remarkable capabilities in discovering more matching candidates, traditional OM validation that relies on domain experts has become overwhelming. Although crowdsourcing can expose OM validation to large online communities, bias and errors from diverse annotators can reduce the quality of crowdsourcing for OM validation. In this study, we explore the use of crowdsourcing for OM validation and introduce a novel quality assurance crowdsourcing system called Crowd-OM. In order to ensure the quality of crowdsourcing for OM validation, we propose three domain-specific mechanisms, namely differential trustworthiness, coherence pre-filling, and time-dependent modelling. Crowd-OM can be integrated with existing OM systems to enable human-in-the-loop validation. The evaluation shows its effectiveness in handling various annotators and different annotation scenarios. We discuss two real-world use cases and current limitations for improvement.

OM has been used in many real-world applications to enable semantic interoperability for knowledge graphs. Matching validation is a crucial step to ensure that the matching output aligns with real-world facts. This procedure is typically conducted by domain experts in surveys, interviews, and workshops. With the popularity of LLMs, OM systems have been widely incorporated with LLMs and LLM agents~\citep{qiang2023agent,hertling2023olala,giglou2024llms4om,zhang2024large,taboada2025ontology,nguyen2025kroma,sousa2025complex,song2026genom}. While such systems have shown advanced capabilities, rapid evaluation of LLMs poses several challenges for OM validation. In the Ontology Alignment Evaluation Initiative (OAEI)~\citep{oaei} campaign over the years, several annual reports find that LLM-based OM systems can discover more matching candidates, but these mappings are not present in current ground-truth references. Miscounting these disputed mappings has skewed the measurement of system performance. To tackle this issue, one popular approach is to employ harness engineering (e.g., chain-of-thoughts~\citep{wei2023chainofthought} and agent debate~\citep{du2024improving}) for LLMs, but LLM hallucinations are not easy to mitigate and can remain unavoidable~\citep{kalai2026evaluating}. For disputed mappings that require additional human validation, it is not easy to find domain experts and they may also have unavoidable human bias~\citep{tversky1974judgment}.

Crowdsourcing is particularly suitable for this scenario. Rather than conducting the validation within a group of domain experts, exposing this procedure to the large online community could significantly mitigate LLM hallucinations and reduce the negative effects of human bias. We consider crowdsourced participants who undertake tasks to be \textit{annotators}. Independent and diverse annotators exposing different options has proven to be an effective way to obtain less biased decisions~\citep{surowiecki2004wisdom}. However, crowdsourcing has several limitations. For example, the diversity of online annotators can include non-experts for validation, and their decisions are typically treated as equivalent to those of experts. This can lead to a phenomenon in which non-experts may dominate decision-making~\citep{selgin1996salvaging}. Moreover, crowdsourcing is labour-intensive and errors increase significantly when tasks require extensive mental effort~\citep{sweller1988cognitive}.

In this study, we explore the use of crowdsourcing for OM validation and introduce a novel crowdsourcing system. The system can be integrated with existing OM systems to enable crowdsourced OM validation. To tackle known issues in crowdsourcing, we propose three domain-specific mechanisms to improve the quality of crowdsourced OM validation. Our main contributions include:

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item We introduce a crowdsourcing system called Crowd-OM for OM validation. The system can be easily integrated with existing OM systems to enable interactive human-in-the-loop matching validation for OM tasks.
\item We propose three domain-specific mechanisms to improve the quality.
\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item Differential trustworthiness uses a set of seed pairs to assess each annotator's trustworthiness and apply the results to the overall agreement measure, therefore giving more weight to the expert's decision and reducing the weight of the non-experts' opinions.
\item Coherence pre-filling uses reasoners to pre-fill annotation pair decisions from the annotator's completed answers, therefore reducing errors from manual input.
\item Time-dependent modelling uses the continuous editing mode to ensure the validation output is always up to date. When annotators change their decisions, the system tracks these changes and modifies accordingly in a timely manner.
\end{itemize}
\item We implement Crowd-OM with the three quality-assurance mechanisms on an existing OM system. We evaluate our proposed mechanisms in controlled scenarios and demonstrate their effectiveness in improving crowdsourced OM validation.
\end{itemize}

\section{Related Work}

OM with human-in-the-loop (a.k.a. interactive OM) aims to overcome the bottleneck in automatic OM approaches that have reached the performance upper bound. Involving domain experts in OM validation has proven an effective way to utilise user feedback to improve OM performance~\citep{paulheim2013towards,dragisic2016user,li2019user}. In the era of LLMs, human-in-the-loop is integral. State-of-the-art LLM fine-tuning methods (e.g. RLHF~\citep{ouyang2022training} and DPO~\citep{rafailov2023direct}) leverage positive and negative user feedback to adjust LLMs for domain-specific tasks. Foreseeing the benefits of human-in-the-loop, the quality of user feedback becomes externally important. If the user's feedback does not provide sufficient information, LLMs may have very limited knowledge to learn or may even learn incorrect knowledge. Therefore, the annotators need to be carefully selected, and the answers need to be carefully filtered and processed.

Crowdsourcing is a popular technique in human-in-the-loop evaluation and is being used in a wide range of ontology engineering tasks. Traditionally, in the context of OM, validation is conducted by domain experts to ensure that the provided ground-truth reference alignments are correct for benchmarking. This approach requires extensive expert labour, which is infeasible for large-scale OM tasks. CROWDMAP~\citep{sarasua2012crowdmap} is an early work that proposes using a workflow model for crowdsourced OM. However, this method is highly dependent on the CrowdFlow platform, and the validation process provides limited support for resolving conflicting or inconsistent cases. To the best of our knowledge, this work is the first attempt to leverage crowdsourcing for quality OM validation with considerations of reliability and feasibility.

\section{Problem Formulation}

Given the reference alignment $R$ and the matcher alignment $A$, OM validation considers non-disputed mappings to be the mappings that appear both in $R$ and $A$ (i.e. $A\cap R$). The mappings that exist only in $R$ (i.e. $R-A$) or only in $A$ (i.e. $A-R$) are disputed mappings and require additional human validation.

\section{System Design}

Crowd-OM operates as a two-sided marketplace, similar to Airtasker~\citep{airtasker}. A group of system users can post their annotation tasks, and another group of system users can participate in them. We initialise three different user types.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item Administrator: The administrator is the superuser of the system. The administrator is responsible for uploading the original datasets and controlling the open/close status. The administrator can also view details of the system users, such as the annotation tasks in which they participate and the decisions they made on each annotation pair.
\item Developer: The developer is a specific type of system user. They are allowed to upload the alignment produced by the matcher into the system and to specify the customised settings for their annotation task. Developers are not allowed to participate in annotation tasks produced by their own matchers.
\item Annotator: The annotator is the main user of the system. They are allowed to annotate the same datasets multiple times for different tasks posted by different matchers.
\end{enumerate}

We allow a single user to have multiple roles in the system. For example, a developer can serve as an annotator by participating in annotation tasks posted by other matchers. We consider a developer to be a user who has registered at least one matcher in the system, whereas an annotator is a user who has started at least one annotation task. Annotators must complete registration (including reading the information sheet and signing the consent form) before participating in the annotation task for data collection.

Figure~\ref{fig: conceptual-model} shows the conceptual model of Crowd-OM. The system consists of datasets from different domains and matchers from different developers. When a matcher produces a system alignment, the result is compared with the corresponding dataset to find disputed mappings. These mappings are formed into an annotation task. Annotators need to make decisions on each disputed mapping contained in the annotation task. Each annotator needs to determine whether the annotation pair (i.e. two entities in the disputed mappings) are ``Equivalent'' or ``Not Equivalent''. They can view the class hierarchy, logic restriction, and textual description side by side to facilitate their decision on equivalence. Crowd-OM follows the majority voting rule. A disputed mapping is considered equivalent if more than 50\% of annotators vote ``Equivalence''. Some domains (e.g. biomedical) require high precision; the system allows the confidence threshold to be adjusted from 50\% to 100\%.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.7\linewidth]{qiang-vldb-2027-figures/database-overview.png}
\caption{Conceptual model of Crowd-OM.}
\label{fig: conceptual-model}
\end{figure}

To ensure the quality of crowdsourcing for OM validation, we propose three novel quality-assurance mechanisms for Crowd-OM system.

\subsection{Differential Trustworthiness}

Crowdsourcing does not restrict non-experts from participating in annotation tasks. The number of non-experts is often greater than that of experts, so the votes of non-experts can dominate the votes of experts. We expect the experts' decisions to carry more weight.

We construct a set of seed pairs to complement the original base pairs. The seed pairs are used to examine the expertise of annotators, and therefore determine the trustworthiness of their decisions. These seed pairs have clear answers of ``Equivalent'' or ``Not Equivalent''. The seed pairs need to be mixed with the original annotation pairs to avoid recognition. We use the following logic to generate positive and negative seed pairs.

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item Positive seed pairs are generated from the non-disputed mappings and consist of two parts: (1) Trivial: entity names (or labels) are similar. (2) Non-trivial: entity names (or labels) are different.
\item Negative seed pairs are generated using the following logic: (1) Trivial: If $(e1, e2)$ exists in non-disputed mappings, then $(e3, e2)$ where $e3 \equiv e1$ should not be correct. This assumes these mappings are one-to-one mappings. (2) Non-trivial: $(e1,e2)$ exist in disputed mappings and fail to pass the ontology coherence check.
\item To ensure that the difficulty of positive and negative seed pairs is similar, we compute the total number and the distribution of trivial and non-trivial rates for positive seed pairs and apply the same ratio to generate negative seed pairs.
\end{itemize}

Given the number of seed pairs $m$ and the number of correct answers $n$ given by the annotator $u$, the trustworthiness $\tau$ is defined as $\tau(u) = n/m$. When moving to the original annotation pairs (i.e. non-seed pairs), $\tau$ is used as a weight applied to each annotator's answer. We define $d(u,q)\in \{0,1\}$ as the score received from the annotator $u$ for an original annotation pair $q$, in which $0$ refers to the answer ``Not Equivalent'' and $1$ refers to the answer ``Equivalent''. The weighted agreement score accumulated for each $q$ is the product of each annotator's answer $d(u,q)$ and their trustworthiness $\tau$, divided by the number of annotators $N$. Hence, the weighted agreement score $w(q)\in (0,1)$ is computed as:

\begin{equation}
w(q) = \frac{1}{N} \sum_{u=1}^{N} d(u,q) \cdot \tau(u)
\end{equation}

\subsection{Coherence Pre-Filling}

Crowdsourcing expects annotators' attention and involvement to be consistent throughout the annotation session. However, several studies have shown that annotators' engagement inevitably declines with time-consuming tasks. We aim to reduce the workload for annotators by automatic pre-filling.

We use the coherence check to achieve this function. While each annotator's decision creates an assertion rule, these rules can be used to infer other supporting or conflicting annotation pairs. This can be applied both within the datasets and between datasets within the same domain. For example, within the dataset, if the annotator labelled $A \equiv B$, then $C \not\equiv B$ can be pre-filled in a one-to-one mapping task; Between datasets within the same domain, if the annotator labelled $A \equiv B$ in one dataset and $B \equiv C$ in another dataset, then a transitive equivalence $A \equiv C$ can be inferred and pre-filled if it appears in the dataset from the same domain.

A reasoner is used to automate this process. We construct an \textit{ontology network} and ask the reasoner to infer the explicit assertions as pre-fills. The \textit{ontology network} contains the original ontology as the base ontology and forms each annotation decision as an assertion within the ontology. For the coherence check between datasets within the same domain, we also combine multiple ontologies.

\subsection{Time-Dependent Modelling}

Typically, there is no persistent ground truth for OM tasks. The reference alignments generated by domain experts are based on their own opinions. For example, ``NCI'' commonly refers to ``National Cancer Institute'' globally, but within the context of Australian research, this abbreviation is more likely to refer to ``National Computational Infrastructure''. Our system allows annotators to modify their decisions over time and to assign a timestamp label to the validation output. When an annotator changes the decision, the overall crowdsourced decision is expected to change accordingly.

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item If the annotator changes the decision on the original annotation pairs, this action directly affects the crowdsourced decision.
\item If the annotator changes the decision on the seed pairs, this action may change their trustworthiness and further affect the crowdsourced decision on each original annotation pair.
\end{itemize}

\section{System Demonstration}

We demonstrate how Crowd-OM can extend existing OM systems to enable crowdsourced human-in-the-loop validation. We select Agent-OM~\citep{qiang2023agent} as the matcher, and the matching output is obtained from the OAEI 2025 campaign~\citep{qiang2025oaei}.

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]

\item \textbf{Administrator Actions.} The system only allows the administrator to upload the reference alignment $R$. The administrator needs to assign the dataset to one registered domain. If the domain does not exist, the administrator can register a new domain. Each dataset requires three files to upload: the two ontology files and the reference alignment between them. For example, the administrator registers a domain called ``conference'' and adds two datasets ``cmt-conference'' and ``cmt-conof'' under the ``conference'' domain. The administrator can edit the settings of the datasets and domains by setting a confidence threshold and opening or closing the domain for annotation. For example, the administrator sets the 50\% confidence threshold for the ``conference'' domain and opens this domain for annotation.

\item \textbf{Developer Actions.} The system only allows the developer to upload the matcher alignment $A$. The developer needs to register the matcher and provide a short description. By doing so, they automatically become the developer of the matcher. The developer can also add other developers. Once the developer completes the upload, the system computes the difference between the matcher alignment $A$ and the reference alignment $R$ to find disputed mappings and form an annotation task. The developer can edit the settings for the annotation task. For example, the developer can enable or disable the differential trustworthiness and coherence pre-filling mechanisms as follows. (1) If differential trustworthiness is being activated, the system automatically generates a set of positive and negative seed pairs. These seed pairs labelled as ``seed'' are visible to developers but not to annotators. (2) If coherence pre-filling is being activated, the system performs a coherence check based on the inputs from the annotator and pre-fill annotation pairs. Annotation pairs labelled as ``pre-filling'' are visible to both developers and annotators, with a short explanation of the description logic involved.

\item \textbf{Annotator Actions}. The system allows the annotator to select an annotation task produced by a single matcher for a specific dataset. They can only annotate the tasks with the matcher for which they are not a registered developer, and the dataset under the domain is currently open for annotation. There are three options available for each annotation pair: ``Equivalent'', ``Not Equivalent'', and ``N/A''. (1) The trustworthiness is computed when the annotator completes the annotation task (i.e. there is no ``N/A'' annotation within the dataset). (2) The coherence pre-filling continuously monitors the annotator's decisions to identify new pre-fills. (3) The annotator can change the decision on each annotation pair at any time. The trustworthiness and coherence pre-filling will respond to changes in the decision accordingly.

\end{itemize}

\section{System Evaluation}

In this section, we simulate the diversity of the annotator groups and different system settings. The purpose is to demonstrate the system's effectiveness in handling real-world challenges of using crowdsourcing for OM validation, such as low expert ratio and knowledge level, or high rates of annotation errors.

We select six OAEI tracks comprising 45 datasets for evaluation. The matcher output is obtained from the Agent-OM results in the OAEI 2025 campaign. For each controlled environment, we simulate 100 human annotators in the system. We use the default confidence threshold of 50\% and the seed number 42 for reproducibility.

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]

\item \textbf{Differential Trustworthiness.} We simulate 100 human annotators with a mixture of experts and non-experts. Experts are expected to have a trustworthiness greater than 0.5, while non-experts are expected to have a trustworthiness less than 0.5. The trustworthiness reflects the accuracy of the annotator's answers. For example, a trustworthiness of 0.7 means that the annotator has a 70\% probability of labelling the TP as ``Equivalent'' and a 30\% probability of labelling the TP as ``Not Equivalent''. Here, we assume that the reference alignments $R$ provided by the OAEI track are complete. The mappings that exist only in $R$ (i.e. $R-A$) are true-positive mappings (TPs), while the mappings only in $A$ (i.e. $A-R$) are false-positive mappings (FPs).

Figure~\ref{fig: simulation-dt-expert-ratio} compares the discovery rates of TPs and FPs as the expert ratio varies from 0.0 to 1.0. Although there is no difference when the expert radio is very low or very high, our differential trustworthiness mechanism shows significant improvements when the expert radio is in the range [0.1, 0.6], which is more common in real-world scenarios. Figure~\ref{fig: simulation-dt-expert-lower} compares the discovery rates of TPs and FPs as the expert knowledge lower bound varies from 0.5 to 1.0. We can see that our differential trustworthiness is particularly useful when the expert knowledge lower bound is less than 0.85. In reality, experts can also make mistakes and achieving the expert knowledge lower bound above 0.85 is almost impossible.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2027-figures/simulation_dt_expert_ratio.png}
\caption{Discovery rates of TPs and FPs vs expert ratio.}
\label{fig: simulation-dt-expert-ratio}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2027-figures/simulation_dt_expert_lower.png}
\caption{Discovery rates of TPs and FPs vs expert knowledge.}
\label{fig: simulation-dt-expert-lower}
\end{figure}

\item \textbf{Coherence Pre-Filling.} We simulate 100 human annotators and each annotator's decision is randomly selected from ``Equivalent'' or ``Not Equivalent''. We do not specify whether annotators are experts or non-experts. For the purpose of assessing the propagation behaviours of coherence pre-filling, we expect this function to work for all annotators. Here, we define an \textit{anchor ontology} for each domain and call datasets containing alignments for this ontology \textit{anchor datasets}. We only simulate the annotator's input on \textit{anchor datasets} and leave others for pre-filling candidates. We use \textit{coverage} to describe the fraction of annotated pairs in the \textit{anchor datasets}.

Figure~\ref{fig: simulation-cpf-type} compares the number of pre-fills by type as coverage varies from 0.1 to 1.0. Only three types exist in the OAEI datasets we evaluated: transitive equivalence, subsumption negativity, and disjointness. Overall, we can see that the coverage within [0.3, 0.8] yields more pre-fills. A low fraction of annotated pairs reduces the number of assertions to discover, whereas a high fraction of annotated pairs leaves little space for pre-filling to be functional. Figure~\ref{fig: simulation-cpf-domain} compares the number of pre-fills by domain as coverage varies from 0.1 to 1.0. We can see that the propagation behaviours of coherence pre-filling vary across different domains. This may be because the ontology design in each domain follows its own well-agreed guidelines, thereby restricting the use of logic expressions.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2027-figures/simulation_cpf_type.png}
\caption{Pre-fills by type vs coverage.}
\label{fig: simulation-cpf-type}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2027-figures/simulation_cpf_domain.png}
\caption{Pre-fills by domain vs coverage.}
\label{fig: simulation-cpf-domain}
\end{figure}

\newpage

\item \textbf{Time-Dependent Modelling.} We simulate 100 human annotators (50\% experts and 50\% non-experts) with varying trustworthiness. Similarly, we assume that TPs are mappings that exist only in the reference and FPs are mappings that exist only in the matcher. Here, we define 0.5/0.5 as both non-experts and experts having trustworthiness 0.5, while 0.1/0.9 means non-experts with trustworthiness 0.1 and experts with trustworthiness 0.9.

Figures~\ref{fig: simulation-tdo-non-seed} and~\ref{fig: simulation-tdo-seed} compare the discovery rates of TPs and FPs as the correction rate varies from 0.0 to 1.0.  We can see that correction in non-seed pairs always increases the discovery rate and follows a linear incremental pattern. For correction in seed pairs, there is only a significant increase with a low spread ratio of 0.5/0.5 or 0.4/0.6 and a low correction fraction within [0.0, 0.2]. Note that the seed pair correction is a cascading operation, as the annotator will be given new correct non-seed pairs due to the increase in trustworthiness. The results indicate that our time-dependent modelling can capture individual decision changes over time with corresponding changes in the overall decision. It also works well with differential trustworthiness to fairly assess changes in the annotator's decisions.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2027-figures/simulation_tdo_non_seed.png}
\caption{Discovery rates of TPs and FPs vs fraction of wrong decisions corrected (non-seed pairs).}
\label{fig: simulation-tdo-non-seed}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-vldb-2027-figures/simulation_tdo_seed.png}
\caption{Discovery rates of TPs and FPs vs fraction of wrong decisions corrected (seed pairs).}
\label{fig: simulation-tdo-seed}
\end{figure}

\end{itemize}

\newpage

\section{Use Cases}

Having evaluated Crowd-OM for improving the quality of OM validation, we present two real-world use cases.

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]

\item \textbf{Reference Evolution.} OAEI is one of the largest communities focused on OM. Over the years, the reference alignment used across several tracks has been out of date. Since the introduction of ChatGPT~\citep{chatgpt} in 2022, new matchers incorporating LLMs have identified more matching candidates that are not present in current references. These mappings seem to be correct, but they lack expert human validation to ensure their quality. While existing reference alignments are curated by domain experts, they may exhibit confirmation bias, in which their judgements are based on their preconceived notions. Crowd-OM can be used to mitigate human bias in this case.

\item \textbf{Ontology Harmonisation.} In the building industry, ontology harmonisation has received significant attention due to the emerging need to integrate building information systems from different vendors. Despite the foundation established by the harmonisation efforts between Brick Schema~\citep{balaji2016brick}, RealEstateCore~\citep{hammar2019realestatecore}, and Project Haystack~\citep{john2020project}, achieving semantic interoperability between these ontologies remains a challenge. Many mappings in these ontologies commonly use abbreviations and domain-specific terminologies. Crowd-OM can be used as an alternative to expert-based validation.

\end{itemize}

\section{Limitations}

It is recommended to have a diverse set of participants for annotation tasks, but this is not controllable in crowdsourcing systems. We consider the bias caused by homogeneity to be minor when there is a considerable number of annotators. Moreover, real-world annotations can be more complicated than those in controlled simulations. For example, we assume the annotator's performance is consistent across seed and non-seed pairs, but it could be that the annotator performs very well on seed pairs but poorly on the real non-seed pairs. These edge cases need to be carefully identified and preprocessed before fitting to the models for analysis.

Crowd-OM currently focuses on the most common one-to-one equivalent matching, but it can be extended to more complex matching tasks. For example, the logic for generating equivalent seed pairs can be extended for subsumption: (1) Positive: If $A \equiv B$ and $C \subseteq A$, then $C \subseteq B$. (2) Negative: If $A \not\equiv B$ and $C \subseteq A$, then $C \not\subseteq B$. Coherence pre-filling can be modified to support subsumption tasks in similar ways.

\section{Conclusions}

In this chapter, we propose a novel crowdsourcing system Crowd-OM for OM validation with three quality-assurance mechanisms. We present the system design and illustrate a system demonstration. The evaluation shows that the proposed quality-assurance mechanisms improve the system's robustness and overcome the inherent challenges of crowdsourcing for OM validation. In the future, we plan to adopt Crowd-OM in real-world use cases and contribute to the creation of robust benchmarks for OM tasks.

In the next chapter we turn to an additional and complementary step in the ontology interoperability framework: data-driven validation using ontology-compliant knowledge graphs.

\paragraph*{Publication Statement}

Most of the work presented in this chapter has been published as~\bibentry{qiang2026unlocking}.

==> qiang-anu-thesis-content/om4ov.tex <==
\chapter{OM4OV: Leveraging Ontology Matching for Ontology Versioning}
\label{chap: om4ov}

Due to the dynamics of the Semantic Web, version control is necessary to manage changes in widely used ontologies. Despite the long-standing recognition of ontology versioning (OV) as a crucial component of efficient ontology management, many approaches treat OV as similar to ontology matching (OM) and directly reuse OM systems for OV tasks. In this study, we systematically analyse similarities and differences between OM and OV and formalise an OM4OV framework to offer more advanced OV support. The framework is implemented and evaluated in the state-of-the-art OM system Agent-OM. The experimental results indicate that OM systems can be effectively reused for OV tasks, but without the necessary extensions, can produce skewed measurements, poor performance in detecting update entities, and limited explanations of false mappings. To tackle these issues, we propose an optimisation method called the cross-reference (CR) mechanism, which builds on existing OM alignments to reduce the number of matching candidates and to improve overall OV performance.

Ontologies serve as the backbone of the Semantic Web, providing formal concept descriptions of shared concepts across various applications~\citep{gruber1993translational}. An ontology is not static, and the need for version control arises. While web data is dynamic, any ontology in use must undergo periodic revisions to keep pace with the growth in domain knowledge, modifications to the application adaptation, or corrections to the shared conceptualisation~\citep {klein2001ontology}. For example, it is unrealistic to expect ontologies created in the 1990s to contain concepts such as ``touchscreen'', ``fingerprint sensor'', or ``WiFi antenna''~\citep{haller2020we}. These modifications may cause undesirable deficiencies in artifacts that conform to or that reuse the ontology being changed, leading to severe non-compliance and incompatibility issues in downstream tasks.

\newpage

Ontology versioning (OV), also known as ontology evolution, aims to distinguish and recognise changes between different ontology versions. This enables data that applies the ontology, ontologies that reuse the ontology, and software that uses the ontology to correctly respond to the ontology version changes~\citep{klein2001ontology}. Although OV plays an important role in ontology management, this area remains underexplored. Many studies~\citep{noy2002promptdiff,noy2004tracking,noy2004ontology,castano2006matchmaking,gross2012computed,zahaf2016alignment,kozierkiewicz2019triggering,kozierkiewicz2019updating,kozierkiewicz2020updating,pietranik2023methods} treat OV as similar to ontology matching (OM) and assume OM systems can be reused for OV tasks. OM is a well-studied problem, so leveraging this deep research legacy for OV should be beneficial. We call this approach ``OM4OV''.

We analyse the complementary relationship between OM and OV tasks and provide a task formulation for the OM4OV framework. We implement the framework in our Agent-OM~\citep{qiang2023agent} system to validate its effectiveness in unifying the OM and OV tasks. We investigate the links between these two tasks in practice and explore optimisations for OM4OV. To the best of our knowledge, this work is the first to systematically analyse the OM4OV framework and to provide theoretical foundations and empirical evidence for its effectiveness and pitfalls. Specifically, our key contributions include:

\begin{itemize}
\item We analyse the similarities and differences between OM and OV. In the OM4OV framework, we describe four disjoint subset alignments produced in the OV process: \textit{remain}, \textit{update}, \textit{add}, and \textit{delete}, each corresponding to a subset of match or non-match in OM. We provide formal definitions and formulations.
\item We extend Agent-OM with the OM4OV framework and call the extended system Agent-OV. We evaluate the performance of OV on the testbed derived from the Ontology Alignment Evaluation Initiative (OAEI)~\citep{oaei} datasets. We find that OM systems can be reused for OV tasks, but extensions are necessary to improve both overall OV performance and its meaningful quality measurement.
\item We propose an optimised OM4OV framework. The new framework introduces a cross-reference mechanism, which builds on prior OM alignments to overcome the pitfalls of the naive OM4OV framework by reducing the number of matching candidates and filtering out ambiguous false mappings, thereby significantly improving overall OV performance.
\end{itemize}

In this study, we assume the OWL 2 Web Ontology Language~\citep{owl2012} is used to represent an ontology. We use both \emph{concept} and \emph{entity} to refer to OWL classes or properties. We use \emph{subsumption} to mean \texttt{rdfs:subClassOf} or \texttt{rdfs:subPropertyOf} and \emph{equivalence} to mean \texttt{owl:equivalentClass} or \texttt{owl:equivalentProperty} as formal class and property inter-relations.

\section{Related Work}

Version control is recognised as a vital element in ontology management. Different versions need to support interoperability so that version changes do not impede the effective and sustainable use of the ontology. One manual approach is to extend the ontology itself with internal version information. The Simple HTML Ontology Extensions~\citep{heflin2000dynamic} uses the tag \texttt{BACKWARD-COMPATIBLE-WITH} to record version information. The authors of~\citep{klein2002ontology} argue that a carefully-managed version numbering system embedded in the URI of the ontology (and therefore the fully expanded name of entities defined in the ontology) can minimise the impact of adopting updated versions because unchanged entities will be unaffected in practice. These approaches have been largely adopted by the later OWL languages, where a set of annotation properties related to version information is defined. These include \texttt{owl:versionInfo} and \texttt{owl:priorVersion} to describe the version number of the ontology, \texttt{owl:backwardCompatibleWith} and \texttt{owl:incompatibleWith} to specify an entity's compatible or incompatible corresponding entity in the previous version, and \texttt{owl:DeprecatedClass} and \texttt{owl:DeprecatedProperty} to declare deprecated entities. Later, the ontology language $\tau$OWL~\citep{zekri2016tau} was introduced to extend the OWL triple schema to a 4-tuple schema to represent the versioning of concepts within an ontology. This idea is now incorporated in the new proposals for RDF 1.2 Schema~\citep{rdf12}, which allow time-varying information to be deduced from a temporal dimension within the 4-tuple. An alternative option is to create a separate version log to track changes in versions. Unlike earlier approaches that use an unstructured plain text file, the authors of~\citep{plessers2005ontology} propose a novel approach that uses a version ontology with a change definition language to create a version log. In~\citep{cardoso2020construction}, the authors construct an historical knowledge graph. Storing the version log in a knowledge graph not only avoids repetition, but also enables advanced search functions. The authors of~\citep{sassi2016supporting} argue that version logs may contain redundancy and inconsistent information. They propose a graph-of-relevance approach to interlink different version logs and remove less relevant versions.

Maintaining version information in the ontology can be labour-intensive and error-prone. Either extending the current standard 3-tuple schema or using change logs requires consistent updating over time. In most cases, this process is hand-crafted by the ontology engineer or requires human intervention (e.g. pre-defining a schema or creating a template for the change log). A manual process is more likely to make mistakes and fail to propagate changes to dependent artifacts. Moreover, an ontology may lack or have incomplete version information. In such cases, current approaches have limited capability to detect incorrect or missing version information. These approaches rely on the version information contained in or attached to the ontology by manual methods. If such information is missing or incorrect, automated versioning of ontology concepts becomes necessary.

Reusing OM systems for OV tasks (OM4OV) is a lightweight and fully automatic approach to detecting changes in ontologies. OM4OV is compatible with ontologies that use different recording methods, including URIs or additional versioning triples, as well as ontologies that lack internal version information. The PromptDiff suite~\citep{noy2002promptdiff,noy2004tracking,noy2004ontology} is the canonical work that integrates different heuristic matchers and applies a matching-like comparison for OV. The concept of ``matching'' is later used in the H-Change methodology~\citep{castano2006matchmaking} to assess the assimilation of new concepts into the old ontology. Several studies~\citep{gross2012computed,zahaf2016alignment} note that updates to an ontology will generally create a requirement to update its existing alignments to external ontologies. Methods~\citep{kozierkiewicz2019triggering,kozierkiewicz2019updating,kozierkiewicz2020updating} are proposed to identify changes that affect alignments, and in some cases the framework is proposed to automate alignment updates~\citep{pietranik2023methods}, but these works do not address the discovery of alignments from an ontology to its own updated version.

While existing OM4OV approaches directly use OM systems for OV and focus on developing new algorithms and architectures for ontology version control, they pay less attention to understanding the underlying differences between OM and OV. OM is not exactly the same as OV. OM determines \textit{matched} entities between two different ontologies, while OV can distinguish \textit{add}, \textit{delete}, \textit{remain}, and \textit{update} changes over different versions of one ontology. The OM input consists of two distinct ontologies, whereas the OV input is expected to consist of two versions of a single ontology. The output of OM is a set of entity mappings, whereas the output of OV comprises four sets, each defined by the nature of the change made. These differences may affect the adaptability of reusing OM systems for OV tasks.

\section{Task Formulation}

We now draw on concepts in OM to formalise OV tasks. Given an ontology $O$, we say that some entity $e\in O$ when $e$ is of interest to ontology matching or ontology versioning, typically representing a concept of the domain of interest being modelled by $O$. We consider an entity to be the full URI of the reference in an ontology, or its equivalent abbreviation via a prefix, for example \texttt{cmt:ProgramCommitteeChair}. We consider an \textit{entity name} to be the substring of an entity that provides a meaningful description of the entity (e.g. \textit{ProgramCommitteeChair}), excluding any entity prefix or expanded URI (e.g. \texttt{cmt:ProgramCommitteeChair} is not an entity name).

\subsection{OM Preliminaries}

OM identifies correspondences between entities of two ontologies~\citep{euzenat2007ontology}. Formally, given a source ontology ($O_s$) and a target ontology ($O_t$), the OM task is to find an alignment $A$ (i.e. a set of mappings) with respect to a given similarity threshold $s \in [0,1]$, defined as~\citep{euzenat2007semantic}: $A = \{(e_1, e_2, r, c) \mid e_1 \in O_s, e_2 \in O_t, s \leq c \leq 1\}$, where $e_1$ and $e_2$ are ontology entities in $O_s$ and $O_t$ respectively, $r$ is the relation between $e_1$ and $e_2$ that may be equivalence ($\equiv$) or subsumption ($\subseteq$), and $c$ is the confidence. For example, \texttt{(cmt:ProgramCommitteeChair, confof:Chair\_PC, $\equiv$, 0.90)} means \texttt{cmt:ProgramCommitteeChair} and \texttt{confof:Chair\_PC} are equivalent with a confidence of 0.90.

An entity match is asserted by a matching system according to its own internal algorithm, its own interpretation of ``match'', and its own assessment of confidence. In general for matching, a source entity may occur in multiple mappings that vary with respect to the target entity, the relation, and the confidence. In this study, we consider only alignments made by matching systems that are comprised of one-to-one equivalence mappings, admitting only matches with the highest $c$ as determined by the matching system and requiring the matching system to resolve tied confidence scores. Typically, equivalence relations are determined by lexical or embedding similarity in matching systems, although logical entailment is equally admissible in our study. OM performance is measured by comparing the matching system alignment (A) with a reference alignment (R) using precision, recall, and F1 score (see Section~\ref{sub-sec: evaluation-criteria} for details).

\subsection{OM4OV Formalisation}

OV identifies correspondences between two versions of a single ontology~\citep{klein2001ontology}. Given an old version of an ontology ($O$) and a new version of the same ontology ($O'$), the OV task can be considered as finding an alignment (A) from the old ontology to the new one. As illustrated in Figure~\ref{fig: om4ov}, while an alignment for OM only mentions matched entities, OV needs to recognise both matched and non-matched entities. Furthermore, OV matched entities are comprised of two subsets: \textit{remain} and \textit{update}, while non-matched entities are comprised of \textit{add} and \textit{delete} entities. While some of these sets are comprised of entities, and others of mappings, when convenient henceforward, we will loosely refer to all of these as either alignments or sets of entities interchangeably.

\begin{figure}[htbp]
\includegraphics[width=1\linewidth]{qiang-tgdk-figures/OM4OV.png}
\caption{Overview of the OM4OV framework. The sets are comprised of entities, with the matched intersection containing entities that are considered equivalent by an ontology alignment.}
\label{fig: om4ov}
\end{figure}

An OV task can be formalised as finding an alignment and a non-alignment, $A_{match}$ and $A_{non-match}$ respectively, between different ontology versions $O$ and $O'$ with respect to a given similarity threshold $s \in [0,1]$. OV focuses only on the equivalence relation; subsumption mappings are beyond the scope of versioning.
\begin{definition}
Given ontologies $O$ and $O'$ and similarity threshold $s \in [0,1]$, the OV task is to find  $A_{match}$ and $A_{non-match}$ as follows:
\begin{equation}
\begin{aligned}
A_{match} = \{(e_1, e_2, c) &\mid e_1 \in O, e_2 \in O', s \leq c \leq 1 \\ &\mbox { and there is no }  (e_1, e_i, c') \mbox{ with } e_i \neq  e_2 \mbox { or with }  c \neq c'  \\ &\mbox{ and there is no } (e_j, e_2, c') \mbox{ with } e_j \neq  e_1 \mbox { or with }  c \neq c' \}  \\
A_{non-match} = \{e \mid e \in O &\cup O' \mbox{ and there is no }  (e_1,e_2,c) \in A_{match} \mbox{ with } e \in \{e_1,e_2\}\}  \\
\end{aligned}
\end{equation}
We say that $e1$ and $e2$ are equivalent whenever there is a $c$ satisfying $(e1,e2,c) \in A_{match}$.
\end{definition}
For convenience, we will sometimes refer to the elements of $A_{match}$ as \emph{entities} rather than \emph{mappings}, by which we mean entities that are mentioned in mappings in $A_{match}$.

The \textit{update} and \textit{remain} entities are entities successfully matched over different ontology versions. The \textit{update} entities are, in general, the closest near-equivalent matches of entities from different ontology versions. We recommend that matching systems assign lower confidence to entity matches when either (a) structural changes have been made near the entity, such as changes to class membership or property restrictions, or (b) the entity's name has changed.

We recommend that all other successful matches not satisfying either (a) or (b) are assigned very high confidence by matching systems, most especially when a so-called \emph{trivial} match is found. These matches are then interpreted as \textit{remain} entities for OV. In particular, we say that an entity is interpreted as not changed in OV for any successful match where the matching system reports a confidence of 1. Further, we recognise that some OV systems may prefer, additionally, to interpret an entity as not changed when the confidence is only slightly less than 1. In some cases, OV systems may consider matches that are near-enough with a confidence slightly less than 1 to be perfect matches. Without loss of generality, we assume in such cases that the OV system reassigns $c$ to be 1.
\begin{definition}
$A_{remain} (A\odot)$ and $A_{update} (A\otimes)$ are defined as:
\begin{equation}
\begin{aligned}
&A\odot = \{(e_1, e_2, c) \mid (e_1, e_2, c) \in A_{match} \mbox{ and } c = 1\}     \\
&A\otimes = \{(e_1, e_2, c) \mid (e_1, e_2, c)  \in A_{match} \mbox{ and } c < 1\}  \\
\end{aligned}
\end{equation}
\end{definition}

We can see that $A_{match} = A\odot \cup A\otimes$. By definition, $A\odot$ and $A\otimes$ are disjoint.

The \textit{add} and \textit{delete} entities are actually non-matched entities between different ontology versions. The \textit{add} entities are the entities in $O'$ that have no matches in $O$. Similarly, we can interpret the \textit{delete} entities as entities in $O$ that have no matches in $O'$.
\begin{definition}
$A_{add} (A\oplus)$ and $A_{delete} (A\ominus)$ are defined as:
\begin{equation}
\begin{aligned}
&A\oplus = \{e \mid e \in O'\mbox{ and } e \in A_{non-match} \}      \\
&A\ominus = \{e \mid e \in O\mbox{ and } e \in A_{non-match} \}      \\
\end{aligned}
\end{equation}
\end{definition}
We can see that $A_{non-match} = A\oplus \cup A\ominus$. By definition, $A\oplus$ and $A\ominus$ are disjoint.

\section{OM4OV Evaluation}
\label{sec: evaluation}

We now consider the evaluation of OM4OV. In the literature, OV are evaluated using OM measures, which we refine here to give better insights into OV performance.

\subsection{Dataset Construction}
\label{sub-sec: dataset-construction}

There is a dearth of benchmark datasets for evaluating OV. The Ontology Alignment Evaluation Initiative (OAEI) contains several datasets related to OM tasks, but none are specifically designed for OV tasks. We propose an approach to constructing synthetic OV datasets from real-world OM datasets. Figure~\ref{fig: dataset-construction} illustrates the generation of OM4OV datasets.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth]{qiang-tgdk-figures/OV-Testbed.png}
\caption{Generation of OM4OV datasets from initial OM inputs of a source ontology, a target ontology, and a reference alignment, and outputs of versioning ontologies and reference alignments with four categories. Optionally, a reference ontology and a replacement corpus may be produced.}
\label{fig: dataset-construction}
\end{figure}

\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item The original OAEI datasets for OM provide two ontologies, the \textit{source} $O_s$ and the \textit{target} $O_t$. We choose either one as the ontology for versioning and duplicate it into $O$ and $O'$. Another ontology will be used later to provide references for synthetic \textit{update} entities. We duplicate this ontology into $O_r$.
\item There are four possible entity changes in OV tasks: \textit{remain}, \textit{update}, \textit{add}, and \textit{delete}. We retrieve all ontology entities from $O$ or $O'$ (since they are identical at this stage). Each ontology entity will be randomly assigned to one of these categories, and the four sets are pairwise disjoint by construction. In real-world OV, entity updates are relatively infrequent. We allow a user-defined parameter to fix the proportion of update entities in the synthetic dataset, defaulting to 25\%. The update entities are randomly selected from the replacement corpus, so the number of update entities is limited by the size of the replacement corpus, which may be less than the user-defined parameter value. For this reason, selection of update entities is prioritised over other categories, and excess entities are redistributed evenly over the other three categories.
\item For each ontology entity $e$ assigned to a category, the corresponding dataset operations are described as follows. While there is no operation for \textit{remain} entities, entities assigned to \textit{add} and \textit{delete} are deleted from all triples that mention them in $O$ or $O'$ respectively. Each \textit{update} mapping requires that all occurrences of its domain entity in triples in $O'$ are replaced by the corresponding co-domain entity of the mapping. We generate four corresponding versioning references based on the entity assignments. These files provide the ground truth for evaluation.
\end{enumerate}

To ensure the replaced entity is reasonable and reflects real-world facts, we use equivalent classes or properties specified in the reference alignment. For example, we could replace \texttt{cmt:ProgramCommitteeChair} with its equivalent class \texttt{confof:Chair\_PC}. This operation is cascaded, meaning that we update not only the entity name but also its related triples, such as changing the semantic information from \texttt{(cmt:ProgramCommitteeChair, rdfs:subClassOf, cmt:ProgramCommitteeMember)} to \texttt{(confof:Chair\_PC, rdfs:subClassOf, confof:Person)}. While this procedure can be unlimited, we restrict it to extract only the triples directly related to the entity (i.e. a 1-hop subgraph) in the ontology $O_r$. For entities whose names are unique identifiers or codes (and not textually meaningful names), we retrieve their meaningful descriptions from annotation properties. For example, we extract an additional annotation triple \texttt{(mouse:MA\_0000270, rdfs:label, ``eyelid tarsus'')} for the entity \texttt{mouse:MA\_0000270}. After extraction, we also need to update the prefix from  \textit{``confof''} to \textit{``cmt''} where the new entity URI will be \texttt{cmt:Chair\_PC} and the replacement triple will be \texttt{(cmt:Chair\_PC, rdfs:subClassOf, cmt:Person)}. Finally, we add these new triples to the existing ontology $O'$. Note that where entity names do not change but structural changes have been made near the entity, this will be represented as an entity update. Table~\ref{tab: dataset-update} summarises the steps to construct an \textit{update} entity $e$ in the benchmark dataset.

\begin{table}[htbp]
\centering
\caption{Steps to construct an \textit{update} entity $e$ in the benchmark dataset.}
\label{tab: dataset-update}
\begin{tabular}{|c|l|}
\hline
\multirow{1}{*}{\textbf{Step}}  & \multirow{1}{*}{\textbf{Dataset Operation}}                               \\ \hline
\multicolumn{1}{|c|}{\#1}       & Remove all the triples related to $e$ in $O'$.                            \\ \hline
\multicolumn{1}{|c|}{\#2}       & Find the equivalent class/property $e_r$ in \textit{replacement corpus}.  \\ \hline
\multirow{2}{*}{\#3}            & Extract all the triples related to $e_r$ in $O_r$.                        \\ \cline{2-2}
& (Optional) Extract annotation triples related to $e_r$ in $O_r$.                                          \\ \hline
\multicolumn{1}{|c|}{\#4}       & Update the prefix from $e_r$ to $e$ and create a new entity $e'$.         \\ \hline
\multicolumn{1}{|c|}{\#5}       & Add all the triples related to $e'$ to $O'$.                              \\ \hline
\end{tabular}
\end{table}

\newpage

Unlike the original OAEI datasets used for OM, we introduce randomness to ensure that the synthetic OAEI datasets for OV are different each time they are constructed. This suits the dynamic nature of OV, where the changes vary between different versions. For this reason, we consider the new OAEI datasets for OV more like a testbed, as they can simulate a variety of situations for OV tasks. When reproducibility is required, we recommend using a fixed seed to control the randomness.

Table~\ref{tab: ov-testbed} details the OAEI tracks selected for the OV testbed. The current version of the OV testbed contains a total of 11 distinct ontologies from three different OAEI tracks. The anatomy track contains two large ontologies, while the MSE track has two medium ontologies, and the conference track has 7 small ontologies. We exclude EMMO~\citep{emmo} from the MSE track because it assigns opaque symbolic codes to entity names, using a naming convention that differs from MaterialInformation~\citep{ashino2010materials} and MatOnto~\citep{matonto}, which use meaningful entity names. Figure~\ref{fig: ov-testbed} shows the number of entities in each ontology in each track.

\noindent
\begin{minipage}[t]{0.65\textwidth}
\centering
\captionof{table}{Selected OAEI tracks for the OV testbed.}
\label{tab: ov-testbed}
\adjustbox{width=\textwidth, valign=t}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{|c|c|c|}
\hline
\multirow{1}{*}{\textbf{Track}}     & \multirow{1}{*}{\textbf{Domain}}  & \multirow{1}{*}{\textbf{\# of Ontologies}}    \\ \hline
\multicolumn{1}{|c|}{Anatomy}       & Human and Mouse Anatomy           & 2                                             \\ \hline
\multicolumn{1}{|c|}{Conference}    & Research Conference               & 7                                             \\ \hline
\multicolumn{1}{|c|}{MSE}           & Materials Science and Engineering & 2                                             \\ \hline
\end{tabular}
}
\end{minipage}
\begin{minipage}[t]{0.34\textwidth}
\centering
\captionof{figure}[Number of entities in each ontology in each track.]{\# of entities in each ontology in each track.}
\label{fig: ov-testbed}
\adjustbox{valign=t}{
\includegraphics[width=1\linewidth]{qiang-tgdk-figures/Ontology-Metadata.png}
}
\end{minipage}

\subsection{Evaluation System}
\label{sub-sec: evaluation-system}

We choose the matching system Agent-OM and its extended version Agent-OV to demonstrate the OM4OV framework. Agent-OM is one of the flagship OM systems powered by large language models (LLMs) and multi-agent architectures. Its foundation framework is designed for traditional OM tasks. We extend Agent-OM with the OM4OV framework so that it can be used for OV tasks. Inherited from Agent-OM, Agent-OV supports a wide range of LLMs, including commercial API-accessed LLMs OpenAI GPT~\citep{llm-gpt} and Anthropic Claude~\citep{llm-claude}, as well as open-source LLMs Meta Llama~\citep{llm-llama}, Alibaba Qwen~\citep{llm-qwen}, Google Gemma~\citep{llm-gemma}, and ChatGLM~\citep{glm2024chatglm}. Inherited from  Agent-OM, $similarity\_threshold$ and $top@k$ are the adjustable key hyperparameters for Agent-OV.

As an aside, we observe that confidence scores for successful matches as determined by OM systems may be unhelpful for direct use in OV for distinguishing \textit{remain} entities from \textit{update} entities. This is because, in practice,  the confidence boundary to best distinguish  \textit{remain} and \textit{update} entities varies in different domains and datasets. In Agent-OV, we handle this problem in the following way. A matched entity is determined to be a \textit{remain} entity when its syntactic name and lexical descriptions are unchanged. Otherwise it is determined to be an \textit{update} entity.  We observe that this approach means that Agent-OV usually considers entities to be \textit{remain} entities when they have structural changes but conserve syntactic names and lexical descriptions. This approach will tend to consider ambiguous entities as \textit{remain} in preference to \textit{update}, so tending to trade off performance in \textit{remain} versus performance in \textit{update}. While other OV systems may handle this differently, we propose that all OM4OV systems could benefit from this approach to partitioning successful matches into \textit{remain} entities and \textit{update} entities.

\subsection{Evaluation Criteria}
\label{sub-sec: evaluation-criteria}

OM typically measures performance using precision, recall, and the F1 score. Given a gold standard reference (R) and a system-discovered alignment (A), precision measures matching correctness and recall measures matching completeness, while F1 score offers a harmonic mean to balance correctness and completeness. OV can reuse these measures, but they need to be extended into four sub-measures for add, delete, remain, and update performance. While an OV method will trade off performance over each of these sets, an OV application problem may well prioritise accuracy on some over others.
\begin{equation}
\begin{aligned}
Precision = \frac{|A \cap R|}{|A|} \quad Recall = \frac{|A \cap R|}{|R|} \quad F_1 \ Score= \frac{2}{Precision^{-1} + Recall^{-1}}
\end{aligned}
\end{equation}

\subsection{Results}
\label{sub-sec: results}

We choose to use the Meta open-source model llama-3-8b~\citep{llama-3-8b} for our experiments in this study, eschewing the higher-end models that offer small improvements that may not justify the financial investment. We use embeddings from the same LLM model to further avoid expensive API calls and thereby provide an entirely free-to-use version of Agent-OV. The hyperparameter settings are $similarity\_threshold = 0.90$ and $top@k = 3$ across all the system alignments generated. We set $top@k = 3$ based on empirical experience that 3-5 works well for Agent-OM. We experiment with the alternative values of the similarity threshold later in this study. The fixed seed for the OV testbed is set to 42. Due to the non-determinism of LLMs, repeated experiments can produce insignificantly different results.

Figure~\ref{fig: evaluation-conference} shows the performance of Agent-OM and Agent-OV on the OAEI Conference Track. The results indicate that it is possible to unify the OM and OV tasks using the OM4OV framework. Both Agent-OM and Agent-OV can produce alignments with precision, recall, and F1 scores. However, we can see that Agent-OM consistently performs surprisingly well across all alignments. This is because the traditional OM system captures only matched entities between two ontologies, which in the OV task correspond to the \textit{remain} and \textit{update} entities. Because \textit{remain} entities typically comprise the major proportion of entities over two different versions, the correctness of \textit{remain} entities dominates the overall evaluation and other categories are de-emphasised. We believe this is a common situation that leads to misleading performance measurement when using an OM system in OV tasks.

Agent-OV overcomes the skewed measure in Agent-OM. By decomposing the measure into four sub-measures, we can observe more informative matching performance across different OV tasks. In general, we observe that the matching performance is highest in \textit{remain}, followed by \textit{add} and \textit{delete}, and relatively low in \textit{update}. This trend is consistent across different tracks and ontologies. The measures for \textit{remain} are typically very close to 100\%. The measures for \textit{add} and \textit{delete} are generally good. Our system uses LLMs as the backend, and LLMs generally have strong background knowledge to detect non-matched entities. The measures for \textit{update} show scope for improvement. This is because finding non-trivial alignments and appropriate similarity thresholds is not easy. We examine the false mappings produced by Agent-OV. Unlike OM tasks, we find that some of these identified false mappings are not actually false. Several examples are listed below with explanations.

\begin{figure}[!t]
\centering
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-conference-cmt.png}
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-conference-conference.png}
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-conference-confof.png}        \\
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-conference-edas.png}
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-conference-ekaw.png}          \\
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-conference-iasted.png}
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-conference-sigkdd.png}        \\
\caption{Evaluation of OAEI Conference Track on the OV testbed. Agent-OM, shown as a red star, determines only the single category of entity matches. The extended Agent-OV, shown as triangles, determines four different categories of entity matches (\textit{remain} or \textit{update}) and non-matches (\textit{add} or \textit{delete}).}
\label{fig: evaluation-conference}
\end{figure}

\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item False mappings in OV can result from flawed ontology design choices.
\begin{lstlisting}
(edas:ConferenceEvent, edas:Event, c)
(edas:ConferenceEvent, edas:AcademicEvent, c)
\end{lstlisting}
In the example, the reference shows \texttt{edas:ConferenceEvent} is updated to \texttt{edas:Event}, but the OV system predicts \texttt{edas:ConferenceEvent} is updated to \texttt{edas:AcademicEvent}. An event can be a non-academic event (e.g. a social event) or an academic event (e.g. a seminar). In the context of a research conference, a conference event is more likely to mean the latter. However, mapping to event still makes sense. Within one ontology, the meaning of two entities is too close to be distinguished and therefore leads to them being synonyms for each other. Ideally, we should avoid this type of ontology design. This example also demonstrates a unique benefit of using OM for OV, which could potentially assist in ontology design.
\item False mappings in OV can create ambiguous ``equivalent'' relationships.
\begin{lstlisting}
(confof:dealsWith, confof:hasSubjectArea, c)
(confof:dealsWith, confof:reviewes, c)
\end{lstlisting}
In the example, the reference shows \texttt{\small confof:dealsWith} is updated to \texttt{\small confof:hasSubjectArea}, but the OV system predicts \texttt{confof:dealsWith} is updated to \texttt{confof:reviewes}. This is not necessarily wrong, but it interprets ``deal with'' differently. It is vital to notice that the term ``equivalent'' in OV is weaker than that in OM. OV allows for roughly ``equivalent'' mappings. The entities mapped in OV can slightly alter their meanings in response to real-world changes in the domain or evolution of natural language.
\item False mappings in OV can arise from different similarity thresholds.
\begin{lstlisting}
(sigkdd:Start_of_conference, None, 0.90)
(sigkdd:Start_of_conference, sigkdd:startDate, 0.80)
\end{lstlisting}
In the example, if $similarity\_threshold = 0.90$, \texttt{sigkdd:Start\_of\_conference} in $O$ will be assigned to \textit{delete} entities as it does not have matching entities; if $similarity\_threshold = 0.80$, \texttt{sigkdd:Start\_of\_conference} in $O$ will be assigned to \textit{update} entities as it has a matching entity \texttt{sigkdd:startDate} in $O'$. Both results are valid because defining the boundary between matching and non-matching is context- and application-dependent. For example, the similarity threshold could be relatively higher in the biomedical domain to ensure that each term is unique, whereas the similarity threshold in the conference domain could be relatively lower to improve the interoperability of terminologies used in research conferences.
\end{enumerate}

We extend our analysis to other OAEI tracks and varying similarity thresholds. Figure~\ref{fig: evaluation-other} shows that the trends are consistent with other medium and large OAEI tracks evaluated on the OV testbed. Additionally, we observe a longer computation time in the Anatomy Track. Although Agent-OV has an optimisation module for the matching candidate selection process (inherited from Agent-OM), it is still insufficient for some OV tasks. There is a need to optimise the framework for OV in large-scale ontologies. Figure~\ref{fig: evaluation-similarity-without-cr} studies the effect of varying similarity thresholds for the Mouse ontology in Agent-OV. We change the similarity threshold from 1.00 to 0.80 to evaluate its effect on matching performance. While OV entities are classified into four different categories, each category requires a corresponding sub-measurement. Similar to OM tasks, changes in hyperparameter settings in OV tasks lead to a trade-off between precision and recall. Moreover, the hyperparameter settings also influence the sub-measures. We find that the similarity threshold has no effect on detecting \textit{remain} entities, but significantly affects the detection of \textit{update} entities and slightly affects the detection of \textit{add} and \textit{delete} entities. Detecting \textit{update} entities and detecting \textit{add} and \textit{delete} entities are negatively correlated, as is expected because a near-miss \textit{update} alignment will fall back to a pair of \textit{non-match} entities, one from each ontology. Therefore, lower similarity thresholds can result in more \textit{update} entities being detected, while higher similarity thresholds may find more \textit{add} and \textit{delete} entities.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-anatomy-human.png}
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-anatomy-mouse.png}    \\
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-mse-MatInfo.png}
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-mse-MatOnto.png}      \\
\caption{Evaluation of OAEI Anatomy and MSE Tracks on the OV testbed.}
\label{fig: evaluation-other}
\end{figure}

\begin{figure}[!t]
\includegraphics[width=1\linewidth]{qiang-tgdk-figures/similarity-cross-reference-False.png}
\caption{Evaluation of varying similarity thresholds in Agent-OV. We apply a 1-D Gaussian filter for smoothing. The standard deviation for a Gaussian kernel is 1 (i.e. $sigma=1$). The similarity threshold has no effect on detecting \textit{remain} entities in the top row, but affects the detection of \textit{update}, \textit{add}, and \textit{delete} entities.}
\label{fig: evaluation-similarity-without-cr}
\end{figure}

\subsection{Discussion}

The experimental results have shown that OM systems can be reused for OV tasks, but they have limitations and require necessary extensions. The following key points need to be taken into account when reusing OM systems for OV tasks.
\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item \textbf{Skewed Measurement:} OM systems exhibit skewed measurement of OV tasks because unchanged \textit{remain} entities dominate in practice. OM measures are reusable, but these measures need to be extended into four sub-measures for \textit{add}, \textit{delete}, \textit{remain}, and \textit{update} performance. Within each sub-measure, the inherent precision-recall trade-off still holds. Across different sub-measures, they are not independent. This is because each change in a part of an alignment in one category will cause other categories to change accordingly. For example, if a new mapping is found in $A\odot$ or $A\otimes$, then the number of mappings in $A\oplus$ and $A\ominus$ will be reduced by one each, and vice versa.
\item \textbf{Update Pitfalls:} OM systems are sensitive to changes in similarity thresholds and backend LLMs. For OV tasks, only \textit{update} entities are sensitive to these changes, while \textit{remain}, \textit{add}, and \textit{delete} are relatively stable across these hyperparameter settings. Poor \textit{update} performance is common, while tuning the similarity threshold trades precision for recall without resolving the underlying difficulty.
\item \textbf{Disputed False Mappings:} OM systems used for OV tasks can produce mappings that are false with respect to ground truth references, but that are true with respect to expert review. This can be caused by flawed ontology design choices, ambiguous ``equivalent'' relationships, or inappropriate similarity threshold settings. This is difficult for OM systems to recognise and generally requires human effort.
\end{enumerate}

\section{OM4OV Optimisation}

Having established the current pitfalls of OM4OV, we explore optimisations for the framework. Often, ontology creators provide cross-references to alternative ontologies to enhance interoperability and facilitate integration. For example, a cross-reference between the Mouse ontology and the Human ontology is provided in the OAEI Anatomy Track. Reusing the cross-references developed for OM tasks, we propose a novel mechanism to reduce the number of matching candidates and also to improve overall OV performance.

Figure~\ref{fig: om4ov-extend} illustrates the cross-reference (CR) mechanism used in the OM4OV framework. We can see that, without using the cross-reference $O_r$, the matching candidates cover the range of $O\cup O'$. This number can be significantly reduced by removing prior matches (i.e. $O \cap O_r \cap O'$) and non-matches (i.e. $ O\cap O_r \setminus O'$ and $O' \cap O_r \setminus O$). The prior matching will be incorporated into the final alignment, while the known non-matching regions will be removed entirely in the subsequent OV process. The OV process then only determines the posterior alignment.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.6\linewidth]{qiang-tgdk-figures/Cross-Reference.png}
\caption{Illustration of the cross-reference (CR) mechanism.}
\label{fig: om4ov-extend}
\end{figure}

In practice, the prior alignment usually contains a large number of \textit{remain} entities and a small number of \textit{update} entities. Matching performance is also enhanced by utilising these established mappings. Since prior matches are inferred from OM references validated by domain experts, they provide a solid ground truth for alignment within a specific domain. Removing known non-matches from the OV process also simplifies posterior alignment detection. The optimised OM4OV framework using the CR mechanism is defined as follows.
\begin{definition}
Given a reference ontology ($O_r$), an old version of an ontology ($O$) and a new version of the same ontology ($O'$), two cross-references between $O$ and $O_r$ ($R_{or}$) and between $O'$ and $O_r$ ($R_{o'r}$) are defined respectively as:
\begin{equation}
\begin{aligned}
R_{or}  &= \{(e_1, e_3, c) \mid e_1 \in O, e_3 \in O_r, s \leq c \leq 1 \mbox{ and there is no } (e_1,e_3,c')\mbox{ with } c'> c\}    \\
R_{o'r} &= \{(e_2, e_3, c) \mid e_2 \in O', e_3 \in O_r, s \leq c \leq 1 \mbox{ and there is no } (e_2,e_3,c')\mbox{ with } c'> c\}   \\
\end{aligned}
\end{equation}
\end{definition}

We can use $R_{or}$ and $R_{o'r}$ to infer some known mappings between $O$ and $O'$ before performing OV. We call these mappings a \textit{prior} alignment ($A_{\pi}$). After subsequently performing OV, we have our \textit{posterior} alignment ($A_{\pi^*}$). In this setting, $A_{match}$ in OV can be decomposed into two parts: $A_{match} = A_{\pi} \cup A_{\pi^*}$. $A_{\pi}$ can be directly inferred from the two cross-references $R_{or}$ and $R_{o'r}$. By assuming the equivalence relation as extracted from the two cross-references is transitive, we have that $e_1 \in O$, $e_2 \in O'$, and $e_3 \in O_r$, if $e_1 \equiv e_3$ and $e_2 \equiv e_3$ then $e_1 \equiv e_2$. $A_{\pi^*}$ aims to detect missing mappings from the cross-reference. None of these mappings would come from any pairwise intersection of $O$, $O_r$, and $O'$ because $O \cap O_r \setminus O'$ and $O' \cap O_r \setminus O$ are pre-defined as non-matched entities, and the matched entities in $O\cap O_r \cap O'$ have been captured in the $A(\pi)$. As a result, $A_{\pi^*}$ can be defined within a smaller scope.
\begin{definition}
\textit{Prior} alignment ($A_{\pi}$) and \textit{posterior} alignment ($A_{\pi^*}$) are defined as:
\begin{equation}
\begin{aligned}
A_{\pi} &= R_{or} \cap R_{o'r} = \{(e_1, e_2, c) \mid e_1, e_2 \in O \cap O_r \cap O', s \leq c \leq 1\}    \\
A_{\pi^*} &= \{(e_1, e_2, c) \mid e_1 \in O\setminus O_r, e_2 \in O' \setminus O_r, s \leq c \leq 1\}       \\
\end{aligned}
\end{equation}
\end{definition}

An ontology can have multiple cross-references available. In such cases, the \textit{prior} reference becomes the union of all known cross-references ($R_{or1}$ ... $R_{orn}$), and the ontology used in the \textit{posterior} alignment ($O_{ra}$) becomes the union of all reference ontologies ($O_{r1}$ ... $O_{rn}$).
\begin{definition}
$A_{\pi}$ and $A_{\pi^*}$ in multiple cross-references can be formulated as:
\begin{equation}
\begin{aligned}
A_{\pi} &= (R_{or1} \cap R_{o'r1}) \cup (R_{or2} \cap R_{o'r2}) \cup ...\cup (R_{orn} \cap R_{o'rn}) \\
A_{\pi^*} &= \{(e_1, e_2, c) \mid e_1 \in O\setminus O_{ra}, e_2 \in O' \setminus O_{ra}, c \geq s\} \ \text{where} \ O_{ra} = O_{r1} \cup O_{r2} \cup... O_{rn} \\
\end{aligned}
\end{equation}
\end{definition}

Figure~\ref{fig: evaluation-cr} compares the OV performance with and without the CR mechanism on the same OV testbed that we analysed in Section~\ref{sec: evaluation}. We can see that the CR mechanism significantly enhances Agent-OV's ability to detect \textit{update} entities and slightly improves its performance in detecting \textit{add} and \textit{delete} entities, with no effect on \textit{remain} entities. More specifically, performance improvement is mainly attributed to recall for \textit{update} entities, whereas it is more evident in precision for \textit{add} and \textit{delete} entities. Figure~\ref{fig: evaluation-similarity-with-cr} compares the effects of different similarity thresholds for the Mouse ontology versioning. The results of the experiment show that the CR mechanism is less sensitive to the similarity threshold than the original OM4OV framework in Figure~\ref{fig: evaluation-similarity-without-cr}, suggesting that it can be helpful in scenarios where the optimal similarity threshold is unclear or difficult to determine.

\begin{figure}[!t]
\includegraphics[width=1\linewidth]{qiang-tgdk-figures/optimise-remain.png}
\includegraphics[width=1\linewidth]{qiang-tgdk-figures/optimise-update.png}
\includegraphics[width=1\linewidth]{qiang-tgdk-figures/optimise-add.png}
\includegraphics[width=1\linewidth]{qiang-tgdk-figures/optimise-delete.png}
\caption{Evaluation of the cross-reference (CR) mechanism on the OV testbed. Each radar chart shows measurements (precision, recall, and F1 score) for a change category over 11 datasets analysed around the perimeter, both with (\textit{orange}) and without (\textit{blue}) the CR mechanism applied.}
\label{fig: evaluation-cr}
\end{figure}

\begin{figure}[!t]
\includegraphics[width=1\linewidth]{qiang-tgdk-figures/similarity-cross-reference-True.png}
\caption{Evaluation of the cross-reference (CR) mechanism on different similarity thresholds. The solid lines contribute to OV performance with the CR mechanism, while the dotted lines contribute to OV performance without the CR mechanism. We apply a 1-D Gaussian filter for smoothing. The standard deviation for a Gaussian kernel is 1 (i.e. $sigma=1$).}
\label{fig: evaluation-similarity-with-cr}
\end{figure}

\section{OM4OV in Real-World Applications}
\label{sec: application}

Brick Schema~\citep{balaji2016brick} is a popular ontology used in the building industry. Introduced in 2016, Brick Schema has undergone several major version changes, including URI changes, schema language changes, and ontology harmonisation (combining Brick Schema with RealEstateCore~\citep{hammar2019realestatecore} and Project Haystack~\citep{john2020project}). We use the change logs from the official GitHub repository to provide near-ground-truth alignments for evaluation. We are not confident about the reliability of the manually-generated logs as we observe instances where the log entry for a change conflicts with the difference observed in the ontology itself. We demonstrate versioning performance over three distinct major version updates: from v1.1.0 to v1.4.0, v1.2.0 to v1.4.0, and v1.3.0 to v1.4.0. We have collapsed multiple human-identified minor version changes into the corresponding major version changes for our experiments to consider more complex version changes than are evident in successive minor versions. We filter out classes and properties that are used in Brick Schema conventions but that user experts determined to be unimportant for version tracking and hence have not been captured in change logs. For example, ``Tag'', ``NodeShape'', and ``PropertyShape'' are excluded from the matching candidates.

Figure~\ref{fig: evaluation-brick} shows that our OM4OV implemented in the OM system is more precise than our previous OM-only system in tracking changes across different versions of Brick Schema. Similar trends are observed in skewed measurements, update pitfalls, and disputed false mappings. We are unable to empirically evaluate our cross-reference mechanism with Brick Schema. Unfortunately, while Brick Schema offers high-level alignments with RealEstateCore and Project Haystack, these alignments are highly incomplete, addressing only few classes and properties. Further, they do not indicate versions of the ontologies to which they apply. We have been unable to locate an alternative ontology that offers the data needed for evaluating our cross-reference mechanism. We hope our work contributes to the quality improvement of OV so that building high-quality versioned reference alignments becomes standard industry practice. At that time, automated system updates with respect to ontology version changes would become feasible, and we could evaluate our cross-reference mechanism on real-world data.

\begin{figure}[!t]
\centering
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-building-brick-v1.1.0-v1.4.0.png}
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-building-brick-v1.2.0-v1.4.0.png}
\includegraphics[width=0.325\textwidth]{qiang-tgdk-figures/result-building-brick-v1.3.0-v1.4.0.png}
\caption{Using the OM4OV framework to track Brick Schema version changes.}
\label{fig: evaluation-brick}
\end{figure}

\section{Conclusion}

In this chapter, we systematically analyse similarities and differences between OM and OV tasks and provide formal definitions and task formulations for OM4OV. The experimental results from Agent-OM and Agent-OV demonstrate that the OM4OV framework is workable, though it presents several limitations. To tackle these issues, we propose a novel optimisation method that uses a cross-reference (CR) mechanism to leverage reference alignments from OM for OV. This method (1) overcomes several pitfalls in using OM for OV tasks, (2) significantly reduces the number of matching candidates, and (3) improves overall OV performance. We showcase the use of our OM4OV framework in tracking version changes in a widely used ontology for the building industry.

OM and OV are useful automated techniques to align concepts from  different ontologies. To improve the matching, in the next chapter we turn to validating the matching output--taking account of human preference. We follow in the subsequent chapter with further validation via real-world instance data.

\newpage

\paragraph*{Supplementary Material Statement}\mbox{}

The following supplementary materials belong to this study:\smallskip
\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(S\arabic*)]
\item
\emph{Software (OM4OV and Agent-OV):} {\small \url{https://github.com/qzc438/ontology-versioning}}. This artifact contains source code for OM4OV and Agent-OV, as well as the versioning datasets mentioned
in Section~\ref{sub-sec: dataset-construction}.
\item\emph{Software (Brick Schema Version Track):}
{\small \url{https://github.com/qzc438/brick-version-track}}. This artifact contains the source code for tracking Brick Schema~\citep{balaji2016brick} version changes mentioned in Section~\ref{sec: application}.
\end{enumerate}
\smallskip
The following resources were used in the mentioned parts of the study:\smallskip
\begin{enumerate}[wide, itemsep=0pt, topsep=0pt, labelindent=0pt, label=(R\arabic*)]
\item \emph{Software (Agent-OM)~\citep{github-R1}:} {\small \url{https://github.com/qzc438/ontology-llm}}. This artifact contains the source code for Agent-OM~\citep{qiang2023agent} mentioned in Sections~\ref{sub-sec: evaluation-system} and~\ref{sub-sec: results}.
\item \emph{Dataset (OAEI Datasets)~\citep{github-R2}:} {\small \url{https://dwslab.github.io/melt/track-repository}}. This artifact shows the Matching EvaLuation Toolkit (MELT)~\citep{hertling2019melt} repository to download
the original OAEI datasets for (S1) (retrieved April 1, 2025). According to the OAEI data policy, ``OAEI results and datasets, are publicly available, but subject to a use policy similar to \href{https://trec.nist.gov/results.html}{the one defined by NIST for TREC}. These rules apply to anyone using these data.'' Please find more details from the official website: \url{https://oaei.ontologymatching.org/doc/oaei-deontology.2.html} (retrieved April 1, 2025).
\item \emph{Dataset (Brick Schema Change Logs)~\citep{github-R3}:} {\small \url{https://github.com/BrickSchema/Brick/releases}}. This artifact shows the link to the Brick Schema~\citep{balaji2016brick} official repository to download the change logs for (S2) (retrieved April 1, 2025).
\end{enumerate}

\paragraph*{Publication Statement}

Most of the work presented in this chapter has been published as~\bibentry{qiang2024om4ov}.

==> qiang-anu-thesis-content/qiang-anu-thesis-case-study.tex <==
\section[Case Study]{A Case Study in the Building Industry}

Driven by the emergence of efficient digital transformation for Industry 4.0, numerous building ontologies have been developed over the past two decades. While building concepts are complex and evolve rapidly, ontology interoperability has become a prominent problem in the building domain. Ontologies used in the building domain encompass diverse concepts and levels of abstraction, and building information systems based on these ontologies face communication hurdles.

We use a running example to illustrate the application and value of our proposed framework for ontology interoperability. The running example concerns sensor observations in the building, for example, ``A sensor is installed in the room to monitor the room temperature.'' The ontologies used in this case are required to capture several main concepts, including sensor, room, temperature, and sensor observation. In the real world, building such an ontology requires considerable effort. The proposed ontology should capture all concepts without overlap or omission; moreover, it should be compact and easy to migrate to another ontology if the system's vendors change over the years.

\subsection{ODPs in the Design Phase}

Ontologies can be built from scratch, but such ontologies are likely to have more customised concepts and limited interoperability. It is commonly recommended to reuse pre-existing ODPs. Figure~\ref{fig: observation} illustrates that four classical ODPs can be used in this case to model the example of sensor observation from different perspectives.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item \textit{Observation Pattern} (used in SOSA~\citep{janowicz2019sosa} and SSN~\citep{compton2012ssn}). Sensor observation is defined as a type of observation. The observation is made by the sensor, which has a feature of interest in the room and the observed property temperature.
\item \textit{Measurement Pattern} (used in the early version of SAREF~\citep{daniele2015created}). Sensor observation is defined as a measurement. The measurement is made by the sensor, which is a measure of the room related to the property temperature.
\item \textit{Event Pattern} (used in DUL~\citep{presutti2016dolce+}). Sensor observation is defined as an event. The event is associated with the sensor, room, and temperature.
\item \textit{Activity Pattern} (used in PROV-O~\citep{w3c-prov}). Sensor observation is defined as an activity. The activity is associated with the sensor that uses the room and generates a temperature measurement.
\end{enumerate}

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{qiang-iswc-2026-dc-figures/ODP-Observation.png}
\caption{Modelling sensor observation using different ODPs.}
\label{fig: observation}
\end{figure}

While all four of these ODPs can effectively capture the main concepts, significant differences in perspective need to be considered, as shown below.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item The definitions of the concepts can differ. Temperature is defined as a property of the room in both the \textit{Observation Pattern} and the \textit{Measurement Pattern}, but in the \textit{Event Pattern} it is treated as a quality measure of the room. \textit{Activity Pattern} defines the temperature as a member of the room.
\item The levels of expressiveness are different. Unlike \textit{Observation Pattern}, \textit{Measurement Pattern}, and \textit{Activity Pattern}, which can only describe a sensor that is installed in the room, the \textit{Event Pattern} can distinguish between a structural attachment (i.e. isPartOf) and a spatial presence (i.e. isLocatedIn).
\end{enumerate}

\subsection{OM\&OV in the Develop Phase}

We assume that the \textit{Observation Pattern} is chosen in the design phase and implemented in two ontologies, SOSA and the original SSN~\citep{compton2012ssn,old-ssn} (also called the old SSN in the W3C standard~\citep{w3c-ssn}). As illustrated in Figure~\ref{fig: ssn&sosa}, SOSA and SSN are very similar because they are built from the same ODPs. However, they are not exactly the same. The OM task is to identify aligned concepts across two ontologies. SOSA and an updated SSN were co-developed, with a published alignment between them. SOSA was conceived as a module of the updated SSN (for which there were other modules too). If we consider SOSA to be an updated and reduced version of SSN, then this OM task is also an OV task. We use OM\&OV here because OM and OV can be unified with minor modifications. OM\&OV tasks have two categories.

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{qiang-iswc-2026-dc-figures/OM-OV-SOSA-SSN.png}
\caption{Aligning SOSA and SSN.}
\label{fig: ssn&sosa}
\end{figure}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item Finding trivial alignments only considers the syntactic matching of the entity name. For example, the mappings between the classes \textit{sosa:Sensor} and \textit{ssn:Sensor}, and the properties \textit{sosa:madeBySensor} and \textit{ssn:madeBySensor} are trivial. We also refer to these mappings as ``seed mappings'' because they serve as the basis for subsequent lexical and semantic matching.
\item Finding non-trivial alignments considers syntactic, lexical, and semantic matching of the entity. For example, the mappings between the classes \textit{sosa:ObservableProperty} and \textit{ssn:Property}, and the properties \textit{sosa:isHostedBy} and \textit{ssn:onPlatform} should be discovered. The alignment should also exclude non-existent and counter-intuitive mappings. For example, \textit{ssn:hasProperty} does not have a direct equivalent mapping in SOSA.
\end{enumerate}

\subsection{OVA in the Deploy Phase}

While the mappings developed by the OM systems are not 100\% reliable, additional human validation is required. A number of experts will sit together to determine whether these mappings are correct. This procedure can be conducted in surveys, interviews, and workshops.

Assume we have developed a validated reference alignment for SOSA and SSN. We now face the question of which ontology of SOSA and SSN should we use in real-world KGs? Some concepts used in a KG may not have the corresponding classes and properties in the chosen ontology. Therefore, we apply these two ontologies separately to the KGs and construct ontology-compliant knowledge graphs (OCKGs) for evaluation. The introduction of OCKGs is a novel DOVA approach that uses a pay-as-you-go model to find the most cost-effective ontology fragment that matches the given KGs. Figure~\ref{fig: ockg-sosa-ssn} shows how OCKGs based on SOSA and SSN can evaluate the utility of SOSA vs SSN. We can see that both ontologies can capture the general concepts of this sensor observation; however, they fail to capture two specific concepts in the given KG.

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{qiang-iswc-2026-dc-figures/OCKG-SOSA-SSN.png}
\caption{Build OCKGs using SOSA and SSN.}
\label{fig: ockg-sosa-ssn}
\end{figure}

\newpage

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item The stimulus of the sensor ``Exceeds 25 Degrees''. The sensor only makes an observation when the temperature exceeds 25 degrees.
\item The actual feature of interest ``Building 001''. The sensor observed the temperature of Room 001. It is not a feature of interest, but a sample of the temperature of Building 001.
\end{enumerate}

To model these two new concepts and adequately integrate them with the other parts of a KG, we need to extend the ODP with the \textit{Stimulus-Sensor-Observation Pattern} from SSN and the \textit{Sampling Pattern} from SOSA, as well as make several design choices between aligned mappings (retrieved from~\citep{w3c-ssn,haller2018modular,taylor2019semantic}).

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item We use \textit{ssn:Property} to replace \textit{sosa:ObservableProperty} because this class is more general and can be applied in a broader context for sensing, including actuation and sampling.
\item We use \textit{sosa:isHostedby} to replace \textit{ssn:onPlatform} because this property is more closely related to describing a sensor physically installed in the room.
\item We use \textit{sosa:hasFeatureOfInterest} to replace \textit{ssn:FeatureOfInterest}. Although there is no restriction for \textit{ssn:FeatureOfInterest} to be used both as a class and as a property, we add the verb ``has'' to distinguish the property from the class for human readability.
\end{enumerate}

Figure~\ref{fig: odp-new} shows the updated ontology and the OCKG built on the updated ontology. It appears that the updated ontology is better suited to the provided KG instance. In industrial scenarios, an ontology can be deployed in multiple KGs, and the procedure described above can be repeated multiple times. It is also possible to choose other alternative ODPs. For example, the class ``BuildingSpace'' in the \textit{Measurement Pattern} is more suitable to describe a room, and the property ``hasLocation/isPartOf'' in the \textit{Event Pattern} is more appropriate to describe the link between the sensor and the room.

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{qiang-iswc-2026-dc-figures/ODP-New.png}
\caption{Updated ontology and new OCKG.}
\label{fig: odp-new}
\end{figure}

\subsection{Implications}

Well-defined ODPs can serve as reusable ontology fragments, thereby reducing the complexity of OM\&OV tasks. As a complement to ODPs, OM\&OV can align detailed classes, properties, and individuals that are not captured by ODPs. On the other hand, while OCKGs are useful tools for validating ontology interoperability and evolving ODPs, their construction relies heavily on precise mappings produced by OM\&OV systems with additional human-in-the-loop validation. OM\&OV is a critical middleware between ODPs and OVA.

\newpage

While there is no preference for one technique over another, these three techniques play different roles in a comprehensive framework for ontology interoperability. We believe that employing ODPs in the design phase, utilising OM\&OV in the develop phase, and using OVA in the deploy phase could significantly improve ontology interoperability throughout the ontology engineering life cycle.

We now move on to present the state-of-the-art of ontology interoperability.

==> qiang-anu-thesis-content/qiang-anu-thesis-conclusion.tex <==
An ontology is designed to achieve semantic interoperability among heterogeneous KGs. However, no ontology is universally applicable. Ontologies are often handcrafted and consistently modified or extended to capture concepts across different domains. This causes an inherent interoperability issue among ontologies, in which concepts may be missing, overlapping, or conflicting. This work introduces a comprehensive framework for ontology interoperability. We believe that ontology interoperability is not achieved in a single stroke but rather through a process. In each stage of the ontology engineering life cycle, the use of an appropriate interoperability technique is indispensable. Our vision for ontology development using our framework runs as follows.

\section{A Guideline for Creating an Interoperable Ontology}

``Ontology Development 101''~\citep{noy2001ontology} is a well-known guideline for creating an ontology. With the growth of the Semantic Web over the last two decades, ontologies have been used in many downstream applications for data integration and knowledge sharing. This introduces a new requirement to build an interoperable ontology that is easy to transfer and reuse in different ontology-driven applications. Building on top of our comprehensive framework for ontology interoperability, we propose ``Ontology Development 102'', a new guideline for creating an interoperable ontology.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item \textbf{Determine domain and scope.} This is an essential step in creating a new ontology. However, we do not expect the competency questions to be complete as we do not create ontology classes, properties, or individuals directly from the competency questions. Instead, competency questions are used to provide a general idea of the domain to facilitate the selection of ODP and ontology candidates.

\item \textbf{Choose an initial ODP.} ODPs can be searched from an ODP corpus, such as \url{https://odpa.github.io/patterns-repository/} (formerly \url{http://ontologydesignpatterns.org}). In practice, a single OPS may not capture all the concepts mentioned in the competency questions, and ODPs can have different levels of abstraction even when they present similar domain concepts. In such cases, it is necessary to integrate multiple ODPs and select ODPs with a suitable level of abstraction based on the competency questions.

\item \textbf{Choose ontology candidates.} Ontology candidates can be searched from the ontology corpus, such as \url{https://ontoportal.org/}. The ontology candidates need to conform to the initial ODP. The ontology candidates that conform to the initial ODPs implicitly conform to the competency questions.

\item \textbf{Find mappings and validate ontology candidates.} This process first uses OM\&OV to align classes, properties, and individuals between ontology candidates. Then, OVA can be used to ensure the mappings are not counter-intuitive and to evaluate the ontology candidates on real KG data.

\item \textbf{Build a new ontology from ontology fragments.} Concepts may be redundant or missing with ontology candidates. In most cases, there is no one ontology that can cover all concepts. We can extract fragments from the ontology candidates and use these ontology fragments to build a new ontology. When merging the ontology fragments, redundant concepts should be removed and missing concepts should be added.

\item \textbf{Revisit and update the initial ODP.} While the new ontology has been validated against the KG data, the initial ODPS should be revisited to update for redundant and missing concepts.

\item \textbf{Iteration process}. Steps (ii)-(vi) can be repeated multiple times until there are no missing or redundant concepts in the updated ODP.

\end{enumerate}

In ``Ontology Development 102'', we suggest creating an ontology not from scratch but by properly referencing existing ODPs and ontologies. This reduces the chance of customised concepts and structural relations being introduced, thereby improving the interoperability of the ontology being created. OM\&OV and OVA provide a solid reference for transferring the ontology from one to another, making it possible for the ontology being created to be interoperable with other downstream applications.

\newpage

\section{Summary of Thesis Contributions}

In Chapter~\ref{chap: literature}, we review the state-of-the-art semantic web technologies for ontology interoperability. While ontology design patterns (ODPs) focus primarily on the conceptual level, ontology matching and validation (OM\&OV) and ontology validation (OVA) focus primarily on the detailed level of mappings between ontology classes and properties. These techniques also employ different paradigms: ODPs and OVA follow a hub-and-spoke matching schema, whereas OM\&OV uses a pairwise matching schema. The characteristics of these techniques are complementary and offer an opportunity to form a framework for ontology interoperability.

In Chapter~\ref{chap: building-odps}, we conduct an empirical study of ODPs in the building industry. We find that there is no one-size-fits-all solution in the building domain and that each of the four building ontologies we analysed has advantages and limitations. Therefore, using ODPs provides a means to address interoperability among systems employing different building ontologies. We propose three distinct building ODPs that span macro-level concepts (e.g. building space and systems) to micro-level concepts (e.g. sensors and measurements).

In Chapters~\ref{chap: agent-om} and~\ref{chap: om4ov}, we focus on OM\&OV. We propose a novel agent-powered LLM-based OM system called Agent-OM. Agent-OM overcomes the limitations of the traditional OM system by relying on pre-defined logic and a pre-built knowledge base. By leveraging LLM agents to access background knowledge and external tools, Agent-OM has demonstrated its ability to handle a wide range of OM tasks. Agent-OV extends Agent-OM for OV tasks. We show that OM and OV can share a unified pipeline, but additional modifications are needed to address skewed measurements, update pitfalls, and false mappings.

In Chapters~\ref{chap: om-validation} and~\ref{chap: ockgs}, we highlight the importance of OVA. We propose a crowdsourced OM validation to align the matching output with human values. With three quality assurance mechanisms, the new system can overcome the limitations of existing crowdsourcing methods in handling the diversity of user groups and system settings. We propose a new paradigm for KGs built from ontologies, the so-called ontology-compliant knowledge graphs (OCKGs) to align matching outputs with data instances. OCKGs not only aim to build ontology-based or ontology-aware KGs but also seek the optimal ontology for given KGs. We present three scenarios in which the ontology needs to fit a single KG, two KGs, or multiple KGs sharing common patterns. OCKGs are useful for ontology selection and decision-making.

While we present our novel approaches to ontology interoperability using semantic web techniques in Chapters~\ref{chap: building-odps}-\ref{chap: ockgs}, we also identify the limitations of each. For example, ODPs are often handcrafted and do not provide detailed mappings between ontology classes and properties; OM\&OV require substantial effort to develop matching systems, and such systems are computationally expensive; and OVA is highly dependent on the output of OM\&OV. Therefore, the appropriate use of each technique at different stages of the OE life cycle is essential to achieve ontology interoperability. We currently position ODPs in the design phase, OM\&OV in the develop phase, and OVA in the deploy phase as the best practice.

\section{Future Work and Broader Directions}

In this section, we outline future work for each component of the ontology interoperability framework. In addition, we present broader directions and future visions for research and impact on ontology interoperability and consequently data integration.

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]

\item \textbf{ODPs for Smart Buildings:} While the evaluation conducted in this study is based on an office building, future work will further the comparison with respect to the capability of extension to other building types, such as commercial and residential buildings. We also plan to apply the comparison and evaluation to more building ontologies to discover solid and generic ontology modelling and design patterns, and to automate the building ontology matching, alignment, and harmonisation. The Linked Building Data Community Group (LBD-CG)~\citep{lbd2023} has similar aims.

\item \textbf{Agent-OM System:} (1) Multimodal OM: We have packaged our system into several natural language-based commands. Our system could be integrated with advanced LLM functions to support multimodal input, such as ontology diagrams and online seminars. The richer information sources might improve OM performance. (2) Multilingual OM: Agent-OM supports ontologies in multiple languages. We tested it on the OAEI MultiFarm Track, an adapted conference dataset with ontologies translated into nine different languages. The results are not included here because there are few benchmarks available. (3) Small language models (SLMs) for OM: SLMs (e.g. gemma-2-2b) are useful in resource-constrained devices, but they have problematic tool interfaces at present.

\item \textbf{OM4OV Pipeline:} (1) While OM has a universal evaluation measure, our proposed measures for OV have four sub-measures. We plan to investigate a merged formula for OV sub-measures in the future, for example, using a harmonic mean to combine sub-measures. (2) We limit the semantic analysis to noting changes in 1-hop subgraph relations that can be either ontology keywords (such as domain, range, and subclass) or domain concepts as object properties. A more complete analysis of structural evolution could employ description-logic-based reasoning for subsumption checking, consistency validation, and detection of semantically equivalent expressions with only syntactic differences. This kind of analysis has not been previously explored in OM and is not addressed in this study, but could be worthwhile further work. (3) We plan to apply the OM4OV framework in emerging domain ontologies that demonstrate regular changes over time. We are working with the Brick Schema development team to encourage adoption of our OM4OV framework.

\item \textbf{Crowd-OM Validation:} We plan to adopt our crowdsourcing systems for reference evolution and ontology harmonisation and contribute to the creation of robust benchmarks for OM tasks.

\item \textbf{Ontology-Compliant Knowledge Graphs:} Further work will focus on justifying the results with the capability to allow ontology compliance on large-scale KGs, and implementing pattern-based compliance in a comprehensive framework that enables automatic ontology fragment integration, evaluation, and selection for real-world application-level KGs.

\end{itemize}

\section{Concluding Remarks}

Ontology interoperability has been a long-standing issue studied in the Semantic Web community. Since the establishment of the International Semantic Web Conference (ISWC), workshops on ontology design and patterns (WOP) and ontology matching (OM@ISWC) have been the two longest-running workshop proceedings. Ontology validation, which focuses on validating the correctness of the ontology, has been used in many ontology-driven applications.

This work explores ontology interoperability at scale. We propose a comprehensive framework that uses ontology design patterns, ontology matching and versioning, and ontology validation throughout the ontology engineering life cycle to improve ontology interoperability. We present several novel approaches for each technique. We expect our work to be an Archimedes' lever that cracks the nuts of ontology interoperability.

==> qiang-anu-thesis-content/qiang-anu-thesis-literature-review.tex <==
\section{Ontology Interoperability}

Ontology interoperability is a fundamental but critical issue in sharing and reusing ontologies across different applications. While various techniques have been applied in this area, this chapter provides a review of three dominant state-of-the-art semantic web techniques: ontology design patterns (ODPs), ontology matching and versioning (OM\&OV), and ontology validation (OVA). We analyse the advantages and disadvantages of each technique and identify opportunities to integrate them to build a comprehensive framework for ontology interoperability.

There is no doubt that using an ontology for knowledge graphs (KGs) can enhance KG interoperability through shared vocabularies and definitions, but the ontology itself is not interoperable. For example, Brick~\citep{balaji2016brick} and RECore~\citep{hammar2019realestatecore} are two popular ontologies in the building domain, but their coverage is different and they do not share the same concepts. Brick offers more detailed concepts for building sensors and actuators, while RECore is better at presenting spatial information about the building. The two ontologies also use different terminologies to describe identical concepts. For example, the building's physical location is referred to as ``Site'' in Brick and ``Land'' in RECore. A proposal~\citep{brickrec} to harmonise these two ontologies began in 2022, but to date, many concepts have remained unaligned. Moreover, this collaboration not only aims to align two building ontologies but also includes many other emerging alignments, such as the Brick alignment to two industry standards, Industry Foundation Classes (IFC)~\citep{pauwels2016express} and ASHRAE Standard 223P~\citep{s223p}.

Ontology interoperability is an essential requirement for ontology engineering. It is not possible for two applications that use different ontologies to communicate without aligning their concepts. Several research areas, such as ontology modularisation~\citep{ontologies2009concepts} and ontology selection~\citep{sabou2006ontology}, are highly dependent on the level of ontology interoperability. When a replacement cannot be found for an ontology entity, the extracted ontology module may treat it as missing. This will lead to an entirely different choice of the ontology.

In this chapter, we provide a comprehensive review of state-of-the-art semantic web techniques for ontology interoperability. These include ontology design patterns (ODPs), ontology matching and versioning (OM\&OV), and ontology validation (OVA). We review the current literature, identify knowledge gaps, and outline future directions. By leveraging their strengths while mitigating their weaknesses, we identify opportunities to build a comprehensive framework across these three techniques to improve ontology interoperability.

\section{Ontology Design Patterns}
\label{sec: odps}

\subsection{Overview}

Ontology design patterns (ODPs) are built on the concept of modularisation and reusability. While they are conceptually similar to modelling upper-level ontologies, ODPs aim to build the smallest and most reusable building blocks for constructing large ontologies~\citep{gangemi2005ontology,gangemi2009ontology,blomqvist2009experiments}. ODPs are extracted or re-engineered from existing ontologies. For example, the Actuation-Actuator-Effect (AAE) ODP is extracted from SAN~\citep{san}, while the Execution-Executor-Procedure (EEP) ODP is re-engineered from SEAS~\citep{seas}, SOSA~\citep{sosa}, SSN~\citep{ssn}, and DUL~\citep{dul}. Ontologies that follow the same ODP are interoperable. One can easily interpret identical ontology classes, properties, and individuals on the basis of shared patterns.

ODPs are not intended to serve as a complete ontology and provide only the design of an ontology part that can  be reused over many domains. A fully implemented ontology that reuses an ODP is commonly referred to as an exemplary ontology, which is often confused with ODPs. Figure~\ref{fig: ODP-Exemplary} shows an example of using the ``part of'' pattern in the ODP and the exemplary ontology for the building domain. The ODP contains only one ``hasPart'' and one ``isPartOf'', but the exemplary ontology repeats these terms multiple times to model domain-specific part-whole relationships among buildings, floors, and rooms.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\columnwidth]{qiang-lr-figures/ODP-Exemplary.png}
\caption{Ontology design pattern vs exemplary ontology.}
\label{fig: ODP-Exemplary}
\end{figure}

\subsection{Ontology Design Patterns in the Wild}

ODPs come in different types, including content ODPs for patterns of classes, properties, and relations, structural ODPs for logical and architectural issues, correspondence ODPs for reengineering and alignment, and other types such as reasoning, presentation, and lexico-syntactic ODPs~\citep{gangemi2009ontology}. Content ODPs are the most widely used ODPs~\citep{presutti2008content}.

The most well-known ODP repository is available at \url{https://odpa.github.io/patterns-repository/} (formerly \url{http://ontologydesignpatterns.org}), with documentation on domain usage and competency questions. ODPs have been used in many domains, such as bioinformatics~\citep{aranguren2008ontology}, geography~\citep{martinez2012logical}, cultural heritage~\citep{carriero2021pattern}, material science~\citep{vardeman2017ontology}, and energy efficiency in buildings~\citep{esnaola2018two}.

\subsection{Knowledge Gaps}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item Content ODPs dominate the current ODPs. We do not see many of the other types of ODPs available, but they can be useful in some cases.

\item Limited research is available on using machine learning (ML) or large language models (LLMs) to facilitate this process. The major problem is determining the level of abstraction for each ODP. Even with a number of samples provided, it seems challenging to apply a few-shot approach to train a model for this purpose.

\item Current ODPs are handcrafted by humans and validated on a case-by-case basis. This makes it challenging to apply ODPs in complex and emerging domains. For example, the building domain encompasses a mixture of building spaces, equipment and systems, points and measurements. We propose a set of ODPs in Chapter~\ref{chap: building-odps}.

\end{enumerate}

\section{Ontology Matching and Versioning}
\label{sec: omov}

\subsection{Overview}

Ontology matching (OM) aims to find similar concepts in different ontologies~\citep{euzenat2007ontology}. OM is also known as ontology alignment (OA), but OA is more commonly used to describe the OM process. Ontology versioning (OV) aims to capture the differences between different versions of an ontology~\citep{klein2001ontology}. It is easy to see that OV is a specific form of OM. In some contexts, ontology evolution is used as a synonym for OV, but OV is preferred because ontologies are not evolved naturally, but rather through human design. Ontologies are interoperable when their classes, properties, and individuals are explicitly aligned with OM\&OV. One can easily transfer terms from one ontology to another using a mapping that has been described in advance.

Given a pair of ontologies, the OM\&OV task can be formed by finding an alignment that contains a set of mappings~\citep{euzenat2007semantic}. OM\&OV tasks target equivalence commonly, as other relations (e.g. subsumption or disjointness) can be derived from equivalent mappings. For example, if A is equivalent to B and B is a subclass of C, then A should also be a subclass of C. Similarly, the OM\&OV task can be more complex and extended to one-to-many and many-to-many mappings, but the most common OM\&OV tasks target one-to-one mappings.

\subsection{Ontology Matching}

Figure~\ref{fig: roadmap-om} illustrates the roadmap of OM. Before ChatGPT (BC), a number of OM systems were developed using traditional logic-based expert systems and ML-based prediction systems. Following the introduction of ChatGPT in 2022~\citep{chatgpt}, there was a brief period of using a purely LLM-based approach to perform OM tasks. Due to the current limitations of LLMs, the period after destress (AD) aims to use LLMs with enhancements.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\columnwidth]{qiang-lr-figures/Roadmap-OM.png}
\caption{Roadmap of ontology matching (OM).}
\label{fig: roadmap-om}
\end{figure}

\newpage

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item Logic-based systems are highly dependent on domain expertise, and mapping is mainly based on the interpretation of logic expressions within the ontology. Typical logic-based OM systems include LogMap~\citep{jimenez2011logmap1}~\citep{jimenez2011logmap2}, AgreementMakerLight (AML)~\citep{faria2013agreementmakerlight}~\citep{faria2014agreementmakerlight}, and FCA-Map~\citep{zhao2018matching}~\citep{li2021combining}. Such systems generally compile the results quickly with acceptable performance for simple OM tasks. However, these systems face a bottleneck that prevents them from performing complex OM tasks. It is not known how to capture a comprehensive list of logic expressions in various domains and applications.

\item ML-based systems are derived from the popular concept of machine learning in the field of artificial intelligence (AI). LogMap-ML~\citep{chen2021augmenting} and BERTMap~\citep{he2022bertmap} are successful examples. Such systems typically include a learning process that requires a certain amount of training data for the model to learn patterns and make predictions. As with ML applications in other domains, ML-based systems face the challenge of sampling high-quality training data from the full dataset. The explainability of a trained model is a long-standing issue within the scope of explainable AI (XAI)~\citep{arrieta2020explainable}.

\item LLM-based systems refer to systems that use LLMs directly for OM. In the early stages of using LLMs for OM, a general approach is to feed ontologies into the LLM entirely with prompt instructions. Such examples can be found in~\citep{he2023exploring} and~\citep{norouzi2023conversational}. The scalability of this approach is problematic. For large-scale ontologies, it may not be feasible to feed the entire ontology into LLMs due to input token limits. In addition, these systems often exhibit low precision and recall due to the inherent hallucinations associated with LLMs.

\item LLM-enhanced systems aim to re-engineer the LLM-based infrastructure for OM because current LLMs are not fully feasible for this domain-specific task. This field is a new research area with two main streams. One is using retrieval-augmented generation (RAG)~\citep{lewis2021retrievalaugmented} to inject external resources and extend the knowledge base of LLMs. This often results in the introduction of novel LLM-based architectures for OM tasks, such as~\citep{hertling2023olala,giglou2024llms4om,zhang2024large,taboada2025ontology,nguyen2025kroma}. The other stream aims to feed external knowledge into LLMs by training or fine-tuning, as in~\citep {he2024language,sousa2025complex,yang2025language}.

\end{enumerate}

Table~\ref{tab: om-system-type} summarises the pros and cons of different types of OM systems. While LLM-enhanced architectures are the state-of-the-art solution for OM systems, they also suffer from high cost and non-determinism, which can be mitigated by integrating traditional system designs.

\begin{sidewaystable*}
\centering
\renewcommand\arraystretch{1.2}
\tabcolsep=0.15cm
\caption{Pros and cons of different types of ontology matching systems.}
\label{tab: om-system-type}
\begin{tabular}{|m{3.2cm}|m{9cm}|m{10cm}|} \hline
\textbf{System Type} & \textbf{Pros} & \textbf{Cons} \\ \hline
Logic-Based
&\begin{itemize}[left=0pt]
\item Acceptable performance for simple tasks
\item Fast and requires low computational power
\end{itemize}
&\begin{itemize}[left=0pt]
\item Requires extensive domain expertise
\item Meet the bottleneck for complex OM tasks
\end{itemize}
\\ \hline
ML-Based
&\begin{itemize}[left=0pt]
\item High accuracy in trained models
\item Models can be generalised for different domains
\end{itemize}
&\begin{itemize}[left=0pt]
\item Lack of high-quality training data
\item Lack of explainability
\end{itemize}
\\ \hline
LLM-Based
&\begin{itemize}[left=0pt]
\item Ease of use with intuitive prompt engineering
\item Provides mapping explanations
\end{itemize}
&\begin{itemize}[left=0pt]
\item Not scalable for large-scale ontologies
\item Low accuracy caused by LLM hallucinations
\end{itemize}
\\ \hline
LLM-Enhanced
&\begin{itemize}[left=0pt]
\item High accuracy in complex tasks
\item Provides precise mapping explanations
\end{itemize}
&\begin{itemize}[left=0pt]
\item Extensive burden for system re-engineering
\item Dynamic outputs due to the LLM non-determinism
\end{itemize}
\\ \hline
\end{tabular}
\end{sidewaystable*}

\subsection{Ontology Versioning}

Figure~\ref{fig: roadmap-ov} illustrates that there are two dominant approaches to OV tasks. One approach is to document versioning information within the ontology and expose it as additional triples. The other approach is to document the versioning information outside the ontology, as a complement to the ontology.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\columnwidth]{qiang-lr-figures/Roadmap-OV.png}
\caption{Roadmap of ontology versioning (OV).}
\label{fig: roadmap-ov}
\end{figure}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item Versioning information within the ontology requires an extension of the current vocabulary. OWL has adopted several annotation properties related to versioning information. These include version tags (versionInfo and priorVersion), compatible tags (backwardCompatibleWith and incompatibleWith), and deprecated tags (DeprecatedClass and DeprecatedProperty). On the other hand, $\tau$OWL~\citep{zekri2016tau} and RDF 1.2~\citep{rdf12} have extended a fourth dimension within the quadruples to capture versioning information. However, this approach can consistently increase the size of the ontology, making it unsuitable for large and rapidly evolving ontologies.

\item Attaching versioning information to the ontology can be done in many ways. Versioning information can be captured as a log~\citep{plessers2005ontology}, a standalone KG~\citep{cardoso2020construction}, or a network of KGs~\citep{sassi2016supporting}. While this approach is more flexible in its support for formats and does not increase the size of the ontology, it requires additional control and stores versioning files.

\end{enumerate}

\subsection{Knowledge Gaps}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item In the era of LLMs, LLMs offer extensive capabilities to perform OM tasks. It is questionable whether the logic and ML used in classical OM systems remain useful in modern LLM-based systems.

\item LLMs are useful tools for OM, but OM systems are complex and lack centralised control, which cannot meet the requirements for large-scale automation. LLM agents could be an interesting area to explore, and LLM hallucinations need to be properly understood and mitigated. We present our novel LLM agents for OM tasks in Chapter~\ref{chap: agent-om}.

\item OV is similar to OM, but it is unclear whether the pipeline for OM tasks can be reused for OV tasks. There is no unified pipeline that combines OM and OV. We solve this problem in Chapter~\ref{chap: om4ov}.

\end{enumerate}

\section{Ontology Validation}
\label{sec: ova}

\subsection{Overview}

Ontology validation (OVA) aims to check the compliance of the ontology. OVA is sometimes confused with ontology verification (OVF), but the two have different goals. OVF refers to ``Do we build the ontology correctly?'', while OVA refers to ``Do we build the correct ontology?''. In other words, OVF ensures that the ontology is intrinsically correct, while OVA ensures that the ontology is extrinsically meaningful.

\subsection{Ontology Matching Validation}

OM outputs cannot be directly used for downstream tasks. It is essential to include a validation step to ensure that the matching outputs align with real-world facts. This process is also known as ``matching repair'', which aims to identify counter-intuitive mappings that are mistakenly detected by OM systems. OM validation can be classified into two categories.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item Logic-based validation via the traditional approach uses reasoners (e.g. FaCT++~\citep{tsarkov2006fact}, Pellet~\citep{sirin2007pellet}, and HermiT~\citep{glimm2014hermit}) to perform a coherence check on the mappings. OM outputs are formed as assertions and combined with the original ontology. A mapping is incorrect if the reasoner finds that the internal rules within the ontology have been violated. Recently, this validation has been extended to use LLM prompts to verify the correctness of mappings~\citep {diallo2025ontology,lushnei2026large,condeherreros2026llm}.
\item Human-in-the-loop validation uses human experts to validate the OM outputs. Common methods include surveys, interviews, and workshops. Several studies~\citep{paulheim2013towards,dragisic2016user,li2019user} have shown that the effectiveness of human-in-the-loop validation is highly dependent on the user groups selected, the user interface used, and the instructions provided.
\end{enumerate}

\subsection{Data-Driven Ontology Validation}

One common type of OVA is to apply ontologies to a specific task or application and validate them using data instances. This process is known as data-driven ontology validation (DDOV). Ontologies that conform to the same data are interoperable. One can easily determine mappings between ontologies if entities are assigned to the same instance. KGs are the data most commonly used for DDOV. Depending on different assumptions and baselines, DDOV can be categorised into two types: ontology-based KGs and ontology-aware KGs. Ontology-based KGs assume the ontology is complete, and KGs need to be modified if they do not conform to the ontology. On the other hand, ontology-aware KGs treat KGs as baselines, and the ontology needs to be modified if it does not conform to them. In the literature, modifying the ontology of an ontology-aware KG is also referred to as ontology enrichment~\citep{petasis2011ontology} and ontology reshaping~\citep{zhou2021towards,zhou2022enhancing,zhou2022ontology}.

Ontology-based KGs validate KGs based on the given ontology. For example, in SSN, ``Feature of Interest'' is defined as the object of ``Observation'' in the ontology. Linking ``Feature of Interest'' directly to a ``Sensor'' in the KG violates this rule. Shapes Constraint Language (SHACL)~\citep{shacl2017} is the W3C recommendation to validate KGs that comply with the ontology. SHACL provides more comprehensive and extensible validation than the built-in logical expressions in the ontology. SHACL allows KGs to conform to a specific ``shape'' defined by the end user. This ``shape'' can be a simple triple, but it can also be a complex shape graph.

Ontology-aware KGs validate the ontology against the given KGs, identifying missing or unused concepts. Ontology enrichment is the process of adding missing concepts to the ontology. For example, if the KG contains multiple kinds of temperature, such as room temperature and HVAC temperature, then the ontology needs to add the new class ``Temperature'' as a kind of ``Observable Property''. Ontology reshaping is the process of removing unused concepts from the ontology. For example, if the KG is only related to sensor observation, then ``Actuation'' used for an actuator can be removed from the ontology.

\subsection{Knowledge Gaps}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item OM validation with human-in-the-loop is labour-intensive. It is not easy to find domain experts and they may also have biases. Using an LLM as an alternative is feasible but introduces the risk of LLM hallucinations, which can reduce the quality of OM validation. We introduce a novel crowdsourcing approach in Chapter~\ref{chap: om-validation}.

\item In reality, ontologies are inherently incomplete. Although ontology-based KGs have been applied to many domains, they are not always applicable, especially in emerging domains where concepts are evolving rapidly. While ontology enrichment adds new concepts and ontology reshaping deletes unused concepts, there is a need to support adding, deleting, and updating functions concurrently. Moreover, ontology-aware KGs assume that the selected ontology is the optimal choice for the given KGs. Limited attention has been paid to finding an optimal ontology from a number of candidates or pattern-based ontology fragments. We propose a new concept of ontology-compliant KGs in Chapter~\ref{chap: ockgs}.

\item There are no standard evaluation metrics and datasets for OVA. This limitation makes it difficult to choose an ontology. For example, the decision can vary when one concept is missing from one ontology and misinterpreted in another.

\end{enumerate}

\section{Discussion}
\label{sec: discussion}

Table~\ref{tab: compare-technique} compares three state-of-the-art semantic web techniques for ontology interoperability. We can see that ODPs, OM\&OV, and DDOV differ from several perspectives, including prerequisite, concept coverage, alignment approach and schema, and medium used.

\begin{sidewaystable*}
\centering
\renewcommand\arraystretch{1.2}
\tabcolsep=0.15cm
\caption{Comparison of three state-of-the-art semantic web techniques for ontology interoperability: ontology design patterns (ODPs), ontology matching and versioning (OM\&OV), and ontology validation (OVA).}
\label{tab: compare-technique}
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{|c|c|c|c|c|c|} \hline
\textbf{Technique} & \textbf{Prerequisite}   & \textbf{Concept Coverage}    & \textbf{Alignment Approach}   & \textbf{Alignment Schema} & \textbf{Medium Used}    \\ \hline
ODPs               & Ontologies Only         & Commonalities Only           & Align Conceptual Model        & Hub-and-Spoke             & Common Patterns         \\ \hline
OM\&OV             & Ontologies Only         & Commonalities + Differences  & Align Ontology Entities       & Pairwise                  & N/A                     \\ \hline
OVA               & Ontologies + References & Differences Only              & Align human values/instances  & Hub-and-Spoke             & Knowledge Graphs        \\ \hline
\end{tabular}
\end{adjustbox}
\end{sidewaystable*}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item ODPs provide high-level guidelines for building ontologies. ODPs achieve ontology interoperability by aligning the conceptual model. This approach often extracts common patterns across different ontologies in a hub and ignores their differences. ODPs can be reused across different ontologies.

\item OM\&OV aim to find the corresponding mappings between two ontologies. OM\&OV achieve ontology interoperability by aligning ontology entities. While OM only reports aligned entities between ontologies (i.e. commonalities), OV also reports unaligned entities (i.e. differences).

\item OVA validates the ontologies to align with human values and data instances. OM validation serves as a prerequisite for DDOV, and DDOV achieves ontology interoperability by aligning the data instances. This approach typically applies a KG hub across multiple ontology spokes. Both OM validation and DDOV process need reference alignments to identify commonalities between ontologies and thereby highlight their differences.

\end{enumerate}

These three techniques can work independently for ontology interoperability, but they also have some inter-dependencies. Therefore, there are opportunities to develop a framework that leverages their strengths while mitigating their weaknesses.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]

\item ODPs provide only high-level guidelines for conceptual modelling and lack detailed mappings between classes, properties, and individuals. ODPs often need to cooperate with OM\&OV and OVA in downstream tasks.

\item  OM\&OV provide detailed mappings for classes, properties, and individuals, but with limited support from the modelling perspective. ODPs can simplify the OM\&OV process. Ontologies that use the same ODP are much easier to align, as they share the same conceptual model. The output of OM\&OV can serve as a reference for OVA.

\item OVA is an evaluation process and does not provide any mappings by nature. OVA reuses the commonalities generated by OM\&OV and thereby identifies missing or overlapping modelling issues. The output of OVA can be used to optimise existing ODPs in the next cycle. For example, the legacy ODP used in IoT-Lite~\citep{bermudez2016iot} lacks the concepts for modelling sensor observations and needs to be updated or replaced with alternative ODPs.

\end{enumerate}

While the introduction of ontologies aims to enable interoperability among KGs, with numerous ontologies developed for different domains and purposes, ontology interoperability is becoming a bottleneck for sharing and reusing ontologies in real-world applications. In this chapter, we review three dominant semantic web techniques for ontology interoperability. We observe that each targets a specific perspective on ontology interoperability and differs in strengths and weaknesses. The inter-dependencies between ODPs, OM\&OV, and OVA offer opportunities to develop a comprehensive framework for ontology interoperability.

We now present our contributions in the following chapters. Chapter~\ref{chap: building-odps} focuses on ontology design patterns (ODPs), Chapters~\ref{chap: agent-om} and~\ref{chap: om4ov} emphasise ontology matching and versioning (OM\&OV), and Chapters~\ref{chap: om-validation} and~\ref{chap: ockgs} concentrate on ontology validation (OVA). Chapter~\ref{chap: conclusion} proposes a guideline for creating an interoperable ontology and summarises our contributions, future work, and broader directions.

\paragraph*{Publication Statement}

Most of the work presented in this chapter has been published as~\bibentry{qiang2025ecosystem}.

==> qiang-anu-thesis-content/qiang-anu-thesis-outline.tex <==
\section{Thesis Outline}

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=\textbf{Chapter \arabic*:}]

\item \textbf{Introduction.} We begin with a Socratic questioning ``Is the ontology itself interoperable?'' and highlight the importance of ontology interoperability for data exchange and integration within knowledge graphs (KGs). A running example in the building domain illustrates the effectiveness of using ontology design patterns (ODPs), ontology matching and versioning (OM\&OV), and data-driven ontology validation (DOVA) across different phases of the ontology engineering life cycle to build a comprehensive framework for ontology interoperability.

\item \textbf{Literature Review.} We provide a comprehensive review of the state-of-the-art semantic web techniques for ontology interoperability, including ontology design patterns (ODPs), ontology matching and versioning (OM\&OV), and data-driven ontology validation (DOVA). We analyse the advantages and disadvantages of each technique and identify opportunities to integrate them to develop a framework for ontology interoperability~\cite{qiang2025ecosystem}.

\item \textbf{Ontology Design Patterns (ODPs).} We systematically analyse four popular ontologies used in the smart building domain and identify the merits and drawbacks of each. We propose building ODPs to capture common and well-agreed concepts and relations in the building domain, including building spaces, equipment and systems, points and measurements~\cite{qiang2023systematic}.

\item \textbf{Ontology Matching and Versioning (OM\&OV).} We develop a novel software system for OM (Agent-OM~\cite{qiang2023agent}) and an extension for OV (Agent-OV~\cite{qiang2024om4ov}). Agent-OM uses state-of-the-art LLM agents that leverage infrastructure to deliver improved OM performance in a fully-automated and domain-independent manner. Agent-OV extends Agent-OM to explicitly target OV tasks, including new task formulation and evaluation, with a cross-reference mechanism that compiles OM tasks. Agent-OM is used to create an LLM hallucination dataset~\cite{qiang2024oaei} for the LLM leaderboard and LLM fine-tuning for OM. Agent-OM also participates in the Ontology Alignment Evaluation Initiative (OAEI)~\cite{oaei} 2025 campaign and showcases its generative capability in handling OM tasks at various levels of granularity~\cite{qiang2025oaei}.

\item \textbf{Data-Driven Ontology Validation (DOVA).} We propose ontology-compliant knowledge graphs (OCKGs) and define three subtasks under OCKGs: ontology compliance within KG, ontology compliance over KGs, and pattern-based compliance. Examples from the building domain demonstrate the process of constraining OCKGs and highlight their efficiency in facilitating ontology validation and decision-making~\cite{qiang2023ontology}.

\item \textbf{Conclusion.} We summarise the contributions made, including several novel solutions for improving ontology design patterns (ODPs), ontology matching and versioning (OM\&OV), and data-driven ontology validation (DOVA). In addition, we outline ongoing work and future directions for applying semantic web techniques to improve ontology interoperability.

\end{enumerate}

==> qiang-anu-thesis-content/qiang-anu-thesis-problem-statement.tex <==
An ontology is ``a formal and explicit specification of a shared conceptualisation''~\citep{gruber1993translational}. Ontologies are commonly used to define terms and relations in a domain of interest, for example, for web pages, catalogues, map search, electronic health records, medical billing, and biological taxonomy. Ontologies improve semantic interoperability for data integration and knowledge sharing. But is an ontology interoperable with others?

Ontologies are crafted by domain experts based on their understanding of the domain of application. There is no guarantee that ontologies in the same domain share the same conceptualisation. Describing a person can use their basic profile (e.g. name, age, and gender), social relationships (e.g. parent-child and friendship), or professional roles (e.g. student and employee). The terminology used in the ontologies may vary.  For example, one ontology can use ``first name'' and ``last name'' to describe a person's full name, and another ontology can use ``given name'' and ``family name'' instead. These concepts need to be harmonised for data conforming to each ontology to be shared across applications. Therefore, ontology interoperability has become a critical issue that limits sharing data and the reuse of ontologies.

Knowledge graphs (KGs) can use ontologies as the backbone. In particular, ontologies serve to provide extensive information for interpreting KGs. KGs are commonly formed as a set of triples, each consisting of a subject, a predicate, and an object. KGs are sometimes not easy to understand. For example, the KG triple (Sydney, travelsTo, Sydney) may cause confusion. We can use an ontology to help. With an ontology that defines a class expression (Person, travelsTo, Place), one can infer that the subject ``Sydney'' refers to a person who is travelling, while the object ``Sydney'' refers to the place being travelled. The KG triple (Sydney, travelsTo, Sydney) describes a filming event in which the American actress Sydney Sweeney travels to the city of Sydney~\citep{sweeney2023}.

\newpage

For large-scale KGs, the use of ontologies has become the general practice for enabling semantic interoperability among KGs. With the increasing size and number of ontologies, the lack of interoperability among ontologies has become apparent and hampers their use in many real-world applications. Missing, overlapping, and conflicting concepts in different ontologies impede data exchange and integration. While several approaches have been proposed for ontology interoperability, they often operate on a case-by-case basis. However, ontology interoperability is a complex issue that can arise at any phase of the ontology engineering (OE) cycle. Currently, there is no streamlined approach to improving ontology interoperability throughout the OE life cycle.

==> qiang-anu-thesis-content/qiang-anu-thesis-publication-statement.tex <==
\paragraph*{Publication Statement}

Most of the work presented in this chapter has been published as~\bibentry{qiang2025ecosystem}.

==> qiang-anu-thesis-content/qiang-anu-thesis-research-context.tex <==
\section{Research Context}
\label{sec: research-context}

\subsection{Ontology}

The ontology is the cornerstone of KGs. KGs built from an ontology are much easier to interpret and understand. Figure~\ref{fig: ontology-kg} shows an example of using an ontology for KGs. The KG describes an event where Glen Powell and Sydney Sweeney travel to the city of Sydney to film a romantic comedy movie ``Anyone But You''~\citep{sweeney2023}. The triples (Glen, travelsTo, Sydney) and (Sydney, travelsTo, Sydney) are triples of the KG, while the triples (travelsTo, domain, Person) and (travelsTo, range, Place) are triples of the ontology. The ontology triples derived from the KG triple (Glen, travelsTo, Sydney) can be used to explain the perplexing KG triple (Sydney, travelsTo, Sydney). By using definitions provided by the ontology, it is easier to infer that the first subject entity ``Sydney'' refers to the person Sydney Sweeney, while the second object entity ``Sydney'' refers to the city of Sydney.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\columnwidth]{qiang-lr-figures/Ontology-KG.png}
\caption{An example of using an ontology to explain a knowledge graph.}
\label{fig: ontology-kg}
\end{figure}

The ontology also provides extensive logical expressions for KGs to represent implicit knowledge from which explicit consequences may be deductively inferred, and to represent constraints on explicit knowledge that may be used to detect violations that are considered to be errors in the KGs. Figure~\ref{fig: ontology-restriction} shows several examples of using logical expressions within the ontology. A person can travel to many places (Restriction 1), but can live in only one place (Restriction 2). If a person travels, they travel to a place (Restriction 3). Every person lives in a place (Restriction 4). These pieces of information cannot be represented in KGs, but can be modelled as machine-readable restrictions within the ontology.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\columnwidth]{qiang-lr-figures/Ontology-Restriction.png}
\caption{Examples of using logical expressions within the ontology.}
\label{fig: ontology-restriction}
\end{figure}

Developing an ontology is not easy and requires extensive domain knowledge, but once it is developed, the ontology can be used across multiple KGs. Both the ontology and the KGs form a set of triples (subject, predicate, object). Still, ontology provides term definitions for entity types (e.g. class, property, individual) as well as more advanced logical expressions (e.g. domain, range, and restriction). These terms can be modelled and formatted in the Web Ontology Language (OWL)~\citep{owl2004} and other languages, such as Resource Description Framework Schema (RDFS)~\citep{rdfs2014} and Simple Knowledge Organisation System (SKOS)~\citep{skos2009}, both of which are strongly tied to OWL.

In general, the ontology serves as the conceptual model, whereas KGs store data instances. There is one exception: a data instance can be defined as an individual within the ontology, but its existence also means that the data instance (i.e. individual) is a well-agreed term that is not always changeable. For example, the term ``Sydney'' can be defined as an individual within the ontology. KGs do not always require an ontology. For some domains, ontology-free KGs are a more rational choice compared to ontology-based KGs. For example, building an ontology for social media is not recommended due to the rapid evolution of terms and the lack of universal agreement. In this context, ``tags'' are commonly used as metadata to describe the content of utterances.

An ontology contains classes, properties, and individuals. In this work, the word \textit{entity} (or equivalently \textit{term} and \textit{concept}) is a general expression for ontology classes, object properties, datatype properties, or individuals (without specifying which). We use \textit{entity uri} to mean a fully expanded entity identifier with respect to its prefix. We use \textit{entity name} to mean an entity identifier trimmed of its prefix.

\subsection{Ontology Interoperability}

Ontologies have been used for decades to improve the interoperability of KGs and relational databases. However, a criticised view is that the ontology itself is not interoperable. An ontology can be built from scratch or reused from existing ontologies, but there is no guarantee that an ontology always contains the same concepts as other ontologies. Overlaps and missing concepts may exist, making it difficult to share and reuse an ontology in different applications. There are various types of interoperability issues in the ontology~\citep{doric-mm-2021}.

\begin{enumerate}[wide, noitemsep, topsep=0pt, labelindent=0pt, label=(\roman*)]
\item Formatting interoperability. The ontology can be expressed as OWL, RDF, or XML. There is a known issue with transferring ontologies to different languages due to differences in their levels of expressiveness.
\item Terminological interoperability. The ontology can use different terminologies to describe the same concepts. For example, ``AHU'' and ``Air Handling Unit''.
\item Logical interoperability. The same concepts can have different meanings in different ontologies. For example, if the class ``Meter'' is the subclass of ``Point'', it means a data point; if the class ``Meter'' is the subclass of ``Device'', it means a physical device.
\item Semantic interoperability. The same concepts can be modelled from different perspectives. For example, the class ``HVAC Zone'' can be logically considered as a functional unit or physically as a concrete spatial element.
\item Contextual interoperability. The same concepts can have different meanings in different domains. For example, the class ``System'' refers to a software application in the building domain, but means a set of organs in human anatomy.
\end{enumerate}

\subsection{How Do Ontologies Interoperate?}

\textbf{Ontology design patterns (ODPs)} identify common ontology fragments across different ontologies~\citep{gangemi2009ontology}. ODPs use a hub-and-spoke matching approach. Once the ODP is determined, each subsequent ontology will conform to this ODP, and the ODP serves as a high-level abstract model to guide the design of these new ontologies. ODPs have some limitations. Firstly, ODPs are conceptual models and do not prescribe the identifiers for entities. This means that it is not possible to control terminology, and ontology creators remain free to make their own choices. Secondly, ODPs are commonly handcrafted based on existing ontologies. They are static and tend not to capture changes over time. Thirdly, the choice of ODPs is entirely reliant on one's experience and preferences; the favoured ODPs may be overwhelming, overlapping, or not applicable for a given KG.

\textbf{Ontology matching and versioning (OM\&OV)} aim to find mappings between different ontologies~\citep{euzenat2007ontology} or different versions of the same ontology~\citep{klein2001ontology}. OM\&OV conform to a pairwise matching approach. This means that each mapping is a pairwise process to find the correspondences between two ontologies. OM\&OV are typically resource-intensive. The complexity of pairwise mapping is proportional to the product of the number of entities in the two ontologies. The pairwise mapping process also needs to be repeated multiple times if multiple ontologies exist. Moreover, OM\&OV tasks focus on conceptual-to-conceptual and instance-to-instance matching, and less attention has been paid to the alignment between conceptual models and data instances.

\textbf{Ontology validation (OVA)} aims to answer the question ``Do we build the ontology correctly?'', in other words, to ensure that the ontology is extrinsically meaningful. In this work, we use OVA to validate interoperability among entities defined in different ontologies. OVA can be performed at the conceptual and instance levels. The former often requires domain experts to manually validate the proposed mappings, whereas the latter typically uses real-world data to validate the effectiveness of an ontology. Today, with the increasing number of domains and applications using ontologies, it is not easy to find domain experts and experts may also have knowledge boundaries for OVA tasks. On the other hand, validating the ontology on KGs is challenging. To determine which candidate ontology best fits the given KG, the KG needs to be modelled for each candidate ontology. This process essentially involves aligning the candidate ontologies, informed by the KG under study.

In addition to these three popular approaches, other methods have been proposed for ontology interoperability, most notably the use of upper ontologies. For example, the upper ontology Basic Formal Ontology (BFO)~\citep{arp2015building} aims to provide a common conceptual model as a foundation for extension to domain-specific ontologies. However, these approaches have been shown to have significant limitations, such as a lack of universal agreement, challenging complex modelling, and inconsistent adoption~\citep{mascardi2007comparison,mascardi2009automatic,schmidt2019matching,haller2020we,trojahn2022foundational}.

==> qiang-anu-thesis-content/qiang-anu-thesis-statement.tex <==
\section{Thesis Statement}

In this work, we aim to build a comprehensive ontology interoperability framework for industry-scale applications. We review three state-of-the-art semantic web techniques: ontology design patterns (ODPs), ontology matching and versioning (OM\&OV), and ontology validation (OVA). By analysing the pros and cons of these techniques, we hypothesise that using these three techniques across different phases of the ontology engineering (OE) life cycle can foster strengths and circumvent weaknesses, thereby streamlining a workflow model for ontology interoperability.

Figure~\ref{fig: overview} illustrates an overview of the framework. Similar to software engineering, OE involves three main phases: design, develop, and deploy. We propose to employ ODPs, OM\&OV, and OVA in different phases. (1) The design phase is responsible for understanding the requirements and creating a blueprint or prototype. In OE, these requirements are collected by competency questions. ODPs can serve as a skeleton to create conceptual models based on competency questions. (2) The develop phase includes turning the prototype into a full product and applying a unit test. In OE, this phase is referred to as ontology construction and evaluation. OM\&OV can be used to evaluate the level of interoperability between two ontologies, or between an ontology and its previous version. (3) The deploy phase usually refers to implementing the product in the real world. In OE, we refer to this as validating the ontology against human values and real-world data instances via OVA, thereby enhancing the design of the ontology in the next cycle.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\linewidth]{qiang-iswc-2026-dc-figures/Framework.png}
\caption{An overview of the framework. We propose to use ODPs in the design phase, OM\&OV in the develop phase, and OVA in the deploy phase to achieve better ontology interoperability.}
\label{fig: overview}
\end{figure}

==> qiang-anu-thesis-content/qiang-anu-thesis-timeline.tex <==
\section*{Proposed Timeline (Deprecated)}

\begin{itemize}[wide, noitemsep, topsep=0pt, labelindent=0pt]
\item 31/01/2026 - 28/02/2026: Chapter 3 and Chapter 4.
\item 01/03/2026 - 15/04/2026: Chapter 1 and Chapter 2.
\item 16/04/2026 - 15/05/2026: Chapter 5 and Chapter 6.
\item 16/05/2026 - 31/05/2026: Abstract and References.
\item 01/06/2026 - 17/07/2026: Supervisor Review and Compliance Check.
\end{itemize}
